BiGONLight: a new package for computing optical observables in Numerical Relativity

The investigation of relativistic effects in the most general way requires a unified treatment of light propagation in cosmology. This goal can be achieved with the new interpretation of the geodesic deviation equation in terms of the bilocal geodesic operators (BGO). The BGO formalism extends the standard formulation, providing a unified framework to describe all possible optical phenomena due to the interaction between light and spacetime curvature. In my dissertation, I present {\tt BiGONLight}, a {\tt Mathematica} package that applies the BGO formalism to study light propagation in numerical relativity. The package encodes the 3+1 bilocal geodesic operators framework as a collection of {\tt Mathematica} functions. The inputs are the spacetime metric plus the kinematics of the observer and the source in the form of the 3+1 quantities, which may come directly from a numerical simulation or can be provided by the user as analytical components. These data are then used for ray tracing and computing the BGOs in a completely general way, i.e. without relying on symmetries or specific coordinate choices. The primary purpose of the package is the computation of optical observables in arbitrary spacetimes. The uniform theoretical framework of the BGO formalism allows for the extraction of multiple observables within a single computation, while the {\tt Wolfram} language provides a flexible computational framework that makes the package highly adaptable to perform both numerical and analytical studies of light propagation.

==> ms <==
 \newcommand{\noop}[1]{}
\begin{thebibliography}{100}

\bibitem{abbott2016observation}
{\sc Abbott, B.~P., Abbott, R., Abbott, T., Abernathy, M., Acernese, F.,
  Ackley, K., Adams, C., Adams, T., Addesso, P., Adhikari, R., et~al.}
\newblock Observation of gravitational waves from a binary black hole merger.
\newblock {\em Physical review letters 116}, 6 (2016), 061102.

\bibitem{Adamek:2020jmr}
{\sc Adamek, J., Barrera-Hinojosa, C., Bruni, M., Li, B., Macpherson, H.~J.,
  and Mertens, J.~B.}
\newblock {Numerical solutions to Einstein's equations in a shearing-dust
  Universe: a code comparison}.
\newblock {\em Class. Quant. Grav. 37}, 15 (2020), 154001.

\bibitem{Adamek:2018rru}
{\sc Adamek, J., Clarkson, C., Coates, L., Durrer, R., and Kunz, M.}
\newblock {Bias and scatter in the Hubble diagram from cosmological large-scale
  structure}.
\newblock {\em Phys. Rev. D 100}, 2 (2019), 021301.

\bibitem{Adamek:2013wja}
{\sc Adamek, J., Daverio, D., Durrer, R., and Kunz, M.}
\newblock {General Relativistic $N$-body simulations in the weak field limit}.
\newblock {\em Phys. Rev. D 88}, 10 (2013), 103527.

\bibitem{adamek2016general}
{\sc Adamek, J., Daverio, D., Durrer, R., and Kunz, M.}
\newblock General relativity and cosmic structure formation.
\newblock {\em Nature physics 12}, 4 (2016), 346--349.

\bibitem{Adamek:2016zes}
{\sc Adamek, J., Daverio, D., Durrer, R., and Kunz, M.}
\newblock {gevolution: a cosmological N-body code based on General Relativity}.
\newblock {\em JCAP 1607}, 07 (2016), 053.

\bibitem{adamek2014distance}
{\sc Adamek, J., Di~Dio, E., Durrer, R., and Kunz, M.}
\newblock Distance-redshift relation in plane symmetric universes.
\newblock {\em Physical Review D 89}, 6 (2014), 063543.

\bibitem{Adamek:2014xba}
{\sc Adamek, J., Durrer, R., and Kunz, M.}
\newblock {N-body methods for relativistic cosmology}.
\newblock {\em Class. Quant. Grav. 31}, 23 (2014), 234006.

\bibitem{planck2020CMB}
{\sc Aghanim, N., Akrami, Y., Ashdown, M., Aumont, J., Baccigalupi, C.,
  Ballardini, M., Banday, A.~J., Barreiro, R., Bartolo, N., Basak, S., et~al.}
\newblock Planck 2018 results-v. cmb power spectra and likelihoods.
\newblock {\em Astronomy \& Astrophysics 641\/} (2020), A5.

\bibitem{planck2018param}
{\sc Aghanim, N., et~al.}
\newblock {Planck 2018 results. VI. Cosmological parameters}.
\newblock {\em Astron. Astrophys. 641\/} (2020), A6.

\bibitem{planck2019anl}
{\sc Akrami, Y., et~al.}
\newblock {Planck 2018 results. IX. Constraints on primordial non-Gaussianity}.
\newblock {\em Astron. Astrophys. 641\/} (2020), A9.

\bibitem{Alcubierre2008}
{\sc Alcubierre, M.}
\newblock {\em Introduction to 3+ 1 numerical relativity}, vol.~140.
\newblock Oxford University Press, 2008.

\bibitem{Aleksandrov1979}
{\sc Aleksandrov, A.~N., and Piragas, K.~A.}
\newblock Geodesic structure.
\newblock {\em Theoretical and Mathematical Physics 38}, 1 (Jan 1979), 48--56.

\bibitem{alexander2009local}
{\sc Alexander, S., Biswas, T., Notari, A., and Vaid, D.}
\newblock Local void vs dark energy: confrontation with wmap and type ia
  supernovae.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2009}, 09 (2009),
  025.

\bibitem{arnowitt1959}
{\sc Arnowitt, R., Deser, S., and Misner, C.~W.}
\newblock Dynamical structure and definition of energy in general relativity.
\newblock {\em Phys. Rev. 116\/} (Dec 1959), 1322--1330.

\bibitem{baiotti2008accurate}
{\sc Baiotti, L., Giacomazzo, B., and Rezzolla, L.}
\newblock Accurate evolutions of inspiralling neutron-star binaries: Prompt and
  delayed collapse to a black hole.
\newblock {\em Physical Review D 78}, 8 (2008), 084033.

\bibitem{baker2006gravitational}
{\sc Baker, J.~G., Centrella, J., Choi, D.-I., Koppitz, M., and van Meter, J.}
\newblock Gravitational-wave extraction from an inspiraling configuration of
  merging black holes.
\newblock {\em Physical review letters 96}, 11 (2006), 111102.

\bibitem{Barausse:2005nf}
{\sc Barausse, E., Matarrese, S., and Riotto, A.}
\newblock {The Effect of inhomogeneities on the luminosity distance-redshift
  relation: Is dark energy necessary in a perturbed Universe?}
\newblock {\em Phys. Rev. D 71\/} (2005), 063537.

\bibitem{bardeen1980gauge}
{\sc Bardeen, J.~M.}
\newblock Gauge-invariant cosmological perturbations.
\newblock {\em Physical Review D 22}, 8 (1980), 1882.

\bibitem{barrera2020gramses}
{\sc Barrera-Hinojosa, C., and Li, B.}
\newblock Gramses: a new route to general relativistic n-body simulations in
  cosmology. part i. methodology and code description.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2020}, 01 (2020),
  007.

\bibitem{Barrera-Hinojosa:2020gnx}
{\sc Barrera-Hinojosa, C., Li, B., Bruni, M., and He, J.-h.}
\newblock {Vector modes in $\Lambda$CDM: the gravitomagnetic potential in dark
  matter haloes from relativistic $N$-body simulations}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 501}, 4 (2021), 5697--5713.

\bibitem{Barrow:1984zz}
{\sc Barrow, J.~D., and Stein-Schabes, J.}
\newblock {Inhomogeneous cosmologies with cosmological constant}.
\newblock {\em Phys. Lett. A103\/} (1984), 315--317.

\bibitem{Bartelmann_2010}
{\sc Bartelmann, M.}
\newblock Gravitational lensing.
\newblock {\em Classical and Quantum Gravity 27}, 23 (nov 2010), 233001.

\bibitem{Bartolo:2005kv}
{\sc Bartolo, N., Matarrese, S., and Riotto, A.}
\newblock {The full second-order radiation transfer function for large-scale
  cmb anisotropies}.
\newblock {\em JCAP 05\/} (2006), 010.

\bibitem{baumgarte1998numerical}
{\sc Baumgarte, T.~W., and Shapiro, S.~L.}
\newblock Numerical integration of einstein’s field equations.
\newblock {\em Physical Review D 59}, 2 (1998), 024007.

\bibitem{baumgarte2010numerical}
{\sc Baumgarte, T.~W., and Shapiro, S.~L.}
\newblock {\em Numerical relativity}.
\newblock Cambridge University Press, 2010.

\bibitem{Bazanski2}
{\sc {Bażański}, S.~L.}
\newblock {Dynamics of relative motion of test particles in general
  relativity}.
\newblock {\em Annales de L'Institut Henri Poincare Section (A) Physique
  Theorique 27\/} (Sept. 1977), 145--166.

\bibitem{Bazanski1}
{\sc {Bażański}, S.~L.}
\newblock {Kinematics of relative motion of test particles in general
  relativity}.
\newblock {\em Annales de L'Institut Henri Poincare Section (A) Physique
  Theorique 27\/} (Sept. 1977), 115--144.

\bibitem{beasley2002vlba}
{\sc Beasley, A., Gordon, D., Peck, A., Petrov, L., MacMillan, D., Fomalont,
  E., and Ma, C.}
\newblock The vlba calibrator survey—vcs1.
\newblock {\em The Astrophysical Journal Supplement Series 141}, 1 (2002), 13.

\bibitem{PhysRevLett.121.021101}
{\sc Bel, J., and Marinoni, C.}
\newblock Proposal for a real-time detection of our acceleration through space.
\newblock {\em Phys. Rev. Lett. 121\/} (Jul 2018), 021101.

\bibitem{Bentivegna:2016stg}
{\sc Bentivegna, E.}
\newblock {An automatically generated code for relativistic inhomogeneous
  cosmologies}.
\newblock {\em Phys. Rev. D 95}, 4 (2017), 044046.

\bibitem{Bentivegna:2015flc}
{\sc Bentivegna, E., and Bruni, M.}
\newblock {Effects of nonlinear inhomogeneity on the cosmic expansion with
  numerical relativity}.
\newblock {\em Phys. Rev. Lett. 116}, 25 (2016), 251302.

\bibitem{bentivegna2018black}
{\sc Bentivegna, E., Clifton, T., Durk, J., Korzy{\'n}ski, M., and Rosquist,
  K.}
\newblock Black-hole lattices as cosmological models.
\newblock {\em Classical and Quantum Gravity 35}, 17 (2018), 175004.

\bibitem{bentivegna2012evolution}
{\sc Bentivegna, E., and Korzy{\'n}ski, M.}
\newblock Evolution of a periodic eight-black-hole lattice in numerical
  relativity.
\newblock {\em Classical and quantum gravity 29}, 16 (2012), 165007.

\bibitem{bentivegna2013evolution}
{\sc Bentivegna, E., and Korzy{\'n}ski, M.}
\newblock Evolution of a family of expanding cubic black-hole lattices in
  numerical relativity.
\newblock {\em Classical and Quantum Gravity 30}, 23 (2013), 235008.

\bibitem{bertacca2015galaxy}
{\sc Bertacca, D., Bartolo, N., Bruni, M., Koyama, K., Maartens, R., Matarrese,
  S., Sasaki, M., and Wands, D.}
\newblock Galaxy bias and gauges at second order in general relativity.
\newblock {\em Classical and Quantum Gravity 32}, 17 (2015), 175019.

\bibitem{bertacca2014observed}
{\sc Bertacca, D., Maartens, R., and Clarkson, C.}
\newblock Observed galaxy number counts on the lightcone up to second order: I.
  main result.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2014}, 09 (2014),
  037.

\bibitem{Bertschinger:1993xt}
{\sc {Bertschinger}, E.}
\newblock {Cosmological Dynamics}.
\newblock In {\em Cosmology and Large Scale Structure\/} (Jan. 1996),
  R.~{Schaeffer}, J.~{Silk}, M.~{Spiro}, and J.~{Zinn-Justin}, Eds., p.~273.

\bibitem{Beutler:2020evf}
{\sc Beutler, F., and Di~Dio, E.}
\newblock {Modeling relativistic contributions to the halo power spectrum
  dipole}.
\newblock {\em JCAP 07}, 07 (2020), 048.

\bibitem{bolejko2011inhomogeneous}
{\sc Bolejko, K., C{\'e}l{\'e}rier, M.-N., and Krasi{\'n}ski, A.}
\newblock Inhomogeneous cosmological models: exact solutions and their
  applications.
\newblock {\em Classical and Quantum Gravity 28}, 16 (2011), 164002.

\bibitem{bondi1947spherically}
{\sc Bondi, H.}
\newblock Spherically symmetrical models in general relativity.
\newblock {\em Monthly Notices of the Royal Astronomical Society 107}, 5-6
  (1947), 410--425.

\bibitem{bonnor:1977pp}
{\sc Bonnor, W., Sulaiman, A., and Tomimura, N.}
\newblock Szekeres's space-times have no killing vectors.
\newblock {\em General Relativity and Gravitation 8}, 8 (1977), 549--559.

\bibitem{bonvin2011galaxy}
{\sc Bonvin, C., and Durrer, R.}
\newblock What galaxy surveys really measure.
\newblock {\em Physical Review D 84}, 6 (2011), 063505.

\bibitem{Bonvin:2006}
{\sc Bonvin, C., Durrer, R., and Gasparini, M.~A.}
\newblock Fluctuations of the luminosity distance.
\newblock {\em Physical Review D 73}, 2 (Jan 2006).

\bibitem{bruni2014computing}
{\sc Bruni, M., Thomas, D.~B., and Wands, D.}
\newblock Computing general-relativistic effects from newtonian n-body
  simulations: Frame dragging in the post-friedmann approach.
\newblock {\em Physical Review D 89}, 4 (2014), 044010.

\bibitem{Bruni:2013mua}
{\sc Bruni, M., Thomas, D.~B., and Wands, D.}
\newblock {Computing General Relativistic effects from Newtonian N-body
  simulations: Frame dragging in the post-Friedmann approach}.
\newblock {\em Phys. Rev. D 89}, 4 (2014), 044010.

\bibitem{buonanno2007inspiral}
{\sc Buonanno, A., Cook, G.~B., and Pretorius, F.}
\newblock Inspiral, merger, and ring-down of equal-mass black-hole binaries.
\newblock {\em Physical Review D 75}, 12 (2007), 124018.

\bibitem{campanelli2006accurate}
{\sc Campanelli, M., Lousto, C.~O., Marronetti, P., and Zlochower, Y.}
\newblock Accurate evolutions of orbiting black-hole binaries without excision.
\newblock {\em Physical Review Letters 96}, 11 (2006), 111101.

\bibitem{carbone2005unified}
{\sc Carbone, C., and Matarrese, S.}
\newblock Unified treatment of cosmological perturbations from superhorizon to
  small scales.
\newblock {\em Physical Review D 71}, 4 (2005), 043508.

\bibitem{carroll2017book}
{\sc Carroll, B.~W., and Ostlie, D.~A.}
\newblock {\em An introduction to modern astrophysics}.
\newblock Cambridge University Press, 2017.

\bibitem{Catelan:1994ze}
{\sc Catelan, P.}
\newblock {Lagrangian dynamics in nonflat universes and nonlinear gravitational
  evolution}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 276\/} (1995), 115.

\bibitem{Catelan:1994kt}
{\sc Catelan, P., Lucchin, F., Matarrese, S., and Moscardini, L.}
\newblock {Eulerian perturbation theory in nonflat universes: Second order
  approximation}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 276\/} (1995), 39.

\bibitem{celerier1999we}
{\sc Celerier, M.-N.}
\newblock Do we really see a cosmological constant in the supernovae data?
\newblock {\em arXiv preprint astro-ph/9907206\/} (1999).

\bibitem{chaurasia2018gravitational}
{\sc Chaurasia, S.~V., Dietrich, T., Johnson-McDaniel, N.~K., Ujevic, M.,
  Tichy, W., and Br{\"u}gmann, B.}
\newblock Gravitational waves and mass ejecta from binary neutron star mergers:
  Effect of large eccentricities.
\newblock {\em Physical Review D 98}, 10 (2018), 104005.

\bibitem{Sam:2020}
{\sc Christian, S.}
\newblock Re-examining the evidence of the hercules–corona borealis great
  wall.
\newblock {\em Monthly Notices of the Royal Astronomical Society 495}, 4 (May
  2020), 4291–4296.

\bibitem{CiufoliniDemianski}
{\sc Ciufolini, I., and Demiański, M.}
\newblock How to measure the curvature of space-time.
\newblock {\em Phys. Rev. D 34\/} (Aug 1986), 1018--1020.

\bibitem{Clarkson:2016zzi}
{\sc Clarkson, C.}
\newblock {Roulettes: A weak lensing formalism for strong lensing - I.
  Overview}.
\newblock {\em Class. Quant. Grav. 33}, 16 (2016), 16LT01.

\bibitem{Clarkson:2016ccm}
{\sc Clarkson, C.}
\newblock {Roulettes: A weak lensing formalism for strong lensing - II.
  Derivation and analysis}.
\newblock {\em Class. Quant. Grav. 33}, 24 (2016), 245003.

\bibitem{clifton2009archipelagian}
{\sc Clifton, T., and Ferreira, P.~G.}
\newblock Archipelagian cosmology: dynamics and observables in a universe with
  discretized matter content.
\newblock {\em Physical Review D 80}, 10 (2009), 103503.

\bibitem{clifton2015applications}
{\sc Clifton, T., Gregoris, D., and Rosquist, K.}
\newblock Applications of black hole lattices in relativistic cosmology.
\newblock In {\em AIP Conference Proceedings\/} (2015), vol.~1693, AIP
  Publishing LLC, p.~070006.

\bibitem{colless20012df}
{\sc Colless, M., Dalton, G., Maddox, S., Sutherland, W., Norberg, P., Cole,
  S., Bland-Hawthorn, J., Bridges, T., Cannon, R., Collins, C., et~al.}
\newblock The 2df galaxy redshift survey: spectra and redshifts.
\newblock {\em Monthly Notices of the Royal Astronomical Society 328}, 4
  (2001), 1039--1063.

\bibitem{Daverio:2019gql}
{\sc Daverio, D., Dirian, Y., and Mitsou, E.}
\newblock {General relativistic cosmological N-body simulations. Part I. Time
  integration}.
\newblock {\em JCAP 10\/} (2019), 065.

\bibitem{DeWittBrehme}
{\sc DeWitt, B.~S., and Brehme, R.~W.}
\newblock Radiation damping in a gravitational field.
\newblock {\em Annals of Physics 9}, 2 (1960), 220 -- 259.

\bibitem{diDio2012back}
{\sc Di~Dio, E., Vonlanthen, M., and Durrer, R.}
\newblock Back reaction from walls.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2012}, 02 (2012),
  036.

\bibitem{Ding:2009xs}
{\sc Ding, F., and Croft, R. A.~C.}
\newblock {Future dark energy constraints from measurements of quasar parallax:
  Gaia, SIM and beyond}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 397\/} (2009), 1739.

\bibitem{DiDio:2016DlPT}
{\sc Dio, E.~D., Montanari, F., Raccanelli, A., Durrer, R., Kamionkowski, M.,
  and Lesgourgues, J.}
\newblock Curvature constraints from large scale structure.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2016}, 06 (Jun
  2016), 013–013.

\bibitem{Dixon2}
{\sc Dixon, W.~G.}
\newblock Dynamics of extended bodies in general relativity. i. momentum and
  angular momentum.
\newblock {\em Proceedings of the Royal Society of London. A. Mathematical and
  Physical Sciences 314}, 1519 (1970), 499--527.

\bibitem{dodelson2003modern}
{\sc Dodelson, S.}
\newblock {\em Modern cosmology}.
\newblock Elsevier, 2003.

\bibitem{Dyer:1974}
{\sc {Dyer}, C.~C., and {Roeder}, R.~C.}
\newblock {Observations in Locally Inhomogeneous Cosmological Models}.
\newblock {\em apj 189\/} (Apr. 1974), 167--176.

\bibitem{east2018comparing}
{\sc East, W.~E., Wojtak, R., and Abel, T.}
\newblock Comparing fully general relativistic and newtonian calculations of
  structure formation.
\newblock {\em Physical Review D 97}, 4 (2018), 043509.

\bibitem{ehlers-jordan-sachs}
{\sc Ehlers, J., Jordan, P., and Sachs, R.~K.}
\newblock {\em {Beitr\"age zur Theorie der reinen Gravitationsstrahlung}},
  vol.~1 of {\em {Abhandlungen der Mathematisch-Naturwissenschaftlichen
  Klasse}}.
\newblock Verlag der Akademie der Wissenschaften und der Literatur in Mainz,
  Wiesbaden, Germany, 1961.

\bibitem{Einstein:1915gr}
{\sc {Einstein}, A.}
\newblock {Die Feldgleichungen der Gravitation}.
\newblock {\em Sitzungsberichte der K{\"o}niglich Preu{\ss}ischen Akademie der
  Wissenschaften (Berlin\/} (Jan. 1915), 844--847.

\bibitem{einstein1945influence}
{\sc Einstein, A., and Straus, E.~G.}
\newblock The influence of the expansion of space on the gravitation fields
  surrounding the individual stars.
\newblock {\em Reviews of Modern Physics 17}, 2-3 (1945), 120.

\bibitem{ellis2012relativistic}
{\sc Ellis, G.~F., Maartens, R., and MacCallum, M.~A.}
\newblock {\em Relativistic cosmology}.
\newblock Cambridge University Press, 2012.

\bibitem{eppley1977evolution}
{\sc Eppley, K.}
\newblock Evolution of time-symmetric gravitational waves: Initial data and
  apparent horizons.
\newblock {\em Physical Review D 16}, 6 (1977), 1609.

\bibitem{etherington}
{\sc Etherington, I.}
\newblock Lx. on the definition of distance in general relativity.
\newblock {\em The London, Edinburgh, and Dublin Philosophical Magazine and
  Journal of Science 15}, 100 (1933), 761--773.

\bibitem{etherington2}
{\sc Etherington, I. M.~H.}
\newblock Republication of: Lx. on the definition of distance in general
  relativity.
\newblock {\em General Relativity and Gravitation 39}, 7 (Jul 2007),
  1055--1067.

\bibitem{Fanizza:2013GLC}
{\sc Fanizza, G., Gasperini, M., Marozzi, G., and Veneziano, G.}
\newblock An exact jacobi map in the geodesic light-cone gauge.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2013}, 11 (Nov
  2013), 019–019.

\bibitem{Fidler:2017pnb}
{\sc Fidler, C., Tram, T., Rampf, C., Crittenden, R., Koyama, K., and Wands,
  D.}
\newblock {General relativistic weak-field limit and Newtonian N-body
  simulations}.
\newblock {\em JCAP 12\/} (2017), 022.

\bibitem{Flanagan:2018yzh}
{\sc Flanagan, E.~E., Grant, A.~M., Harte, A.~I., and Nichols, D.~A.}
\newblock Persistent gravitational wave observables: General framework.
\newblock {\em Physical Review D 99}, 8 (Apr 2019).

\bibitem{Fleury:2014gha}
{\sc Fleury, P.}
\newblock {Swiss-cheese models and the Dyer-Roeder approximation}.
\newblock {\em JCAP 1406\/} (2014), 054.

\bibitem{Giblin:2015vwq}
{\sc Giblin, J.~T., Mertens, J.~B., and Starkman, G.~D.}
\newblock {Departures from the Friedmann-Lemaitre-Robertston-Walker
  Cosmological Model in an Inhomogeneous Universe: A Numerical Examination}.
\newblock {\em Phys. Rev. Lett. 116}, 25 (2016), 251301.

\bibitem{Giblin:2017ezj}
{\sc Giblin, J.~T., Mertens, J.~B., Starkman, G.~D., and Zentner, A.~R.}
\newblock {General Relativistic Corrections to the Weak Lensing Convergence
  Power Spectrum}.
\newblock {\em Phys. Rev. D 96}, 10 (2017), 103530.

\bibitem{Goldberg:2016lcq}
{\sc Goldberg, S.~R., Clifton, T., and Malik, K.~A.}
\newblock {Cosmology on all scales: a two-parameter perturbation expansion}.
\newblock {\em Phys. Rev. D 95}, 4 (2017), 043503.

\bibitem{Goode:1982pg}
{\sc Goode, S.~W., and Wainwright, J.}
\newblock {Singularities and evolution of the Szekeres cosmological models}.
\newblock {\em Phys. Rev. D26\/} (1982), 3315--3326.

\bibitem{gourgoulhon20123+}
{\sc Gourgoulhon, E.}
\newblock {\em 3+ 1 formalism in general relativity}, vol.~846.
\newblock Springer Science \& Business Media, 2012.

\bibitem{gradshteyn2014table}
{\sc Gradshteyn, I.~S., and Ryzhik, I.~M.}
\newblock {\em Table of integrals, series, and products}.
\newblock Academic press, 2014.

\bibitem{Grasso:2018mei}
{\sc Grasso, M., Korzy\'nski, M., and Serbenta, J.}
\newblock {Geometric optics in general relativity using bilocal operators}.
\newblock {\em Phys. Rev. D 99}, 6 (2019), 064038.

\bibitem{Grasso:2021iwq}
{\sc Grasso, M., and Villa, E.}
\newblock {BiGONLight: light propagation with bilocal operators in numerical
  relativity}.
\newblock {\em Class. Quant. Grav. 39}, 1 (2022), 015011.

\bibitem{Grasso:2021zra}
{\sc Grasso, M., Villa, E., Korzy\'nski, M., and Matarrese, S.}
\newblock {Isolating nonlinearities of light propagation in inhomogeneous
  cosmologies}.
\newblock {\em Phys. Rev. D 104}, 4 (2021), 043508.

\bibitem{green2011new}
{\sc Green, S.~R., and Wald, R.~M.}
\newblock New framework for analyzing the effects of small scale
  inhomogeneities in cosmology.
\newblock {\em Physical Review D 83}, 8 (2011), 084020.

\bibitem{green2012newtonian}
{\sc Green, S.~R., and Wald, R.~M.}
\newblock Newtonian and relativistic cosmologies.
\newblock {\em Physical Review D 85}, 6 (2012), 063512.

\bibitem{Gressel:2019jxw}
{\sc Gressel, H.~A., Bonvin, C., Bruni, M., and Bacon, D.}
\newblock {Full-sky weak lensing: a nonlinear post-Friedmann treatment}.
\newblock {\em JCAP 05\/} (2019), 045.

\bibitem{hahn1964two}
{\sc Hahn, S.~G., and Lindquist, R.~W.}
\newblock The two-body problem in geometrodynamics.
\newblock {\em Annals of Physics 29}, 2 (1964), 304--331.

\bibitem{Harte:2018wni}
{\sc Harte, A.~I.}
\newblock {Gravitational lensing beyond geometric optics: I. Formalism and
  observables}.
\newblock {\em Gen. Rel. Grav. 51}, 1 (2019), 14.

\bibitem{Hellaby:2017soj}
{\sc Hellaby, C., and Walters, A.}
\newblock {Calculating observables in inhomogeneous cosmologies. Part I:
  general framework}.
\newblock {\em JCAP 1802}, 02 (2018), 015.

\bibitem{hinder2018eccentric}
{\sc Hinder, I., Kidder, L.~E., and Pfeiffer, H.~P.}
\newblock Eccentric binary black hole inspiral-merger-ringdown gravitational
  waveform model from numerical relativity and post-newtonian theory.
\newblock {\em Physical Review D 98}, 4 (2018), 044015.

\bibitem{Hobbs:2019arz}
{\sc Hobbs, D., et~al.}
\newblock {All-sky visible and near infrared space astrometry}.
\newblock {\em Exper. Astron. 51}, 3 (2021), 783--843.

\bibitem{howlett2012cmb}
{\sc Howlett, C., Lewis, A., Hall, A., and Challinor, A.}
\newblock Cmb power spectrum parameter degeneracies in the era of precision
  cosmology.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2012}, 04 (2012),
  027.

\bibitem{hubble1988relation}
{\sc Hubble, E.}
\newblock A relation between distance and radial velocity among extra-galactic
  nebulae.
\newblock {\em The Early Universe: Reprints\/} (1988), 9.

\bibitem{PhysRev.166.1263}
{\sc Isaacson, R.~A.}
\newblock Gravitational radiation in the limit of high frequency. i. the linear
  approximation and geometrical optics.
\newblock {\em Phys. Rev. 166\/} (Feb 1968), 1263--1271.

\bibitem{PhysRev.166.1272}
{\sc Isaacson, R.~A.}
\newblock Gravitational radiation in the limit of high frequency. ii. nonlinear
  terms and the effective stress tensor.
\newblock {\em Phys. Rev. 166\/} (Feb 1968), 1272--1280.

\bibitem{jones2017precision}
{\sc Jones, B.~J.}
\newblock {\em Precision cosmology: the first half million years}.
\newblock Cambridge University Press, 2017.

\bibitem{kasai}
{\sc Kasai, M.}
\newblock The triangulation in a perturbed friedmann universe.
\newblock {\em Prog. Theor. Phys. 79\/} (1988), 777.

\bibitem{kermack_mccrea_whittaker_1934}
{\sc Kermack, W.~O., McCrea, W.~H., and Whittaker, E.~T.}
\newblock Iv.—on properties of null geodesics, and their application to the
  theory of radiation.
\newblock {\em Proceedings of the Royal Society of Edinburgh 53\/} (1934),
  31–47.

\bibitem{kodama1984cosmological}
{\sc Kodama, H., and Sasaki, M.}
\newblock Cosmological perturbation theory.
\newblock {\em Progress of Theoretical Physics Supplement 78\/} (1984), 1--166.

\bibitem{WMAP:2008lyn}
{\sc Komatsu, E., et~al.}
\newblock {Five-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations:
  Cosmological Interpretation}.
\newblock {\em Astrophys. J. Suppl. 180\/} (2009), 330--376.

\bibitem{kopp2014newton}
{\sc Kopp, M., Uhlemann, C., and Haugg, T.}
\newblock Newton to einstein—dust to dust.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2014}, 03 (2014),
  018.

\bibitem{Korzynski:2019oal}
{\sc Korzy\'nski, M., and Villa, E.}
\newblock {Geometric optics in relativistic cosmology: new formulation and a
  new observable}.
\newblock {\em Phys. Rev. D 101}, 6 (2020), 063506.

\bibitem{Korzynski:2018}
{\sc Korzyński, M., and Kopiński, J.}
\newblock Optical drift effects in general relativity.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2018}, 03 (2018),
  012.

\bibitem{krasinski2012drift}
{\sc Krasinski, A., and Bolejko, K.}
\newblock Drift of light rays induced by nonsymmetric cosmic flow: an
  observational test of homogeneity of the universe+ a few general comments on
  inhomogeneous models.
\newblock {\em arXiv preprint arXiv:1212.4697\/} (2012).

\bibitem{lemaitre1927univers}
{\sc Lema{\^\i}tre, G.}
\newblock Un univers homog{\`e}ne de masse constante et de rayon croissant
  rendant compte de la vitesse radiale des n{\'e}buleuses extra-galactiques.
\newblock In {\em Annales de la Soci{\'e}t{\'e} scientifique de Bruxelles\/}
  (1927), vol.~47, pp.~49--59.

\bibitem{lemaitre1933univers}
{\sc Lema{\^\i}tre, G.}
\newblock L'univers en expansion.
\newblock In {\em Annales de la Soci{\'e}t{\'e} scientifique de Bruxelles\/}
  (1933), vol.~53, p.~51.

\bibitem{Lepori:2020ifz}
{\sc Lepori, F., Adamek, J., Durrer, R., Clarkson, C., and Coates, L.}
\newblock {Weak-lensing observables in relativistic N-body simulations}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 497}, 2 (2020), 2078--2095.

\bibitem{linquist1957dynamics}
{\sc Linquist, R., and Wheeler, J.}
\newblock Dynamics of a lattice universe by the schwarzschild-cell methods.
\newblock {\em Rev. Mod. Phys 29\/} (1957), 432.

\bibitem{loeb}
{\sc Loeb, A.}
\newblock {Direct Measurement of Cosmological Parameters from the Cosmic
  Deceleration of Extragalactic Objects}.
\newblock {\em Astrophys. J. 499\/} (1998), L111--L114.

\bibitem{loffler2012einstein}
{\sc L{\"o}ffler, F., Faber, J., Bentivegna, E., Bode, T., Diener, P., Haas,
  R., Hinder, I., Mundim, B.~C., Ott, C.~D., Schnetter, E., et~al.}
\newblock The einstein toolkit: a community computational infrastructure for
  relativistic astrophysics.
\newblock {\em Classical and Quantum Gravity 29}, 11 (2012), 115001.

\bibitem{KiDS:2021opn}
{\sc Loureiro, A., et~al.}
\newblock {KiDS \& Euclid: Cosmological implications of a pseudo angular power
  spectrum analysis of KiDS-1000 cosmic shear tomography}.
\newblock {\em arXiv\/} (10 2021).

\bibitem{low}
{\sc {Low}, R.~J.}
\newblock {Celestial spheres, light cones, and cuts.}
\newblock {\em Journal of Mathematical Physics 34\/} (Jan. 1993), 315--319.

\bibitem{gaiadr2-parallaxes}
{\sc {Luri, X.}, {Brown, A. G. A.}, {Sarro, L. M.}, {Arenou, F.},
  {Bailer-Jones, C. A. L.}, {Castro-Ginard, A.}, {Bruijne, J. de}, {Prusti,
  T.}, {Babusiaux, C.}, and {Delgado, H. E.}}
\newblock Gaia data release 2 - using gaia parallaxes.
\newblock {\em A\&A 616\/} (2018), A9.

\bibitem{Macpherson:2021gbh}
{\sc Macpherson, H.~J., and Heinesen, A.}
\newblock Luminosity distance and anisotropic sky-sampling at low redshifts: A
  numerical relativity study.
\newblock {\em Physical Review D 104}, 2 (Jul 2021).

\bibitem{macpherson2017}
{\sc Macpherson, H.~J., Lasky, P.~D., and Price, D.~J.}
\newblock Inhomogeneous cosmology with numerical relativity.
\newblock {\em Physical Review D 95}, 6 (2017), 064028.

\bibitem{Macpherson:2018akp}
{\sc Macpherson, H.~J., Lasky, P.~D., and Price, D.~J.}
\newblock {The trouble with Hubble: Local versus global expansion rates in
  inhomogeneous cosmological simulations with numerical relativity}.
\newblock {\em Astrophys. J. 865}, 1 (2018), L4.

\bibitem{Marcori:2018cwn}
{\sc Marcori, O.~H., Pitrou, C., Uzan, J.-P., and Pereira, T.~S.}
\newblock {Direction and redshift drifts for general observers and their
  applications in cosmology}.
\newblock {\em Phys. Rev. D98}, 2 (2018), 023517.

\bibitem{matarrese1998relativistic}
{\sc Matarrese, S., Mollerach, S., and Bruni, M.}
\newblock Relativistic second-order perturbations of the einstein--de sitter
  universe.
\newblock {\em Physical Review D 58}, 4 (1998), 043504.

\bibitem{mater}
{\sc Matarrese, S., and Terranova, D.}
\newblock Post-newtonian cosmological dynamics in lagrangian coordinates.
\newblock {\em Mon. Not. R. Astron. Soc. 283\/} (1996), 400--418.
\newblock astro-ph/9511093.

\bibitem{mccracken2003virmos}
{\sc McCracken, H., Radovich, M., Bertin, E., Mellier, Y., Dantel-Fort, M.,
  Le~Fevre, O., Cuillandre, J., Gwyn, S., Foucaud, S., and Zamorani, G.}
\newblock The virmos deep imaging survey-ii: Cfh12k bvri optical data for the
  0226-04 deep field.
\newblock {\em Astronomy \& Astrophysics 410}, 1 (2003), 17--32.

\bibitem{mccrea}
{\sc McCrea, W.~H.}
\newblock Observable relations in relativistic cosmology.
\newblock {\em Zeitschrift für Astrophysik 9\/} (1935), 290.

\bibitem{Mertens:2015ttp}
{\sc Mertens, J.~B., Giblin, J.~T., and Starkman, G.~D.}
\newblock {Integration of inhomogeneous cosmological spacetimes in the BSSN
  formalism}.
\newblock {\em Phys. Rev. D93}, 12 (2016), 124059.

\bibitem{Meures:2011ke}
{\sc Meures, N., and Bruni, M.}
\newblock Exact nonlinear inhomogeneities in $\lambda$ cdm cosmology.
\newblock {\em Physical Review D 83}, 12 (2011), 123519.

\bibitem{Meures:2011gp}
{\sc Meures, N., and Bruni, M.}
\newblock {Redshift and distances in a $\Lambda$CDM cosmology with non-linear
  inhomogeneities}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 419\/} (2012), 1937.

\bibitem{Milillo:2015cva}
{\sc Milillo, I., Bertacca, D., Bruni, M., and Maselli, A.}
\newblock {Missing link: A nonlinear post-Friedmann framework for small and
  large scales}.
\newblock {\em Phys. Rev. D 92}, 2 (2015), 023519.

\bibitem{mtw}
{\sc Misner, C.~W., Thorne, K.~S., and Wheeler, J.~A.}
\newblock {\em Gravitation}.
\newblock W. H. Freeman and Company, New York, 1973.

\bibitem{vogelsberger2014introducing}
{\sc Nelson, D., Pillepich, A., Genel, S., Vogelsberger, M., Springel, V.,
  Torrey, P., Rodriguez-Gomez, V., Sijacki, D., Snyder, G., Griffen, B., and
  et~al.}
\newblock The illustris simulation: Public data release.
\newblock {\em Astronomy and Computing 13\/} (Nov 2015), 12–37.

\bibitem{nelson2021illustristng}
{\sc Nelson, D., Springel, V., Pillepich, A., Rodriguez-Gomez, V., Torrey, P.,
  Genel, S., Vogelsberger, M., Pakmor, R., Marinacci, F., Weinberger, R.,
  Kelley, L., Lovell, M., Diemer, B., and Hernquist, L.}
\newblock The illustristng simulations: Public data release, 2021.

\bibitem{peebles1970structure}
{\sc Peebles, P.}
\newblock Structure of the coma cluster of galaxies.
\newblock {\em The Astronomical Journal 75\/} (1970), 13.

\bibitem{peebles1993principles}
{\sc Peebles, P. J.~E., and Peebles, P.~J.}
\newblock {\em Principles of physical cosmology}.
\newblock Princeton university press, 1993.

\bibitem{Penzias:1965}
{\sc {Penzias}, A.~A., and {Wilson}, R.~W.}
\newblock {A Measurement of Excess Antenna Temperature at 4080 Mc/s.}
\newblock {\em apj 142\/} (July 1965), 419--421.

\bibitem{perlick}
{\sc Perlick, V.}
\newblock On redshift and parallaxes in general relativistic kinematical world
  models.
\newblock {\em Journal of Mathematical Physics 31}, 8 (1990), 1962--1971.

\bibitem{perlick-lrr}
{\sc Perlick, V.}
\newblock Gravitational lensing from a spacetime perspective.
\newblock {\em Living Reviews in Relativity 7}, 1 (Sep 2004), 9.

\bibitem{Perlmutter_1999}
{\sc Perlmutter, S., Aldering, G., Goldhaber, G., Knop, R.~A., Nugent, P.,
  Castro, P.~G., Deustua, S., Fabbro, S., Goobar, A., Groom, D.~E., and et~al.}
\newblock Measurements of omega and lambda from 42 high‐redshift supernovae.
\newblock {\em The Astrophysical Journal 517}, 2 (Jun 1999), 565–586.

\bibitem{2001A&A...369..339P}
{\sc {Perryman}, M.~A.~C., {de Boer}, K.~S., {Gilmore}, G., {H{\o}g}, E.,
  {Lattanzi}, M.~G., {Lindegren}, L., {Luri}, X., {Mignard}, F., {Pace}, O.,
  and {de Zeeuw}, P.~T.}
\newblock {GAIA: Composition, formation and evolution of the Galaxy}.
\newblock {\em Astronomy and Astrophysics 369\/} (Apr. 2001), 339--363.

\bibitem{pirani}
{\sc Pirani, F. A.~E.}
\newblock {On the Physical significance of the Riemann tensor}.
\newblock {\em Acta Phys. Polon. 15\/} (1956), 389--405.

\bibitem{Poisson2011}
{\sc Poisson, E., Pound, A., and Vega, I.}
\newblock The motion of point particles in curved spacetime.
\newblock {\em Living Reviews in Relativity 14}, 1 (Sep 2011), 7.

\bibitem{Pretorius:2005gq}
{\sc Pretorius, F.}
\newblock {Evolution of binary black hole spacetimes}.
\newblock {\em Phys. Rev. Lett. 95\/} (2005), 121101.

\bibitem{Puetzfeld:2015uxi}
{\sc Puetzfeld, D., and Obukhov, Y.~N.}
\newblock {Generalized deviation equation and determination of the curvature in
  General Relativity}.
\newblock {\em Phys. Rev. D93}, 4 (2016), 044073.

\bibitem{Quartin:2009xr}
{\sc Quartin, M., and Amendola, L.}
\newblock {Distinguishing Between Void Models and Dark Energy with Cosmic
  Parallax and Redshift Drift}.
\newblock {\em Phys. Rev. D81\/} (2010), 043522.

\bibitem{Quercellini:2010zr}
{\sc Quercellini, C., Amendola, L., Balbi, A., Cabella, P., and Quartin, M.}
\newblock {Real-time Cosmology}.
\newblock {\em Phys. Rept. 521\/} (2012), 95--134.

\bibitem{Quercellini:2009ni}
{\sc Quercellini, C., Cabella, P., Amendola, L., Quartin, M., and Balbi, A.}
\newblock {Cosmic Parallax as a probe of late time anisotropic expansion}.
\newblock {\em Phys. Rev. D80\/} (2009), 063527.

\bibitem{Quercellini:2008ty}
{\sc Quercellini, C., Quartin, M., and Amendola, L.}
\newblock {Possibility of Detecting Anisotropic Expansion of the Universe by
  Very Accurate Astrometry Measurements}.
\newblock {\em Phys. Rev. Lett. 102\/} (2009), 151302.

\bibitem{Rampf:2016wom}
{\sc Rampf, C., Villa, E., Bertacca, D., and Bruni, M.}
\newblock {Lagrangian theory for cosmic structure formation with vorticity:
  Newtonian and post-Friedmann approximations}.
\newblock {\em Phys. Rev. D 94}, 8 (2016), 083515.

\bibitem{rasanen}
{\sc R\"{a}s\"{a}nen, S.}
\newblock A covariant treatment of cosmic parallax.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2014}, 03 (2014),
  035.

\bibitem{Riess:2014uga}
{\sc Riess, A.~G., Casertano, S., Anderson, J., Mackenty, J., and Filippenko,
  A.~V.}
\newblock {Parallax Beyond a Kiloparsec from Spatially Scanning the Wide Field
  Camera 3 on the Hubble Space Telescope}.
\newblock {\em Astrophys. J. 785\/} (2014), 161.

\bibitem{Riess:2018uxu}
{\sc Riess, A.~G., et~al.}
\newblock {New Parallaxes of Galactic Cepheids from Spatially Scanning the
  Hubble Space Telescope: Implications for the Hubble Constant}.
\newblock {\em Astrophys. J. 855}, 2 (2018), 136.

\bibitem{Riess:1998}
{\sc Riess, A.~G., Filippenko, A.~V., Challis, P., Clocchiatti, A., Diercks,
  A., Garnavich, P.~M., Gilliland, R.~L., Hogan, C.~J., Jha, S., Kirshner,
  R.~P., and et~al.}
\newblock Observational evidence from supernovae for an accelerating universe
  and a cosmological constant.
\newblock {\em The Astronomical Journal 116}, 3 (Sep 1998), 1009–1038.

\bibitem{rosquist}
{\sc Rosquist, K.}
\newblock Trigonometric parallaxes of distant objects — what they could tell
  about the universe.
\newblock {\em Astrophys. J. 331\/} (1988), 648.

\bibitem{Ruan:2021rqv}
{\sc Ruan, C.-Z., Cuesta-Lazaro, C., Eggemeier, A., Hern\'andez-Aguayo, C.,
  Baugh, C.~M., Li, B., and Prada, F.}
\newblock {Towards an accurate model of small-scale redshift-space distortions
  in modified gravity}.
\newblock {\em arXiv\/} (10 2021).

\bibitem{sachs}
{\sc {Sachs}, R.}
\newblock {Gravitational Waves in General Relativity. VI. The Outgoing
  Radiation Condition}.
\newblock {\em Proceedings of the Royal Society of London Series A 264\/} (Nov.
  1961), 309--338.

\bibitem{sandage}
{\sc {Sandage}, A.}
\newblock {The Change of Redshift and Apparent Luminosity of Galaxies due to
  the Deceleration of Selected Expanding Universes.}
\newblock {\em Astrophys. J. 136\/} (Sept. 1962), 319.

\bibitem{Sanghai:2017yyn}
{\sc Sanghai, V. A.~A., Fleury, P., and Clifton, T.}
\newblock {Ray tracing and Hubble diagrams in post-Newtonian cosmology}.
\newblock {\em JCAP 07\/} (2017), 028.

\bibitem{Euclid:2021icp}
{\sc Scaramella, R., et~al.}
\newblock {Euclid preparation: I. The Euclid Wide Survey}.
\newblock {\em arXiv\/} (8 2021).

\bibitem{Scrimgeour:2012wt}
{\sc Scrimgeour, M., et~al.}
\newblock {The WiggleZ Dark Energy Survey: the transition to large-scale cosmic
  homogeneity}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 425\/} (2012), 116--134.

\bibitem{Julius-spherical}
{\sc Serbenta, J., and Korzy\'nski, M.}
\newblock Bilocal geodesic operators in spherically-symmetric spacetimes.
\newblock {\em in preparation\/} (2021).

\bibitem{Julius}
{\sc Serbenta, J., and Korzy\'nski, M.}
\newblock Redshift drift in general relativity in the bi-local formulation of
  geometrical optics.
\newblock {\em in preparation\/} (\noop{3001}).

\bibitem{shibata1995post}
{\sc Shibata, M., and Asada, H.}
\newblock Post-newtonian equations of motion in the flat universe.
\newblock {\em Progress of Theoretical Physics 94}, 1 (1995), 11--31.

\bibitem{shibata1995evolution}
{\sc Shibata, M., and Nakamura, T.}
\newblock Evolution of three-dimensional gravitational waves: Harmonic slicing
  case.
\newblock {\em Physical Review D 52}, 10 (1995), 5428.

\bibitem{Smarr:1977uf}
{\sc Smarr, L., and York, Jr., J.~W.}
\newblock {Kinematical conditions in the construction of space-time}.
\newblock {\em Phys. Rev. D 17\/} (1978), 2529--2551.

\bibitem{COBE:1992syq}
{\sc Smoot, G.~F., et~al.}
\newblock {Structure in the COBE differential microwave radiometer first year
  maps}.
\newblock {\em Astrophys. J. Lett. 396\/} (1992), L1--L5.

\bibitem{Stafford:2021uvk}
{\sc Stafford, S.~G., McCarthy, I.~G., Kwan, J., Brown, S.~T., Font, A.~S., and
  Robertson, A.}
\newblock {Testing extensions to LCDM on small scales with forthcoming cosmic
  shear surveys}.
\newblock {\em arXiv\/} (9 2021).

\bibitem{SyngeBook}
{\sc {Synge}, J.~L.}
\newblock {\em {Relativity: The general theory}}.
\newblock North-Holland Publishing Company, Amsterdam, 1960.

\bibitem{szekeres}
{\sc Szekeres, P.}
\newblock The gravitational compass.
\newblock {\em Journal of Mathematical Physics 6}, 9 (1965), 1387--1391.

\bibitem{Szekeres:1974ct}
{\sc Szekeres, P.}
\newblock {A Class of Inhomogeneous Cosmological Models}.
\newblock {\em Commun. Math. Phys. 41\/} (1975), 55.

\bibitem{thomas2015fully}
{\sc Thomas, D.~B., Bruni, M., and Wands, D.}
\newblock The fully non-linear post-friedmann frame-dragging vector potential:
  Magnitude and time evolution from n-body simulations.
\newblock {\em Monthly Notices of the Royal Astronomical Society 452}, 2
  (2015), 1727--1742.

\bibitem{Thomas:2014aga}
{\sc Thomas, D.~B., Bruni, M., and Wands, D.}
\newblock {Relativistic weak lensing from a fully non-linear cosmological
  density field}.
\newblock {\em JCAP 09\/} (2015), 021.

\bibitem{tolman1934effect}
{\sc Tolman, R.~C.}
\newblock Effect of inhomogeneity on cosmological models.
\newblock {\em Proceedings of the national academy of sciences of the United
  States of America 20}, 3 (1934), 169.

\bibitem{tomita1988post}
{\sc Tomita, K.}
\newblock Post-newtonian equations of motion in an expanding universe.
\newblock {\em Progress of theoretical physics 79}, 2 (1988), 258--262.

\bibitem{tsujikawa2003introductory}
{\sc Tsujikawa, S.}
\newblock Introductory review of cosmic inflation.
\newblock {\em arXiv preprint hep-ph/0304257\/} (2003).

\bibitem{Umeh:2012pn}
{\sc Umeh, O., Clarkson, C., and Maartens, R.}
\newblock {Nonlinear relativistic corrections to cosmological distances,
  redshift and gravitational lensing magnification: I. Key results}.
\newblock {\em Class. Quant. Grav. 31\/} (2014), 202001.

\bibitem{Uzun:2018yes}
{\sc Uzun, N.}
\newblock {Reduced phase space optics for general relativity: Symplectic ray
  bundle transfer}.
\newblock {\em Class. Quant. Grav. 37}, 4 (2020), 045002.

\bibitem{Villa:2011vt}
{\sc Villa, E., Matarrese, S., and Maino, D.}
\newblock Post-newtonian cosmological dynamics of plane-parallel perturbations
  and back-reaction.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2011}, 08 (2011),
  024.

\bibitem{Villa:2015ppa}
{\sc Villa, E., and Rampf, C.}
\newblock Relativistic perturbations in $\lambda$cdm: Eulerian \& lagrangian
  approaches.
\newblock {\em Journal of Cosmology and Astroparticle Physics 2016}, 01 (2016),
  030.

\bibitem{Vincent:2012kn}
{\sc Vincent, F.~H., Gourgoulhon, E., and Novak, J.}
\newblock {3+1 geodesic equation and images in numerical spacetimes}.
\newblock {\em Class. Quant. Grav. 29\/} (2012), 245005.

\bibitem{Vines:2014oba}
{\sc Vines, J.}
\newblock {Geodesic deviation at higher orders via covariant bitensors}.
\newblock {\em Gen. Rel. Grav. 47}, 5 (2015), 59.

\bibitem{vogt2005deep}
{\sc Vogt, N.~P., Koo, D.~C., Phillips, A.~C., Wu, K., Faber, S., Willmer,
  C.~N., Simard, L., Weiner, B.~J., Illingworth, G.~D., Gebhardt, K., et~al.}
\newblock The deep groth strip survey. i. the sample.
\newblock {\em The Astrophysical Journal Supplement Series 159}, 1 (2005), 41.

\bibitem{wald2010general}
{\sc Wald, R.~M.}
\newblock {\em General relativity}.
\newblock University of Chicago press, 2010.

\bibitem{weinberg-letter}
{\sc Weinberg, S.}
\newblock Direct determination of the metric from observed redshifts and
  distances.
\newblock {\em The Astrophisical Journal 161\/} (1970), L233--L234.

\bibitem{Yadav:2010cc}
{\sc Yadav, J.~K., Bagla, J.~S., and Khandai, N.}
\newblock {Fractal Dimension as a measure of the scale of Homogeneity}.
\newblock {\em Mon. Not. Roy. Astron. Soc. 405\/} (2010), 2009.

\bibitem{york2000sloan}
{\sc York, D.~G., Adelman, J., Anderson~Jr, J.~E., Anderson, S.~F., Annis, J.,
  Bahcall, N.~A., Bakken, J., Barkhouser, R., Bastian, S., Berman, E., et~al.}
\newblock The sloan digital sky survey: Technical summary.
\newblock {\em The Astronomical Journal 120}, 3 (2000), 1579.

\end{thebibliography}


==> template/App_comparison.tex <==


\chapter{The wall universe and the Szekeres model}
\MG{from non-linearities}
\label{par:crfSzekeres}

In this section we compare the Szekeres spacetime with the plane-parallel case considered in this work. \MG{USED IN CHAP1: CHANGE HERE! In his original paper \cite{Szekeres:1974ct}, Szekeres studied all the solutions to the Einstein field equation with irrational dust for line elements having the form
\begin{equation}
ds_{\rm Sz}^2=-d t^2 + e^{2 \alpha(t,q_{\rm 1},q_{\rm 2},q_{\rm 3})} dq_{\rm 1}^2 + e^{2 \beta(t,q_{\rm 1},q_{\rm 2},q_{\rm 3})} (dq_{\rm 2}^2+ dq_{\rm 3}^2)
\label{eq:Old_Szekeres_metric}
\end{equation}
Two different classes of solutions can be distinguished: class-\textsc{I} solutions are a generalization of the  Lema\^{i}tre-Bondi-Tolman model while class-\textsc{II} solutions are a generalization of Kantowski-Sachs and FLRW model. 
Subsequently, Barrow and Stein-Schabes \cite{Barrow:1984zz} generalized the Szekeres solutions by adding a cosmological constant $\Lambda$ to the dust. 
More recently, Bruni and Meures \cite{Meures:2011ke} presented a new formulation of the class-\textsc{II} Szekeres solutions in which the separation between inhomogeneities and the FLRW background is explicitly provided and thus the spacetime metric is presented in a more convenient form for cosmological applications. We compare our plane-parallel metric with their formulation. We begin by summarizing the results presented in \cite{Meures:2011ke}.

The authors focused their analysis on the Szekeres solutions which admit a flat FLRW background and such that the line element\footnote{We choose here to use  our notation instead that of that of  \cite{Meures:2011ke}. The line element (\ref{eq:Szekeres_metric}) is different from the one presented in \cite{Meures:2011ke} since we use conformal time and we have chosen a different axis of symmetry. Of course this does not affect any results, since it is easy to show that the two metrics are equivalent under a coordinate transformation.} can be written as
\begin{equation}
ds_{\rm Sz}^2=a^2 \left( -d \eta^2 + \gamma^{\rm{Sz}}_{\rm 11} dq_{\rm 1}^2 + \gamma^{\rm{Sz}}_{\rm 22} dq_{\rm 2}^2+ \gamma^{\rm{Sz}}_{\rm 33}dq_{\rm 3}^2 \right)
\end{equation}
where
\begin{equation} \label{eq:Szekeres_metric}
\begin{split}
\gamma^{\rm{Sz}}_{\rm 11} =& X^2(\eta,q_{\rm 1},q_{\rm 2},q_{\rm 3}) \\
\gamma^{\rm{Sz}}_{\rm 22}= & 1\\
\gamma^{\rm{Sz}}_{\rm 33}=& 1.
 \end{split}
\end{equation}
As it is shown in \cite{Meures:2011ke}, thanks to the symmetry of the problem, the function $X(\eta,q_{\rm 1},q_{\rm 2},q_{\rm 3})$ can be decomposed as 
\begin{equation}\label{eq:sz_X}
X(\eta,q_{\rm 1},q_{\rm 2},q_{\rm 3})=F(\eta,q_{\rm 1})+A(q_{\rm 1},q_{\rm 2},q_{\rm 3})\,,
\end{equation}
where the function $F(\eta, q_{\rm 1})$ satisfies the Newtonian evolution equation for the first-order density contrast\footnote{This was shown implicitly in Sec.~$5$ of the Szekeres' original paper \cite{Szekeres:1974ct} and subsequently by many other authors as those of \cite{bonnor:1977pp}. However, it was Goode and Wainwright who recognized explicitly that the relativistic equations for the density fluctuations in Szekeres model are the same as in Newtonian gravity, \cite{Goode:1982pg}. They also provide a new formulation of the Szekeres solutions, much more useful in cosmology, in which the relationship with the FLRW solution is clarified.}
\begin{equation} \label{eqforF}
\ddot{F} +\mathcal{H}\dot{F}-\frac{3}{2}\mathcal{H}_0^2\Omega_{m_0}\frac{F}{a}=0\,,
\end{equation}
which admits two linearly independent solutions, the growing and decaying modes, as is well known. Then $F(\eta, q_{\rm 1})$ coincides with the linear density contrast and more precisely we have $F(\eta, q_{\rm 1})= -\delta_{\rm Lin}(\eta, q_{\rm 1})$ \footnote{The minus sign between $F$ and $\delta$ follows from the fact that in eq. ($A8$) of \cite{Meures:2011ke} the authors set, in full generality,  $\delta_{in}=-\frac{F_{in}}{F_{in}+A}$.}. Neglecting the decaying modes it is possible, without loss of generality, to factorize $F(\eta, q_{\rm 1})$ as\footnote{The time-dependent-only growing mode is denoted by $f_+$ in \cite{Meures:2011ke} and it is given in a dimensionless time variable $\tau$ in Eq.~(11b). To match $\cal D$ in \eqref{eq:growth_fact} and  $f_+$ one needs to: first transform $f_+(\tau)$ to conformal time $f_{+}(\eta)$ and then normalise such that $f_{+}(\eta_{\rm 0})=1$. The final result is $F(\eta, q_{\rm 1})$ as in \eqref{eq:F_Sz}.}
\begin{equation}
\label{eq:F_Sz}
F(\eta, q_{\rm 1})= {\cal D}(\eta) \beta_+(q_{\rm 1})\, ,
\end{equation}
where $\mathcal{D}$ is the growing mode solution for the density contrast given by (see e.g. Eq.~($5.13$) in \cite{Villa:2015ppa}, where we have already normalized in order to have $\mathcal{D}_0=1$)
\begin{equation}
\mathcal{D} (\eta) = \frac{a}{\frac{5}{2}\Omega_{\rm{m 0}} } \sqrt{1+\frac{\Omega_{\rm{\Lambda 0}}}{\Omega_{\rm{m 0}}}a^3}\,  {}_2 F_{1} \left( \frac{3}{2}, \frac{5}{6}, \frac{11}{6}, -\frac{\Omega_{\rm{\Lambda 0}}}{\Omega_{\rm{m 0}}}a^3 \right)\,,
\label{eq:growth_fact}
\end{equation}
with ${}_2 F_{1} \left(a,b,c, x\right)$ being the Gaussian (or ordinary) hypergeometric function. }

On the other hand, our Newtonian plane-parallel metric is given by:
\begin{equation} \label{eq:app_metricNWT}
\begin{split}
\gamma^{\rm{N}}_{11} =& \left(1-\frac{2}{3}\frac{ \mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{ \stuff} \right)^2 \\
\gamma^{\rm{N}}_{22}= & 1\\
\gamma^{\rm{N}}_{33}=& 1.
 \end{split}
\end{equation}

We now investigate the link between \eqref{eq:app_metricNWT} and \eqref{eq:Szekeres_metric} by comparing the two forms of $\gamma_{\rm 11}$ and referring to Eqs.~\eqref{eq:sz_X} and \eqref{eq:F_Sz}. Let us start from~\eqref{eq:F_Sz}: to fix the time-independent function $\beta_{\rm +}(q_{\rm 1})$, one can take advantage from the fact that $\delta_{\rm Lin}(\eta, q_{\rm 1})=-{\cal D}(\eta) \beta_+(q_{\rm 1})$ and use the cosmological Poisson equation \eqref{eq:Poisson_eq} to find
\begin{equation}
\beta_+(q_{\rm 1}) = - \frac{2}{3}\frac{\partial_{\rm q_{\rm 1}}^2 \phi_{\rm 0}(q_{\rm 1})}{\stuff}\, .
\label{eq:beta+}
\end{equation}
At this point we have completely fixed $F(\eta, q_{\rm 1})$. Now, by looking at Eq.~\eqref{eq:sz_X} it is straightforward to conclude that the two metrics \eqref{eq:app_metricNWT} and \eqref{eq:Szekeres_metric} are fully equivalent if $A(q_{\rm 1},q_{\rm 2},q_{\rm 3})= 1$\footnote{To be more precise it would be enough to neglect the dependence on $(q_{\rm 2}, q_{\rm 3})$  in~\eqref{eq:sz_X} by imposing that $A(q_{\rm 1},q_{\rm 2},q_{\rm 3})\equiv A(q_{\rm 1})$, i.e. $$X(\eta, q_{\rm 1})= A(q_{\rm 1})+F(\eta, q_{\rm 1})\, .$$ 
However, if this were the case, it is easy to show that performing the coordinate transformation $\tilde{q_{\rm 1}}=\int A(q_{\rm 1}) d q_{\rm 1}$ and rescaling $\tilde{F}(\eta, \tilde{q}_{\rm 1})=\frac{F(\eta, q_{\rm 1})}{A(q_{\rm 1})}$, we obtain again $X(\eta, \tilde{q}_{\rm 1})= 1 + \tilde{F}(\eta, \tilde{q}_{\rm 1})$. }.
However, this cannot be the case, as we will now show. Let us start by noticing that planar symmetry implies that the metric components can depend only on the coordinates $(\eta, q_{\rm 1})$, while in the Szekeres symmetry the metric can depend in general on all spatial coordinates (and time). In~\cite{Meures:2011ke} this dependence is encoded in $A(q_{\rm 1},q_{\rm 2},q_{\rm 3})$ in Eq.~\eqref{eq:sz_X} and has the form
\begin{equation}
A= 1+ B \beta_{\rm +}(q_{\rm 1})\left[\left(q_{\rm2}+\gamma(q_{\rm 1})\right)^2+\left(q_{\rm 3}+\omega(q_{\rm 1})\right)^2 \right] \, ,
\label{eq:Sz_A}
\end{equation}
thus the only possibility to have $A=1$ is that $B=0$.
After simple manipulations of the Einstein equations together with Eq.~\eqref{eq:Sz_A} we find that 
\begin{equation}
2 B=\frac{3}{2}\frac{\stuff}{a} \mathcal{D} + \mathcal{H} \dot{\mathcal{D}} \, .
\end{equation}
In \cite{Villa:2015ppa} it is shown that the R.H.S. is constant and it is always different from zero. Indeed, from Eq.($5.52$) in \cite{Villa:2015ppa} we find
\begin{equation}
B= \frac{5}{4} \stuff \frac{\cal D_{\rm in}}{a_{\rm in}}\, ,
\label{eq:link_on_B}
\end{equation}
where $\mathcal{D}_{\rm in}= a_{\rm in}$ for Einstein-de Sitter initial conditions. We finally conclude that the two metrics \eqref{eq:Szekeres_metric} and \eqref{eq:app_metricNWT} cannot coincide.
\endinput


==> template/App_linear_obs.tex <==
\chapter{BGO at linear PT and linear observables} 
\label{apx:linear_obs}

\MG{da non-linearities}
\subsection{Solutions for the plane-parallel universe}

In this appendix we consider the flat FLRW background with linear perturbations in the synchronous-comoving gauge. We obtain the linearised evolution equations for the BGO, Eq.~\eqref{eq:1PT_BGO_syst}, the general expressions for their solutions, Eq.~\eqref{eq:1PT_BGO}, and the linear angular diameter distance $D_{\rm ang}^{\rm Lin}$ written in terms of the BGO, Eq.\eqref{eq:Dlin_lambda}.
We then specialise the general solutions to the $\Lambda$CDM background with perturbations at first order in standard cosmological perturbation theory and within our plane-parallel toy model and finally obtain the analytic expressions for $z^{\rm Lin}$ and $D_{\rm ang}^{\rm Lin}$ that we used in Section~\ref{sec:method}. 

The spacetime metric has the form
\begin{equation}
\tilde{g}_{\mu \nu}=a^2 g_{\mu \nu}
\end{equation}
and is expanded at first order as
\begin{equation}
\tilde{g}_{\mu \nu}= a^2 (\bar{g}_{\mu \nu}+\delta g_{\mu \nu})
\end{equation}
where $\bar{g}_{\mu \nu}$ is the conformal flat FLRW background, i.e. the Minkowski metric and $\delta g_{\mu \nu}$ represents the first-order scalar perturbations in the synchronous-comoving gauge, in general given by $\delta g_{\mu \nu}= {\rm Diag}(0, \delta g_{11}, \delta g_{22}, \delta g_{33})$.

The first observable that we study in this work is the redshift, defined as in Eq.~\eqref{eq:redshift_def}
\begin{equation}
1+z=\frac{\left.\tilde{g}_{\mu \nu}\tilde{\ell}^{\mu}\tilde{u}^{\nu}\right|_{\mathcal{S}}}{\left.\tilde{g}_{\mu \nu}\tilde{\ell}^{\mu}\tilde{u}^{\nu}\right|_{\mathcal{O}}}\,.
\label{eq:redshift_def_app}
\end{equation}
In the above expression ${u}^{\mu} $ is the four-velocity of the observer (source) and $\ell^{\mu}$ is the tangent vector to the photon geodesics. For our coordinates choice, all observers and sources are comoving with the cosmic flow with four-velocity given by 
\begin{equation}
\tilde{u}^{\mu}\equiv \frac{1}{a}\bar{u}^{\mu} =\frac{1}{a}\left(1 ,0, 0, 0\right)
\end{equation}
at all orders and the null tangent vector is expanded as
\begin{equation}
\tilde{\ell}^{\mu}=\frac{a^2_{\rm \mathcal{O}}}{a^2}\left(\bar{\ell}^{\mu}+\delta \ell^{\mu}\right)
\end{equation}
with $\bar{\ell}^{\mu}=\left(\bar{\ell}^{0}, \bar{\ell}^{i}\right)$
\footnote{The conformal tangent vector in the FLRW background $\bar{\ell}^{\mu}$ is constant. Note that usually the normalisation $\bar{\ell}^{0}\pm 1$ is used for the temporal component. Here, however, we leave it unnormalised.}. 
The linear redshift is then given by
 \begin{equation}
 1+z=\frac{a_{\mathcal{O}}}{a_{\mathcal{S}}}\left[ 1 +\frac{1}{\bar{\ell}^0} \left( \left.  \delta \ell^{0}\right|_{\mathcal{S}} - \left.  \delta \ell^{0}\right|_{\mathcal{O}} \right) \right]\, ,
 \label{eq:linear_z}
 \end{equation}
 where $\delta \ell^{0}$ is founded from the first-order geodesic equation
 \begin{equation}
 \frac{d \delta \ell^{\mu}}{d \lambda}= \frac{1}{2}\bar{g}^{\mu \sigma} \partial_{\sigma} \delta g_{\alpha \beta} \bar{\ell}^{\alpha}\bar{\ell}^{\beta}-\bar{g}^{\mu \sigma}\bar{\ell}^{\alpha} \partial_{\alpha} \delta g_{\sigma \beta}\bar{\ell}^{\beta}\,.
 \label{eq:lin_geod}
 \end{equation}
 
The second observable is the angular diameter distance $\tilde{D}_{\rm ang}$. However, it is more convenient to expand the conformal angular distance $D_{\rm ang}$ which we write here in terms of the BGO as (for a derivation see \cite{Grasso:2018mei} and \cite{Korzynski:2019oal})
\begin{equation}
D_{\rm ang}=\left. \ell^{\mu}u_{\mu}\right|_{\mathcal{O}}|\mathrm{det}(\WXL{}\UD{\boldsymbol{A}}{\boldsymbol{B}})|^{\frac{1}{2}}
\label{eq:dang_def_app_lin}
\end{equation}
and then obtain $\tilde{D}_{\rm ang}$ from the very well-known conformal transformation $\tilde{D}_{\rm ang}= \frac{a}{a_{\mathcal{O}}} D_{\rm ang}$, that we verified for Eq. \eqref{eq:dang_def_app_lin}.
The BGO $\WXL{}\UD{\boldsymbol{A}}{\boldsymbol{B}}$ are expanded as
\begin{equation}
\WXL{}\UD{\boldsymbol{A}}{\boldsymbol{B}}=\overline{\WXL}{}\UD{\boldsymbol{A}}{\boldsymbol{B}}+ \delta \WXL{}\UD{\boldsymbol{A}}{\boldsymbol{B}}\,,
\end{equation}
where $\overline{\WXL}$ and $\delta \WXL$ are found by solving the linearised GDE \eqref{eq:GDE_for_BGO} in conformal space
\begin{equation}
\frac{d}{d \lambda} \mathcal{W}=\begin{pmatrix}
0 & \mathbb{1}_{4 \times 4}\\
R_{\ell \ell} & 0
\end{pmatrix} \mathcal{W}
\end{equation} 
Notice that the optical tidal matrix in the frame is purely a first-order quantity - the conformal Riemann tensor vanishes in the background - and it is given by:
\begin{equation}
R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}=\bar{\phi}^{\rho \boldsymbol{\mu}} \delta R_{\rho \alpha \beta \sigma}\bar{\ell}^{\alpha} \bar{\ell}^{\beta}
 \bar{\phi}\UD{\sigma}{\boldsymbol{\nu}}
\end{equation}
where $\delta R_{\rho \alpha \beta \sigma}$ is the first-order Riemann tensor and $\bar{\phi}\UD{\mu}{\boldsymbol{\alpha}}=(u^{\mu}, \bar{\phi}\UD{\mu}{\boldsymbol{A}}, \bar{\ell}^{\mu})$ is the background parallel transported frame along the background geodesic.

Let us start by solving the background GDE, which reads:
\begin{equation}
\left\{\begin{array}{l}
\frac{d \, \overline{\WXX}{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}=\overline{\WLX}{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
\frac{d \, \overline{\WLX}{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}=0\\
\frac{d \, \overline{\WXL}{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}= \overline{\WLL}{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
\frac{d \, \overline{\WLL}{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}=0
\end{array}\right.
\label{eq:background_BGO_syst}
\end{equation}
with initial conditions $\overline{\mathcal{W}}=\mathbb{1}_{8 \times 8}$. The solution is
\begin{equation}
\overline{\mathcal{W}}=\begin{pmatrix}
\delta\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}} & (\lambda - \lambda_{\mathcal{O}})\delta\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
0 & \delta\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}
\end{pmatrix}
\label{eq:BGO_background}
\end{equation}
Next we find the first-order BGO from:
\begin{equation}
\left\{\begin{array}{l}
\frac{d \, \delta \WXX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}=\delta \WLX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
\frac{d \, \delta \WLX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}=R\UDDD{\boldsymbol{\mu}}{\ell}{ \ell}{ \boldsymbol{\nu}} \\
\frac{d \, \delta \WXL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}= \delta \WLL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
\frac{d \,  \delta \WLL {}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d \lambda}= (\lambda - \lambda_{\mathcal{O}})R\UDDD{\boldsymbol{\mu}}{\ell}{ \ell}{ \boldsymbol{\nu}} 
\end{array}\right.
\label{eq:1PT_BGO_syst}
\end{equation}
with initial conditions $\delta \mathcal{W}=\boldsymbol{0}_{8 \times 8}$, where we have replaced the background solutions \eqref{eq:BGO_background}.
We obtain
\begin{equation}
\left\{\begin{array}{l}
\delta \WXX{}\UD{\boldsymbol{\mu}}{ \boldsymbol{\nu}}=\int^{\lambda_{\mathcal{O}}}_{\lambda}\int^{\lambda_{\mathcal{O}}}_{\lambda'}R\UDDD{\boldsymbol{\mu}}{\ell}{ \ell}{ \boldsymbol{\nu}} d\lambda'd\lambda''\\
\delta \WXL{}\UD{\boldsymbol{\mu}}{ \boldsymbol{\nu}}= \int^{\lambda_{\mathcal{O}}}_{\lambda}(\lambda_{\mathcal{O}}-\lambda')(\lambda- \lambda')R\UDDD{\boldsymbol{\mu}}{\ell}{ \ell}{ \boldsymbol{\nu}} d\lambda'\\
\delta \WLX{}\UD{\boldsymbol{\mu}}{ \boldsymbol{\nu}}= -\int^{\lambda_{\mathcal{O}}}_{\lambda}R\UDDD{\boldsymbol{\mu}}{\ell}{ \ell}{ \boldsymbol{\nu}} d\lambda'  \\
\delta \WLL{}\UD{\boldsymbol{\mu}}{ \boldsymbol{\nu}}= \int^{\lambda_{\mathcal{O}}}_{\lambda}(\lambda_{\mathcal{O}}-\lambda')R\UDDD{\boldsymbol{\mu}}{\ell}{ \ell}{ \boldsymbol{\nu}} d\lambda'
\end{array}\right.\,.
\label{eq:1PT_BGO}
\end{equation}
In order to find $D_{\rm ang}^{\rm Lin}$ from the expansion of Eq.~\eqref{eq:dang_def_app_lin} we need the second of the above solutions and we recall that the expansion of the square root of the determinant is given by
\begin{equation}
\sqrt{\mathrm{det} W_{XL}}  = \sqrt{\mathrm{det} \left(\overline{W_{XL}}\right)}\left[ 1+\frac{1}{2}\mathrm{tr}\left(\overline{W_{XL}}^{-1} \delta W_{XL} \right) \right]
\end{equation}
Now, looking at Eqs.~\eqref{eq:BGO_background} and~\eqref{eq:1PT_BGO} we have that
\begin{equation}
\left\{\begin{array}{l}
\sqrt{\mathrm{det} \left(\overline{W_{XL}}\right)}=(\lambda-\lambda_{\cal O})\\
\mathrm{tr}\left(\overline{W_{XL}}^{-1} \delta W_{XL} \right)=\frac{\int^{\lambda_{\mathcal{O}}}_{\lambda}(\lambda_{\mathcal{O}}-\lambda')(\lambda- \lambda')R\UDDD{\boldsymbol{A}}{\ell}{ \ell}{ \boldsymbol{A}} d\lambda'}{(\lambda-\lambda_{\cal O})}
\end{array}\right.
\end{equation}
The final result for $D^{\rm Lin}_{\rm ang}$ is
\begin{equation}
\begin{array}{c}
D_{\rm ang}^{\rm Lin}=(\ell^{0}_{\mathcal{O}}+\delta \ell^0_{\mathcal{O}})(\lambda_{\mathcal{O}}-\lambda)\\
-\frac{\ell^{0}_{\mathcal{O}}}{2}\int^{\lambda_{\mathcal{O}}}_{\lambda}(\lambda_{\mathcal{O}}-\lambda')(\lambda- \lambda')\mathrm{tr}\left(R\UDDD{\boldsymbol{A}}{\ell}{ \ell}{ \boldsymbol{B}}\right) d\lambda'\,.
\end{array}
\label{eq:Dlin_lambda}
\end{equation}
It is important to stress that all the quantities are evaluated along the background geodesic, i.e. $\eta \equiv \bar{\eta}$ and $\bar{q}_{\rm 1}(\eta)\equiv \frac{\bar{\ell}^1}{\bar{\ell}^0}(\bar{\eta}_{\rm \mathcal{O}}-\bar{\eta})+\bar{q}_{\rm 1}(\bar{\eta}_{\rm \mathcal{O}})$

We checked that our result coincides with the standard result in the literature, e.g. \cite{di2016curvature}, by simply noting that the quantity $-\frac{1}{2}\mathrm{tr}\left(R\UDDD{\boldsymbol{A}}{\ell}{ \ell}{ \boldsymbol{B}}\right)$ is nothing more than the Ricci part of the optical tidal matrix $\mathcal{R}$, usually defined as
\begin{equation}
\mathcal{R}=\frac{1}{2}R_{\alpha \beta} \ell^{\alpha} \ell^{\beta}=-\frac{1}{2}R\UDDD{\mu}{\alpha}{\beta}{\mu} \ell^{\alpha} \ell^{\beta}\,,
\end{equation}
and evaluated at first order. 

We finally specialise the above results for our plane-parallel model. The linear perturbation of the spacetime metric around the flat $\Lambda$CDM background is
\begin{equation}
\delta g_{\mu \nu}=\begin{pmatrix}
0 & 0 & 0 & 0\\
0 & -\mathcal{F}-\frac{10}{3 c^2}\phi_{\rm 0} & 0 & 0\\
0 & 0 & -\frac{10}{3 c^2}\phi_{\rm 0} & 0\\
0& 0 & 0 & -\frac{10}{3 c^2}\phi_{\rm 0}
\end{pmatrix}\, ,
\label{eq:sync_gauge_quantities}
\end{equation}
where we define 
\begin{equation}
\mathcal{F}(\eta, q_{\rm 1})=\frac{4}{3}\frac{\partial^2_{\rm q_{\rm 1}}\phi_{\rm 0}(q_{\rm 1})}{\stuff}\mathcal{D}(\eta)
\end{equation}
A straightforward substitution gives for the redshift
 \begin{equation}
 \begin{array}{l}
 1+z^{\rm Lin}=\\
 \vspace*{0.5 cm} \frac{a_{\mathcal{O}}}{a_{\mathcal{S}}}\left[ 1 -\left(\frac{\bar{\ell}^1}{\bar{\ell}^0}\right)^2 \int^{\bar{\eta}_{\mathcal{O}}}_{\bar{\eta}_{\mathcal{S}}} \frac{2}{3}\frac{\partial_{\rm q_{\rm 1}} \phi_{\rm 0}(q_{\rm 1}(\bar{\eta}'))}{\stuff}\partial_{0}{\mathcal{D}}(\bar{\eta}')   d \bar{\eta}' \right]
 \end{array}
 \label{eq:zlin_plane-parallel_2}
 \end{equation}
and for the angular diameter distance
\begin{equation}
\tilde{D}^{\rm Lin}_{\rm ang}(\eta)=\frac{a}{a_{\mathcal{O}}}\left[(\bar{\eta}_{\rm \mathcal{O}}-\bar{\eta})+ \frac{\bar{\ell}^{1^2}}{2 \bar{\ell}^{0^2}}\int^{\eta_{\rm \mathcal{O}}}_{\eta} \int^{\eta_{\rm \mathcal{O}}}_{\eta'}  \dot{\mathcal{F}} d\eta'd\eta''+\int^{\eta_{\rm \mathcal{O}}}_{\eta}(\eta_{\rm \mathcal{O}}-\eta')(\eta-\eta') \frac{\mathcal{R}(\eta')}{\bar{\ell}^{0^2}}  d\eta'\right]
\label{eq:Dang_time_conf}
\end{equation}
The two last relations are those we use in section~\ref{sec:method} for our comparison.
\endinput


==> template/App_package.tex <==
\chapter{APPENDIX B: \\ BiGONLight functions's descriptions}

\endinput


==> template/App_units.tex <==
\chapter{Units}
\MG{da bigonlight paper}
\label{apx:Units}

Throughout this article all quantities are expressed in geometric units, i.e. units defined by the relation $G = c = 1$, thus such that masses, time and lengths have the same unit of measurement. For instance, we can fix a unit of length\footnote{The same can be done by fixing a unit of time $T$ to define $[mass]=T \frac{c^3}{G}$ as unit of mass and $[length]=T c$ as unit of length, or fixing a unit of mass $M$ to define $[time]=M \frac{G}{c^3}$ as unit of time and $[length]=M \frac{G}{c^2}$ as unit of length.} $[length]=L$ and define $[mass]=\frac{c^2 L}{G}$ as unit of mass and $[time]=\frac{L}{c}$ as unit of time: in geometric units they all reduce to $[mass]=[time]=[length]=L$. Within this choice, every physical quantity $Q_{\rm phys}$ can be expressed as $Q_{\rm phys}=Q_{\rm comp} L^{\alpha}$, where $Q_{\rm comp}$ is dimensionless, $L$ is a arbitrary length to be chosen, and $\alpha$ is a certain exponent. This way of writing is particularly useful in numerical simulations, where all physical quantities are represented as dimensionless numbers and units are assigned when analysing the results.
Usually $L$ is fixed to be a length meaningful for the specific physical situation under consideration. For example, a common choice in numerical cosmological dynamics is to set $L$ equal to a characteristic length of the simulation (e.g. N-body and GR hydrodynamics), such as the side of the simulated box. 
In cosmology it is usually chosen to set $L$ equal to the conformal time in Mpc, i.e. $L=\eta^{\rm phys}$, thus $\eta^{\rm comp}=1$, at some special instant like e.g. at initial time or today. This choice is particularly convenient, since  conformal time is found by integrating the Friedmann equation and reads
 \begin{equation}
 %\dfrac{\dot{a}}{a}=H_0 a E(a)
 \eta =\dfrac{1}{H_0}  \mathlarger{\int}^{a}_{0} \dfrac{d \tilde{a}}{\tilde{a}^2E(\tilde{a})}\, ,
 \label{eq:UNITS_eta}
 \end{equation}
where $E(a)=\sqrt{\Omega_{\rm m_0}\left(\frac{a_0}{a}\right)^3+\Omega_{\rm \Lambda}}$ for a universe containing cold dark matter and a cosmological constant. 

For the $\Lambda$CDM model, Sec.~\ref{sec:LCDM}, and for the Szekeres model, Sec.~\ref{sec:Szekeres}, we choose $L=\eta_0$ and we normalize the scale factor to 1 today. This is the natural choice for this two cases since we studied light propagation backward in time.
By integrating Eq.~\eqref{eq:UNITS_eta} together with the normalization $a_0=1$ for the value of the today scale factor we have
\begin{equation}
 %\eta =\dfrac{ \mathlarger{\int}^{a_0}_{a} \dfrac{\tilde{a}^{-2}}{\sqrt{\tilde{a}^{-3}\Omega _{\rm m0}+ \Omega _{\Lambda }}} \, d \tilde{a} }{\mathcal{H}_0}
\eta^{\rm \Lambda CDM} = \dfrac{1}{\mathcal{H}_0  3^{\frac{1}{4}} \Omega_{\Lambda}^{\frac{1}{6}} \Omega_{\rm m_0}^{\frac{1}{3}}} F\left( \arccos\left(\frac{1+(1-\sqrt{3})\sqrt[3]{\frac{\Omega_{\Lambda}}{\Omega_{\rm m_0}}}a}{1+(1+\sqrt{3})\sqrt[3]{\frac{\Omega_{\Lambda}}{\Omega_{\rm m_0}}}a}\right);\frac{\sqrt{2+\sqrt{3}}}{2}\right)\, ,
\label{eq:UNITS_eta_LCDM}
 \end{equation}
with $F(x;y)$ being the elliptic integral of the first kind. Substituting the values of the cosmological parameters from \cite{planck2018param}, $\Omega_{\rm m_0}=0.315$ and $\Omega_{\rm \Lambda}=0.685$ and expressing the Hubble constant in Mpc, i.e. $\mathcal{H_{\rm 0}}=2.2469 \times 10^{-4}\, {\rm Mpc^{-1}}$, Eq.~\eqref{eq:UNITS_eta_LCDM} gives $L=\eta^{\rm \Lambda CDM}_0=\eta^{\rm Sz}_0=14.4152\,  \text{Gpc}$.

For the EdS model, Sec.~\ref{sec:ET}, we study light propagation forward in time and we decided to use the same conventions as the one implemented in the ET. Here, the simulation is carried out in a cubic domain volume of comoving side $2L$, which is initialised at initial time  $\eta_{\rm in}$ (and not today) and the scale factor is normalised to 1 at $\eta_{\rm in}$. Let us start by integrating \eqref{eq:UNITS_eta} for the EdS model, i.e. $\Omega_{\rm m_0}=1$ and $\Omega_{\rm \Lambda}=0$, which gives
\begin{equation}
\eta^{\rm EdS}=\dfrac{2}{\mathcal{H}_0}\sqrt{\dfrac{a}{a_0}}\, .
\label{eq:UNITS_eta_EdS}
\end{equation}
The value of $L$ is set by evaluating Eq.~\eqref{eq:UNITS_eta_EdS} at initial time and choosing $\eta^{\rm EdS}_{\rm in}=L$. Substituting $a_{\rm in}=1$ and $\sqrt{a_0}=33.2$ from the numerical simulation, and $\mathcal{H}_{0}=2.2469 \times 10^{-4}\, {\rm Mpc^{-1}}$ from \cite{planck2018param} in Eq.~\eqref{eq:UNITS_eta_EdS}, it follows that the value of $L$ is
\begin{equation}
L=268.11 \, {\rm Mpc}\, .
\end{equation}

We report for completeness the dimensions of all the main quantities in units of the characteristic length $L$
\begin{table}[ht!]
\centering
\begin{tabular}{|l|l|}
\hline
 \multicolumn{2}{|c|}{Physical quantities in units of $L$} \\
 \hline
Hubble constant & $\mathcal{H}_0^{\text{phys}}  = \mathcal{H}_0^{\text{comp}}L^{-1}$\\
Conformal time & $\eta_{\rm phys}=\eta_{\rm comp} L $\\
Spatial coordinates & $x_{\rm phys}^i=x_{\rm comp}^i L$\\
Gravitational potential & $\phi_0^{\rm phys}= \phi_0^{\rm comp} L^0$\\
Velocity field & $\nabla \phi_0^{\rm phys}= \nabla \phi_0^{\rm comp} L^{-1}$\\
Density field & $\nabla^2 \phi_0^{\rm phys}= \nabla^2 \phi_0^{\rm comp} L^{-2}$\\
Frequency & $\omega^{phys}=\omega^{comp} L^{-1}$\\
Angular diameter distance &  $D_{\rm ang}^{phys}=D_{\rm ang}^{comp} L$\\
Parallax distance &  $D_{\rm par}^{phys}=D_{\rm par}^{comp} L$\\
Redshift drift & $\zeta^{phys}=\zeta^{comp} L^{-1}$\\
Redshift $z$ & dimensionless\\
Scale factor $a(\eta)$ & dimensionless\\
Growing mode $\mathcal{D}(\eta)$ & dimensionless\\
Cosmological parameters $\Omega_i$ & dimensionless\\
\hline
\end{tabular}
\end{table}
\endinput


==> template/bigonlight.tex <==
\chapter{The BiGONLight package}%bigonlight
\label{chap:bigonlight}
The BGO framework in Sec.~\ref{sec:BGO} offers a uniform theoretical approach to describe various optical phenomena due to light propagation in a curved spacetime. The only limits to the formalism are imposed by those of the GDE, which are valid for most of the observations in astronomy. Conversely, no assumptions are made on the details of the spacetime geometry, making the BGO the ideal machinery to study general and nonperturbative relations between gravitational lensing, parallax effects and drift effects all within the same framework. 
The most straightforward application of the BGO formalism is the computation of observables in astrophysics and cosmology, since the observables are easily given as combination of BGO and the source and the observer four-velocities and four-accelerations. This method is particularly useful in numerical relativity, when it is applied to extract observables from numerical relativistic simulations of the spacetime. In fact, it just requires of solving a number of linear ODE's using geometric data collected along a null geodesic. Numerical relativistic simulations are currently becoming one of the most important tools of theoretical cosmology, able to reproduce  ``virtual copies'' of the universe on which perform tests and measurement forecasts \cite{Bentivegna:2012ei, Yoo:2013yea, Bentivegna:2013jta, Yoo:2014boa, Bentivegna:2015flc, Giblin:2015vwq, Mertens:2015ttp, Adamek:2015eda, Adamek:2016zes, Macpherson:2016ict, Macpherson:2018akp}. In this prospective, the use of drift effects to constraint cosmological models has recently been considered by many authors \cite{quercellini,Quercellini:2008ty,Fontanini:2009qq,Quercellini:2009ni,Krasinski:2012ty, Krasinski:2011iw, Krasinski:2012nw, Krasinski:2010rc,rasanen,  KrasiNSki:2015nta}. However, while the null geodesic tracking is a fairly standard problem in numerical relativity \cite{Vincent:2012kn, Bentivegna:2016fls}, extracting the drift effects is not. It is, of course, possible to do it without the BGO, by doing ray tracing of a number of geodesics connecting observer and emitter at consecutive moments, but this procedure is rather cumbersome.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this chapter we present {\tt BiGONLight}\footnote{{\color{blue}{\tt {https://github.com/MicGrasso/bigonlight.git}}}.}, \textbf{Bi}local \textbf{G}eodesic \textbf{O}perators framework for \textbf{N}umerical \textbf{Light} propagation, a \texttt{Mathematica} package developed for extracting observables from numerically generated spacetimes using the BGO formalism. The principal aim of the package is to provide a unified procedure to calculate multiple observables in numerical relativity: this is guaranteed since, once that the BGO are determined from the output metric of a numerical simulation, a all set of observables are obtained within the same computation. In order to be compatible with the majority of the codes in Numerical Cosmology, {\tt BiGONLight} encodes the BGO formalism in $3+1$ form and it uses the \texttt{Mathematica} powerful symbolic algebra manipulation and precision control options. The concepts presented in this chapter are published in \cite{Grasso:2021iwq}.
%The paper is organized as follows: in Sec.~\ref{sec:light}, we give the fundamentals of light propagation and its formulation in terms of Bi-local Geodesic Operators. In Sec.~\ref{sec:3+1} we  present {\tt BiGONLight} and the equations to compute the BGO in $3+1$ form encoded into the package. The recipe to compute observables in numerical relativity using {\tt BiGONLight} and the expressions of the observables in terms of BGO are given in Sec.~\ref{sec:obs}. The last section of this paper, Sec.~\ref{sec:test}, is dedicated to the code tests, which are performed in the following three cosmological models: $\Lambda$CDM (see Sec.~\ref{sec:LCDM}), Szekeres (see Sec.~\ref{sec:Szekeres}), and a numerically evolved dust universe (see Sec.~\ref{sec:ET}). We draw our conclusions in Sec.~\ref{sec:concl}.\\

%\section{State of the art on light propagation in numerical relativity}

%The increasing amount of observational data we had in the last decades has triggered significant progress in the field of cosmology. The theoretical framework commonly used to interpret these data is the $\Lambda$CDM model, which assumes that the large scale geometry of the Universe is described by the spatially homogeneous and isotropic Friedmann-Lema\^{i}tre-Robertson-Walker (FLRW) model, with galaxies and clusters of galaxies producing just small metric perturbations. The dynamics of the FLRW model is governed by the Friedmann equations with an equation of state sourced mainly by two unknown substances: the dark energy, a mysterious energy responsible for the accelerated expansion of the universe, and the (cold) dark matter, an exotic type of matter interacting with radiation and ordinary matter only through gravity. \MG{If from one side the dynamics of the universe as a whole is described by the Friedmann equations, on the other side we still need to describe the formation of structures like galaxies and clusters of galaxies which are visible on smaller scales.} The current large scale structure of the universe is evolved from the primordial small fluctuations, which are visible in the CMB. These perturbations acted like initial seeds from which, under the influence of gravity, grew all other structures like galaxies and cluster of galaxies.
%The evolution of these cosmic seeds is described by general relativity and several methods have been developed to do that. \MG{At early times, these small inhomogeneities are well described by linear perturbation theory, i.e. their dynamics is described by the solution of the Einstein equation at linear order. However, GR is a nonlinear theory implying that nonlinear effects in the inhomogeneities dynamics may be relevant in the structure formation.}
%The role of the nonlinear General-Relativistic effects from these inhomogeneities has been discussed by many authors \cite{}, with particular emphasis in their contribute to the accelerated expansion of the universe.

%Therefore, treating non-linearities in the cosmological structure dynamics is of crucial importance and several approximation schemes were developed specifically or approximations used in other contexts were applied to cosmology. (PLACE A BRIEF EXPLANATION ON WHAT THEY DO) They include: the post-Newtonian (PN) approximation (see \cite{mater, carbone2005unified} for formulations of PN cosmology in two different gauges), the post-Friedmann approximation (see \cite{Milillo:2015cva, Rampf:2016wom} for a different approach, which adapts to cosmology the weak-field post-Minkowskian approximation and reproduces linear-order cosmological perturbation theory at their zeroth-order), the weak-field approximation\footnote{The leading order of the last two approximation schemes were shown to be equivalent for a dust universe in the Poisson gauge in \cite{kopp2014newton}, whereas \cite{mater, carbone2005unified} were constructed on purpose to include second-order perturbation theory at their PN order.} (see \cite{green2011new} for the development of the framework and \cite{Adamek:2013wja} for estimations with the use of Newtonian simulations for a plane-symmetric universe), and, more recently, a two-parameters gauge-invariant approximation (see \cite{Goldberg:2016lcq}). 
%In addition, over the past few decades, numerical simulations have increasingly become a powerful tool in cosmology to model the growth of nonlinear structures. Since Newtonian dynamics seems to be a good approximation to describe late-time structure formation, the first generation of cosmological simulations adopted Newtonian gravity to simulate cosmological dynamics. Then, Newtonian simulations were used to feed approximate field equations coming from General Relativity (GR) as e.g. in \cite{Bruni:2013mua, Adamek:2014xba, Fidler:2017pnb}. Only recently we assist to a revolution in cosmological simulations with the birth of codes aiming at simulating fully general relativistic dynamics, \cite{loffler2012einstein, Bentivegna:2016stg, mertens2016integration, adamek2016general, macpherson2017, barrera2020gramses}: for the state of the art and the comparison among different codes, see \cite{Adamek:2020jmr}.

%%However, a sophisticated general relativistic (exact or approximated) description of cosmological dynamics is not the end of the story. The key point is how (much) it affects light propagation, the final aim being to characterize and (hopefully) measure nonlinear GR effects in the observables on cosmological scales or, at least, quantify their bias in observations. These studies are still in their infancy but they are addressed with several approaches most of which we briefly sketched above. A noncomprehensive list includes \cite{Thomas:2014aga, Barreira:2016wqo, Borzyszkowski:2017ayl, Sanghai:2017yyn, Giblin:2017ezj, Adamek:2018rru, Gressel:2019jxw, Lepori:2020ifz, Macpherson:2021gbh}.
%%Despite being too early to draw definitive conclusions, it seems that the codes that approximate GR dynamics are in agreement with Newtonian simulations for what concerns weak-lensing observables \cite{Thomas:2014aga, Lepori:2020ifz} but a modification in the statistics of the luminosity distance \cite{Adamek:2018rru} was found. In addition, the PN approximation for some models gives predictions different from $\Lambda$CDM \cite{Sanghai:2017yyn}. A bit of work is still needed to adapt to (observational) cosmology the truly GR numerical codes. 

%\MG{The simulations represent a virtual laboratory where recreate copies of the universe, which are then used to perform tests and comparison with real observations. On this point it is fundamental the analysis of optical phenomena like gravitational lensing and the forecast of observables like e.g. the luminosity distance to test the distance-redshift relation, main indication of dark energy. }
%On the other hand relativistic effects in the non-linear regime have recently become to be investigated with relativistic simulations in galaxy clustering and lensing observables, and the Hubble diagram, see e.g. \cite{Borzyszkowski:2017ayl, Zhu:2017jfl, Giblin:2017ezj, Breton:2018wzk, Adamek:2018rru, Beutler:2020evf, Lepori:2020ifz, Guandalin:2020snp, Lepori:2021lck} and refs. therein. \MG{Add that light propagation and observables are computed using perturbative schemes (refer to papers where D lum is computed at first and second order) whose expression depends on the geometrical characteristics of the model and on the perturbation scheme  (and order) used!}

%%%%%%QUI
%%\MG{Several ways to include non-linearities: PT, PN, other perturbative schemes where inhomogeneites are considered small statistical fluctuations over a homogeneous background. On the other hand, numerical method can be used to solve einstein equation as an evolutionary problem starting from appropriate initial conditions. Firstly used in strong field regime to describe binary systems, GW emission, BH accretion, it was also used in cosmology to describe an ensamble of galaxies moving with newtonian dynamics over a homogeneous background. Take from nonlinearities paper! + ``In order to make the most from this revolution in observational astronomy and cosmology, the same accuracy is required in the theoretical predictions and interpretations of what we measure. This tough task requires much effort from two sides. At one hand the most recent progress on cosmological dynamics are represented by  general-relativistic simulations of cosmic structures with no assumed symmetries employing exact solutions of Einstein equations, \cite{loffler2012einstein,Giblin:2015vwq,Bentivegna:2016stg,macpherson2017,Clesse:2017jjp,East:2017qmk,Daverio:2019gql}, or approximated treatments, \cite{adamek2016general,barrera2020gramses}. The common ambitious aim is to have a description valid from large to small scales which accounts for relativistic effects. '' }. 



%\MG{In this panorama the new approach of BGO \cite{Grasso:2018mei} represents the perfect machinery to study light propagation in numerical relativity, providing a unified framework to extract multiple observables within the same calculation and this is easily adaptable to perform light propagation on-the-fly with a simulation of relativistic dynamics. }
%For this purpose, we develop {\tt BiGONLight} (\textbf{Bi}-local \textbf{G}eodesic \textbf{O}perator framework for \textbf{N}umerical \textbf{Light} propagation), a {\tt Mathematica} package which simulates light propagation in Numerical Relativity within the BGO formalism, described in Sec.~\ref{sec:BGO}. It is publicly available at the repository {\color{blue}{\tt {https://github.com/MicGrasso/bigonlight.git}}} and it works as an external library that can be called inside a {\tt Mathamatica} notebook.  %\texttt{Mathematica} provides a large variety of numerical methods that can be used and customized to adapt them to the particular problem, as well as several precision control options, which allows the user to set the  precision and accuracy of numerical result through the commands \texttt{WorkingPrecision}, \texttt{SetPrecision} and \texttt{SetAccuracy}.
%%  This is exploited in the functions {\tt SolveGeodesic[]}, {\tt SolveEnergy[]}, {\tt PTransportedFrame[]} and {\tt SolveBGO[]} in which the user can choose the numerical methods used to solve the system of ODE\footnote{The user can choose between three different methods: $``RK''$ a $4^{th}$ order Runge-Kutta method, $``A''$ which lets {\tt Mathematica} to decide what is the best method to use, and $``SS''$ denoting the Stiffness-Switching method, which allows to switch between implicit and explicit methods to resolve stiff problems.}. Another useful feature is the \texttt{Mathematica}'s precision control options, which allows the user to set the  precision and accuracy of numerical result through the commands \texttt{WorkingPrecision}, \texttt{SetPrecision} and \texttt{SetAccuracy}. 
%In the following we will show how to recast as an evolutionary problems the covariant equations in the BGO framework, and the procedure to obtain the BGO implemented in the code. %We dedicate a separate chapter, Chap.~\ref{cha:obs}, to the computation of the observables once the BGO are known. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{The BGO framework in 3+1 form}
\label{sec:3+1}

\MG{USED IN CHAP. COSMOLOGY: To perform  simulations of full-GR dynamical systems in numerical relativity, one needs to separate the temporal and the spatial dependence in the Einstein field equation, to recast their expression in the form of an evolutionary problem. This procedure is known as $3+1$ splitting of the spacetime and it commonly used by the numerical codes in cosmology and astrophysics. To be compatible with the numerical output generated by these codes, in {\tt BiGONLight} we adopt the BGO framework expressed in the 3+1 form.
In the following we summarise some basic definitions of the 3+1 formalism and report the 3+1 version of all the equations for light propagation used to compute the BGO. For comprehensive references of the 3+1 formalism see e.g. \cite{Smarr:1977uf, Alcubierre2008, baumgarte2010numerical, gourgoulhon20123+}.

The procedure of splitting a four-dimensional spacetime $(\mathcal{M},g_{\mu \nu})$ into its $3+1$ form, the so-called ADM formalism, was introduced by Arnowitt, Deser and Misner in \cite{arnowitt1959}. It is constructed by foliating a four-dimensional manifold $\mathcal{M}$ with a family of 3D space-like hypersurfaces $\Sigma_t$, labelled by a monotonic function $t$, such that $t=\const$ on each slice. This space-like foliation defines the time-like vector field $n^{\mu}$, which is orthonormal to the slices and it can be regarded as the four-velocity of Eulerian observes. 
The geometry on each hypersurface is described by the following quantities:
\begin{itemize}
\item the induced metric $\gamma_{\mu \nu}$ is defined as the covariant form of the orthogonal projector onto the slices 
\begin{equation}
\gamma_{\mu \nu}=g_{\mu \nu} + n_{\mu}n_{\nu}
\end{equation}
and it is used to measure proper distances on $\Sigma_t$;
\item the covariant derivative on the slice
\begin{equation}
D_{\nu}V^{\mu}=\gamma\UD{\sigma}{\nu}\gamma\UD{\mu}{\rho}\nabla_{\sigma}V^{\rho} \, ,
\label{eq:3D_covD}
\end{equation}
which is written in terms of the 3D Christoffel symbol ${}^{(3)}\Gamma^{k}_{\ i j}=\frac{1}{2}\gamma^{k l}(\frac{\partial \gamma_{l j}}{\partial x^i}+\frac{\partial \gamma_{i l}}{\partial x^j}-\frac{\partial \gamma_{i j}}{\partial x^l})$, once a coordinate system ${x^i}$ on $\Sigma_{t}$ is introduced;
\item the extrinsic curvature $K_{\mu \nu}$ defined as
\begin{equation}
K_{\mu \nu}=-\gamma\UD{\sigma}{\mu}\gamma\UD{\rho}{\nu}\nabla_{\sigma}n_{\rho}\, ,
\label{eq:K_def}
\end{equation}
which represents the curvature of the 3D hypersurfaces with respect to the 4D embedding spacetime.
\end{itemize}
A natural choice for a coordinate system $x^{\mu}$ is the one adapted to the foliation: the corresponding reference frame is such that the three vectors $\partial^{\mu}_i=\left(\frac{\partial}{\partial x^i}\right)^{\mu}$ are tangent to the hypersurface while $\partial^{\mu}_0=\left(\frac{\partial}{\partial t}\right)^{\mu}$ is transverse to it. In particular, the time-like vector field $\left(\frac{\partial}{\partial t}\right)^{\mu}$ is tangent to a congruence of world-lines of coordinate observers and it is given by
\begin{equation}
\left(\dfrac{\partial}{\partial t}\right)^{\mu}=\alpha n^{\mu}+\beta^{\mu}\, ,
\end{equation}
where $\alpha$ is the lapse function, which measures the proper time of the Eulerian observers, and $\beta^{\mu}$ is the  shift vector, which quantifies the displacement on $\Sigma_t$ of the coordinate observer $\left(\frac{\partial}{\partial t}\right)^{\mu}$ with respect to the Eulerian observer $n^{\mu}$. 
The components of the normal vector and the metric $g_{\mu \nu}$ in the adapted coordinates are written with the lapse, the shift and the induced metric as
\begin{equation}
n^{\mu}=(\dfrac{1}{\alpha},-\dfrac{\beta^i}{\alpha})\, ,
\label{eq:nu_nd}
\end{equation}
and
\begin{equation}
g_{\mu \nu}=\begin{pmatrix}
\beta_{i}\beta^i-\alpha^2 &~ \beta_i\\
\beta_j &~ \gamma_{i j}
\end{pmatrix}\, ,
\label{eq:g_3+1}
\end{equation}
where the Latin indices runs from $1$ to $3$. A generic 4D tensor is projected on the slice as 
\begin{equation}
{}^{(3)}T^{\mu_{\rm 1} \cdots \mu_{\rm m}}_{ \ \ \nu_{\rm 1} \cdots \nu_{\rm n}}={}^{(4)} T^{\rho_{\rm 1} \cdots \rho_{\rm m}}_{ \ \ \sigma_{\rm 1} \cdots \sigma_{\rm n}} \gamma\UD{\mu_{\rm 1}}{\rho_{\rm 1}}\cdots\gamma\UD{\mu_{\rm m}}{\rho_{\rm m}} \gamma\UD{\sigma_{\rm 1}}{\nu_{\rm 1}}\cdots\gamma\UD{\sigma_{\rm n}}{\nu_{\rm n}}\, .
\label{eq:3Dproj}
\end{equation}  

}

The idea behind the design of our package is to create a tool which is adaptable to perform analytical as well as numerical studies of light propagation, using only few   inputs provided by the user.
The required input are the specetime metric and the source/observer kinematics, which can be provided in two different ways: (i) from the output of a relativistic numerical simulation of the spacetime dynamics, i.e. directly the ADM quantities ($\alpha, \, \beta^i,\, \gamma_{i j},\, K_{i j}$) generated by a numerical simulation, (ii) from the analytical expression of the metric $g_{\mu \nu}$ and the emitter/observer four-velocities ($u^{\mu}_{\mathcal{S}}$, $u^{\mu}_{\mathcal{O}}$) and four-accelerations ($w^{\mu}_{\mathcal{S}}$, $w^{\mu}_{\mathcal{O}}$) for some exact model. In this case, the ADM quantities are computed in {\tt BiGONLight} by the function {\tt ADM[]} accordingly to Eqs.~\eqref{eq:K_def},~\eqref{eq:nu_nd},~\eqref{eq:g_3+1}.
On top of that, \texttt{BiGONLight} contains other functions to calculate the Christoffel symbols, \texttt{Christoffel[]}, and the Riemann tensor, \texttt{Riemann[]}. 
Note that in both cases, the input metric is provided in form of components within a specific coordinate system and not in full tensorial form. The package is designed to work in any gauge and any coordinate system, leaving the choice to the user. 
Once we have summarized the basics, we will now describe in more details and step by step the procedure for obtaining the BGO in the 3+1 decomposition: we report the 3+1 version of the geodesic equation following \cite{Vincent:2012kn} and we derive all the 3+1 ingredients for the evolution equation of the BGO.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Geodesic equation in $3+1$ decomposition}
The first code solving the $3+1$ geodesic equation was presented in \cite{hughes1994finding} and it was used to map the event horizon in numerical simulations with black holes (like heads-on collision of two black holes), while a more recent formulation of the $3+1$ geodesic equation was presented in~\cite{Vincent:2012kn}. Here, we briefly resume the procedure in~\cite{Vincent:2012kn}, since we will use their approach throughout all our calculations.

The null geodesics representing light rays connecting source and observer is obtained by solving 
\begin{equation}
\ell^{\sigma}\nabla_{\sigma} \ell^{\mu}=0
\label{eq:covar_geo}
\end{equation}
where $\ell^{\mu}$ is the tangent vector which obeys to the null condition
\begin{equation}
\ell^{\sigma}\ell_{\sigma}=0\, .
\label{eq:null_cond}
\end{equation}
It is $3+1$ decomposed as:
\begin{equation}
\ell^{\mu}=\calE(n^{\mu}+V^{\mu})\, ,
\label{eq:l_split}
\end{equation} 
where $\calE$ is defined by $\calE=-n^{\mu} \ell_{\mu}$ and $V^{\mu}n_{\mu}=0$. In other words, $\calE V^{\mu}$ is the component of $\ell^{\mu}$ tangent to $\Sigma_t$ and $\calE n_{\nu}$ is the orthogonal one. Substituting Eq.~\eqref{eq:l_split} in the geodesic equation~\eqref{eq:covar_geo}
after a long but straightforward calculation, see~\cite{Vincent:2012kn}, the geodesic equation decouples in two differential equations
\begin{equation}
\dfrac{d \calE}{d t}= \calE \left(\alpha K_{i k} V^j V^k - V^j \partial_j \alpha \right)\, ,
\label{eq:3+1_geodE}
\end{equation}
\begin{equation}
\left\{ \begin{array}{l}
\dfrac{d x^i}{d t}= \alpha V^i - \beta^i \\
 \\
\dfrac{d V^i}{d t}= \alpha V^j \left[V^i \left( \partial_j \log \alpha - K_{j k} V^k \right) +2K^i_{\ \ j} - {}^{(3)}\Gamma^i_{\ j k} V^k \right] - \gamma^{i j} \partial_j \alpha - V^j \partial_j \beta^i
\end{array}\right.
\label{eq:3+1_geodV}
\end{equation}
for the orthogonal and the tangent components, respectively.

In the \texttt{BiGONLight} package the two functions  \texttt{EnergyEquations[]} and \texttt{GeodesicEquations[]} give the differential equations~\eqref{eq:3+1_geodE} and~\eqref{eq:3+1_geodV}, respectively. Next, we need to specify the initial conditions. The function \texttt{InitialConditions[]} is specifically constructed to get the initial conditions for $V^i$ and $\calE$ consistent with the null condition~\eqref{eq:null_cond} and the decomposition~\eqref{eq:l_split}.
The ODE~\eqref{eq:3+1_geodE} and~\eqref{eq:3+1_geodV} are then solved by using two customized versions of the Mathematica \texttt{NDSolve[]} function: \texttt{SolveEnergy[]} and \texttt{SolveGeodesic[]}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Parallel transport equation in the $3+1$ decomposition}
The BGO map the changes of the deviations ($\delta x^{\mu}$, $\Delta \ell^{\mu}$) between the observer $\calO$ and the source $\cal S$ along the photon geodesic $\gamma$, see Eq.~\eqref{eq:compact_W(S,O)}. This is possible only if we introduce a frame parallel transported along $\gamma$, which allows us to compare quantities at the observation point and at source position. For our purposes, the definition and the parallel transport of the frame have to be split into the 3+1 form. 
Let us start with the parallel transport of a generic vector $e^{\mu}$ along a given geodesic with tangent $\ell^{\mu}$, which is governed by
\begin{equation}
\ell^{\alpha}\nabla_{\alpha}e^{\mu}=0\, .
\label{eq:parallel_transport}
\end{equation}
The 3+1 decomposition of $e^{\mu}$ reads
\begin{equation}
e^{\mu}=C n^{\mu}+E^{\mu}\, ,
\label{eq:e_split}
\end{equation}
where we have defined the orthogonal component $C n^{\mu}=-n_{\alpha}e^{\alpha} n^{\mu}$ and the tangent component $E^{\mu}=\gamma\UD{\mu}{\alpha} e^{\alpha}$. 
The parallel transport equation~\eqref{eq:parallel_transport} becomes
\begin{equation}
n^{\mu}(n^{\alpha}\nabla_{\alpha} C+V^{\alpha}\nabla_{\alpha}C)+C(n^{\alpha}\nabla_{\alpha}n^{\mu}+V^{\alpha}\nabla_{\alpha}n^{\mu})+n^{\alpha}\nabla_{\alpha}E^{\mu}+V^{\alpha}\nabla_{\alpha}E^{\mu}=0\, .
\label{eq:PT_interm_1}
\end{equation}
Now, we make use of some $3+1$ well-known relations: for the first term we have $n^{\mu}\nabla_{\mu}C=\frac{1}{\alpha} \mathcal{L}_{\alpha \vec{n}}C$, in the second bracket we substitute $n^{\alpha}\nabla_{\alpha}n^{\mu}=D^{\mu}\log\alpha$ and the definition of the extrinsic curvature $\nabla_{\alpha}n^{\mu}=-K\UD{\mu}{\alpha}$, and for the expansion of the last two terms we use the two identities:
\begin{align*}
V^{\alpha}\nabla_{\alpha}E^{\mu}&=V^{\alpha}D_{\alpha}E^{\mu}-K_{\alpha \beta}V^{\alpha}E^{\beta} n^{\mu}\\
 \\
n^{\nu}\nabla_{\nu}E^{\mu}&=\dfrac{1}{\alpha}\left( \mathcal{L}_{\alpha \vec{n}}E^{\mu}+E^{\nu}\nabla_{\nu}(\alpha n^{\mu})\right)=\dfrac{1}{\alpha} \mathcal{L}_{\alpha \vec{n}}E^{\mu} - E^{\nu}K\UD{\mu}{\nu}+E^{\nu}\partial_{\nu}(\log\alpha) \  n^{\mu}\, .
\end{align*}
We then re-write Eq.~\eqref{eq:PT_interm_1} split into two parts, the one proportional to $n^{\mu}$ and the other tangent to $\Sigma_t$ as
\begin{equation}
\left\{\begin{array}{l}
\dfrac{1}{\alpha} \mathcal{L}_{\alpha \vec{n}}C
+V^{\nu}\partial_{\nu}C + E^{\nu}\partial_{\nu}(\log\alpha) -K_{\nu \rho}V^{\nu}E^{\rho}=0\\
 \\
\dfrac{1}{\alpha} \mathcal{L}_{\alpha \vec{n}}E^{\mu} - E^{\nu}K\UD{\mu}{\nu} +V^{\nu}D_{\nu}E^{\mu}+ C\left(\gamma^{\mu \nu}D_{\nu}\log\alpha -K\UD{\mu}{\nu}V^{\nu}\right)  =0\, ,
\end{array}\right.
\label{eq:separated_PT}
\end{equation}
where both must vanish individually in order to satisfy the parallel transport condition~\eqref{eq:parallel_transport}. The last steps consist in expanding the Lie derivative
\begin{equation}
\mathcal{L}_{\alpha \vec{n}}=\dfrac{\partial}{\partial t}-\mathcal{L}_{ \vec{\beta}}
\end{equation}
and converting partial derivatives with respect to the time $t$ into total derivative via
\begin{equation}
\dfrac{\partial}{\partial t}=\dfrac{d }{d t}-\alpha V^j\partial_j + \beta ^j\partial_j \, .
\end{equation}
The final result for the $3+1$ parallel transport equation is
\begin{equation}
\left\{ \begin{array}{l}
\dfrac{1}{\alpha} \dfrac{d C}{d t} + E^{i}\partial_{i}\log\alpha -K_{i j}V^{i}E^{j}=0\\
\\
 \dfrac{1}{\alpha}\left(\dfrac{d E^{i}}{d t}+ E^j\partial_j \beta^i \right)+ \ ^{(3)}\Gamma^i_{\ j k} V^j E^{k} - K\UD{i}{ j}E^{j} +C\left( \gamma^{i j}D_{j}\log\alpha -K\UD{i}{j}V^{j}\right)  =0\, ,
\end{array} \right.
\label{eq:3+1PT}
\end{equation}
where we have only spatial indices $i, j=1,2,3$ since all the quantities lie on $\Sigma_t$.

The system of equations~\eqref{eq:3+1PT} has to be solved for each vector of the frame we choose. 
Following \cite{Grasso:2018mei}, we choose the semi-null frame (SNF) composed by the tetrad of vectors 
\begin{equation}
\phi\UD{\mu}{\boldsymbol{\alpha}}=(u^{\mu},\phi\UD{\mu}{\mathbf{1}},\phi\UD{\mu}{\mathbf{2}},\ell^{\mu})\, ,
\end{equation}
where $u^{\mu}$ is the matter four-velocity, $\ell^{\mu}$ is the tangent of the photon geodesic. The two vectors $\phi\UD{\mu}{\boldsymbol{A}}$ are  orthonormal to both $u^{\mu}$ and $\ell^{\mu}$, namely:
\begin{equation}
\left\{ \begin{array}{l}
%g_{\mu \nu} u^{\mu}u^{\nu}=-1\\
g_{\mu \nu} u^{\mu}\phi\UD{\mu}{\mathbf{A}}=0\\
g_{\mu \nu} \ell^{\mu}\phi\UD{\mu}{\mathbf{A}}=0\\
g_{\mu \nu} u^{\mu}\ell^{\nu}=Q\\
g_{\mu \nu} \phi\UD{\mu}{\mathbf{A}}\phi\UD{\mu}{\mathbf{B}}=\delta_{\mathbf{A} \mathbf{B}}\\
%g_{\mu \nu} \ell^{\mu}\ell^{\nu}=0\, ,
\end{array}\right.
\label{eq:SNF_def_rel}
\end{equation}
%\justify
with $Q$ a real number. Each vector of the SNF is then decomposed in $3+1$ form as
\begin{equation}
\phi^{\mu}_{\boldsymbol{\alpha}}=\Phi_{\boldsymbol{\alpha}}n^{\mu}+F^{\mu}_{\boldsymbol{\alpha}}\,
\label{eq:3+1vec}
\end{equation}
and parallelly propagated by solving Eq.~\eqref{eq:3+1PT} for its orthogonal and tangent components, i.e. $\Phi_{\boldsymbol{\alpha}} n^{\mu}=-n_{\sigma}\phi^{\sigma}_{\boldsymbol{\alpha}} n^{\mu}$ and $F^{\mu}_{\boldsymbol{\alpha}}=\gamma\UD{\mu}{\sigma} \phi^{\sigma}_{\boldsymbol{\alpha}}$. 

In {\tt BiGONLight} this is demanded to the function \texttt{PTransportedFrame[]}, which gives as output the components in~\eqref{eq:3+1vec} of the SNF parallel transported. The function \texttt{PTransportedFrame[]} uses \texttt{ParallelTransport[]} to obtain Eq.~\eqref{eq:3+1PT} for each vector of the frame and then solve them with a customised {\tt NDSolve[]} function.


\subsection{The optical tidal matrix and the GDE for the BGO}
\label{sec:W3+1}
So far the $3+1$ equations Eqs.~\eqref{eq:3+1_geodE}-\eqref{eq:3+1_geodV} and Eq.~\eqref{eq:3+1PT} we presented are valid for any type of geodesics and to parallelly transport any type of vectors along that geodesic. From now on, we will restrict the BGO formalism to the case of a SNF parallelly propagated along a null-like geodesic.
The equation for the BGO has then to be projected onto the SNF. The result is simply given by
\begin{equation}
\dfrac{d}{d \lambda} \mathcal{W}=\begin{pmatrix}
0 & \mathbb{1}\\
R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}} & 0
\end{pmatrix} \mathcal{W}\, ,
\label{eq:GDE_for_BGO_inframe}
\end{equation}
where the only formal difference with respect to Eq.~\eqref{eq:GDE_for_BGO} is that the covariant derivative along the photon geodesic $D/D\lambda$ reduces to the total derivative $d/d\lambda$ in the SNF.
In Eq.~\eqref{eq:GDE_for_BGO_inframe}, the optical tidal matrix is projected in the SNF and it is given by 
\beq
R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}=h^{\boldsymbol{\mu} \boldsymbol{\omega}}R_{\boldsymbol{\omega} \ell \ell \boldsymbol{\nu}}=\phi^{\rho \boldsymbol{\mu}}R_{\rho \alpha \beta \sigma} \ell^{\alpha}\ell^{\beta} \phi\UD{\sigma}{\boldsymbol{\nu}}
\label{eq:RinSNF}
\eeq
where the inverse of the induced metric of the frame
\begin{equation}
 h^{\boldsymbol{\mu} \boldsymbol{\omega}}=\begin{pmatrix}
0 & 0 & 0 & \frac{1}{Q} \\
0 & 1 & 0 & 0 \\
0 & 0 & 1 & 0 \\
\frac{1}{Q} & 0 & 0 & \frac{1}{Q^2}
\end{pmatrix}\, 
\label{eq:frame_matrix}
\end{equation}
is used to raise the indices.
In general $R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}$ is a $4 \times 4$ matrix with non trivial components. However, in the SNF it is easy to use the symmetries of the Riemann tensor to show that the components $R\UDDD{\boldsymbol{0}}{\ell}{\ell}{\boldsymbol{\nu}}=R\UDDD{\ell}{\ell}{\ell}{\boldsymbol{\nu}}$ and $R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{0}}=R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\ell}$ vanish.
Now, let us use Eq.~\eqref{eq:l_split} and Eq.~\eqref{eq:3+1vec} in Eq.~\eqref{eq:RinSNF} to write the optical tidal matrix in terms of $3+1$ quantities
\beq
\begin{array}{l}
R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}=(\Phi^{\boldsymbol{\mu}} n^{\rho} + F^{\boldsymbol{\mu} \rho})R_{\rho \alpha \beta \sigma}\mathcal{E}^2( n^{\alpha}n^{\beta}+n^{\alpha}V^{\beta}+V^{\alpha}n^{\beta}+V^{\alpha}V^{\beta})(\Phi_{\boldsymbol{\nu}} n^{\sigma} + F\UD{\sigma}{\boldsymbol{\nu}})
\end{array}
\eeq
After some tedious but straightforward calculations, we finally obtain
\begin{equation}
\begin{array}{lc}
 R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}= & \calE^2 h^{\boldsymbol{\mu} \boldsymbol{\rho}} \left[ \mathcal{R}_{\beta \alpha}\left(\Phi_{\boldsymbol{\rho}} F\UD{\beta}{\boldsymbol{\nu}}V^{\alpha}+\Phi_{\boldsymbol{\nu}} F\UD{\beta}{\boldsymbol{\rho}}V^{\alpha}-\Phi_{\boldsymbol{\rho}}\Phi_{\boldsymbol{\nu}} V^{\beta}V^{\alpha}-F\UD{\alpha}{\boldsymbol{\rho}}F\UD{\beta}{\boldsymbol{\nu}}\right)+\right.\\
 & \mathcal{C}_{\sigma \beta \alpha}\left(\Phi_{\boldsymbol{\rho}} F\UD{\sigma}{\boldsymbol{\nu}}V^{\alpha}V^{\beta}+\Phi_{\boldsymbol{\nu}} F\UD{\sigma}{\boldsymbol{\rho}}V^{\alpha}V^{\beta}-F\UD{\alpha}{\boldsymbol{\rho}} F\UD{\sigma}{\boldsymbol{\nu}}V^{\beta}-F\UD{\alpha}{\boldsymbol{\nu}} F\UD{\sigma}{\boldsymbol{\rho}}V^{\beta} \right)+\\
 & \left.\mathcal{G}_{\omega \alpha \beta \sigma} F\UD{\omega}{\boldsymbol{\rho}}V^{\alpha}V^{\beta} F\UD{\sigma}{\boldsymbol{\nu}}\right]
\end{array}
\label{eq:3+1_opt}
\end{equation}
where
\begin{align}
 \mathcal{G}_{\mu \alpha \beta \nu}&=R_{\rho \delta \theta \sigma}\gamma\UD{\rho}{\mu}\gamma\UD{\delta}{\alpha}\gamma\UD{\theta}{\beta}\gamma\UD{\sigma}{\nu}= {}^{(3)}R_{\mu \alpha \beta \nu}+ K_{\mu \beta} K_{\alpha \nu}-K_{\mu \nu} K_{\beta \alpha} \label{eq:Gauss}\\
%\nonumber  \\
 \mathcal{C}_{\mu \alpha \beta}&=R_{\rho \delta \theta \sigma}n^{\rho}\gamma\UD{\delta}{\alpha}\gamma\UD{\theta}{\beta}\gamma\UD{\sigma}{\mu}= D_{\alpha}K_{\mu \beta}-D_{\mu}K_{\alpha \beta} \label{eq:Codazzi}\\
% \nonumber \\
 \mathcal{R}_{\mu \nu}&=R_{\rho \delta \theta \sigma}n^{\rho}\gamma\UD{\delta}{\nu}\gamma\UD{\theta}{\mu}n^{\sigma}= \mathcal{L}_{\mathbf{n}}K_{\nu \alpha}+\dfrac{1}{\alpha}D_{\nu}D_{\alpha}\alpha+ K\UD{\rho}{\alpha}K_{\nu \rho}
\label{eq:Ricci}
\end{align}
are the Gauss relation, the Codazzi relation and the Ricci relation, respectively (see e.g. \cite{baumgarte2010numerical}).
In \texttt{BiGONLight}, the three functions \texttt{GaussRelation[]}, \texttt{CodazziRelation[]}, \texttt{RicciRelation[]} compute the relations in Eqs.~\eqref{eq:Gauss}-\eqref{eq:Ricci} and the function \texttt{OpticalTidalMatrix[]} collects all previous results together in order to obtain the optical tidal matrix $R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{ \boldsymbol{\nu}} / \calE^2$ in Eq.~\eqref{eq:3+1_opt} as output.
We now have the equation for the BGO, Eq.~\eqref{eq:GDE_for_BGO_inframe}, projected onto the SNF and written in terms of $3+1$ quantities. To solve it, it is easier to change the derivation variable from the affine parameter $\lambda$ to the time $t$ according to
\begin{equation}
\dfrac{d }{d \lambda}=\dfrac{d \, t}{d \lambda}\dfrac{d }{d t}=\frac{ \mathcal{E}}{\alpha}\dfrac{d }{d t} \, ,
\end{equation}
where we used the time component of the tangent vector in Eq.~\eqref{eq:l_split}, i.e. $\ell^0=d \, t / d \lambda= \mathcal{E} / \alpha$.
The GDE for the BGO, Eq.~\eqref{eq:GDE_for_BGO_inframe}, decouples in two systems of first-order ODE, one for $(\WXX, \WLX)$ and the other for $(\WXL, \WLL)$, computed separately using the function \texttt{BGOequations[]}:
\begin{equation}
\left\{\begin{array}{l}
\dfrac{d \, \WXX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d t}=\dfrac{\alpha}{ \mathcal{E}}\, \WLX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
 \\
\dfrac{d \, \WLX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d t}=\dfrac{\alpha}{ \mathcal{E}}\, R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\sigma}}\WXX{}\UD{\boldsymbol{\sigma}}{\boldsymbol{\nu}}
\end{array}\right.\ , \
\left\{\begin{array}{l}
\dfrac{d \, \WXL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d t}=\dfrac{\alpha}{ \mathcal{E}}\, \WLL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
 \\
\dfrac{d \, \WLL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}}{d t}=\dfrac{\alpha}{ \mathcal{E}}\, R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\sigma}}\WXL{}\UD{\boldsymbol{\sigma}}{\boldsymbol{\nu}}
\end{array}\right.
\label{eq:GDE_BGO_syst}
\end{equation}
with initial conditions:
\begin{equation}
\left\{\begin{array}{l}
\WXX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\left|_{\rm \calO}\right.=\delta\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
\WXL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\left|_{\rm \calO}\right.=0\\
\WLX{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\left|_{\rm \calO}\right.=0\\
\WLL{}\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\left|_{\rm \calO}\right.=\delta\UD{\boldsymbol{\mu}}{\boldsymbol{\nu}}\\
\end{array}\right.
\label{eq:GDE_BGO_IC}
\end{equation}
The systems in Eq.~\eqref{eq:GDE_BGO_syst} are solved separately in {\tt BiGONLight} by \texttt{SolveBGO[]}. Getting the BGO with the procedure just described is one important part of {\tt BiGONLight}. Let us recall that the only inputs required are the spacetime metric, the observer four-velocity components and the initial and ending points.

With initial conditions in Eq.~\eqref{eq:GDE_BGO_IC}, Eq.~\eqref{eq:GDE_BGO_syst} gives the BGO $\mathcal{W}(p_\lambda,\mathcal{O})$ integrated backward in time from the observer. Similarly, if the initial conditions were set at the source $\calS$, the solution of Eq.~\eqref{eq:GDE_BGO_syst} gives the BGO $\mathcal{W}(p_\lambda,\mathcal{S})$ integrated forward in time. However, in this case, to be used in observables calculation we need to implement the transformations Eqs.~\eqref{eq:WXX_inverse}-\eqref{eq:WLL_inverse} to obtain the backward integrated BGO $\mathcal{W}(p_\lambda,\mathcal{O})$ from $\mathcal{W}(p_\lambda,\mathcal{S})$.
These relations are coded in the section ``Forward to backward transformation for $\mathcal{W}$ operators'' of each sample notebook in the repository {\color{blue}{\tt {https://github.com/MicGrasso/\\ 
bigonlight.git}}}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The recipe to calculate observables with BiGONLight}
\MG{incollare da bigonlight}
\label{sec:obs}
The recipe to obtain optical observables using \texttt{BiGONLight} can be summarized as follows. One needs to:
\begin{enumerate}
\item specify the spacetime metric $g_{\mu \nu}$ and the source $\mathcal{S}$ and observer $\mathcal{O}$ kinematics, namely four-velocity $u^{\mu}$ and four-acceleration $w^{\mu}$. They can be given already in $3+1$ components or as 4D quantities and the functions {\tt ADM[]} and {\tt Vsplit[]} will do the splitting of $g_{\mu \nu}$, and $u^{\mu}$ and $w^{\mu}$ respectively;
\item set up the initial photon geodesic using {\tt Vsplit[]} for the null tangent $\ell^{\mu}$, which gives its $3+1$ components $\calE$ and $V^{i}$. Alternatively one can give $\calE$ and a vector $V^{i}$ that has to be assigned by specifying the spatial direction $V^2$ and $V^3$ and use {\tt InitialConditions[]} to get $V^1$ from the null condition; \\
\item obtain the geodesic equations Eq.~\eqref{eq:3+1_geodE} and Eq.~\eqref{eq:3+1_geodV} from {\tt GeodesicEquations[]} and {\tt EnergyEquations[]}, and then solve them with {\tt SolveGeodesic[]} and {\tt SolveEnergy[]}\footnote{For the purposes of our paper, we need to solve only photon geodesics. However, the code can be used to trace any type of geodesics, namely time-like and space-like also, by specifying the appropriate initial tangent vector in the $3+1$ splitting with {\tt Vsplit[]}.};\\
\item set up the initial conditions for the SNF according to Eq.~\eqref{eq:SNF_def_rel}, directly in $3+1$ components or using {\tt SNF[]}, which is specifically designed to compute the SNF in $3+1$. Then {\tt PTransportedFrame[]} will give the SNF parallel transported along the light ray;\\
\item compute separately $R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}$ projected into the SNF with {\tt OpticalTidalMatrix[]};\\
\item obtain the ODE system for the BGO in Eq.~\eqref{eq:GDE_BGO_syst} with {\tt BGOequations[]} and, together with the initial conditions in Eq.~\eqref{eq:GDE_BGO_IC}, solve it using {\tt SolveBGO[]} to finally find the full $\mathcal{W}$ matrix;\\
\end{enumerate}
Note that the components of the optical tidal matrix can have a very complicated expression, that may cause problems in solving the GDE \eqref{eq:GDE_BGO_syst}. This can be overcame by using an interpolated form of $R\UDDD{\boldsymbol{\mu}}{\ell}{\ell}{\boldsymbol{\nu}}$: the {\tt Mathematica Interpolation[]} function allows to use different methods and reach an excellent precision, see Sec.\ref{sec:test}.

Step (vi) is the starting point to compute the optical observables, which are all given by different combinations and/or functions of the $\mathcal{W}$ components. It is important to remark that all the observables in the BGO formalism are written in terms of $\mathcal{W}(\calS, \calO)$, namely the map computed from the observer to the source. As we already recalled, this is obtained directly by integrating the GDE backward in time. However in some cases, e.g. if the spacetime model comes from a numerical simulation, it may be more convenient to get the inverse BGO map $\mathcal{W}^{-1}(\calS, \calO)$ and then use the transformations Eqs.~\eqref{eq:WXX_inverse}-\eqref{eq:WLL_inverse} to obtain the $\mathcal{W}$ needed for the observables. 

In the next chapter we will use this recipe to test the accuracy of {\tt BiGONLight} in reproducing well-known results. The tests are conducted comparing a number of observables of interest in cosmology obtained by using two different method, i.e. with {\tt BiGONLight} and with the standard calculation present in the literature. The tests are conducted for several cosmological models and for each model we will consider four observables: the redshift $z$, the angular diameter distance $D_{\rm ang}$, the parallax distance $D_{\rm par}$ and the redshift drift $\zeta$, as they are defined in Sec.~\ref{sec:observables}.




%For different cosmological models we will compute a number of observables using {\tt BiGONLight} and we will compare them with the corresponding observable obtained by standard calculation. The observables that we will analyse are

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput


Here we list the four observables that we study in this paper. The redshift is simply given by its definition
\begin{equation}
1+z = \dfrac{\left(\ell_{\sigma } u^{\sigma}\right)|_{\cal S}}{\left(\ell_{\sigma } u^{\sigma}\right)|_{\cal O}}\, ,
\label{eq:redshift_def}
\end{equation}
where $\ell^{\sigma}$ is the tangent to the light ray, and $u^{\sigma}_{\mathcal{O}}$ and $u^{\sigma}_{\mathcal{S}}$ are the observer and source four-velocities. The same definition in $3+1$ splitting reads:
\begin{equation}
1+z=\frac{\mathcal{E}_{\mathcal{S}}}{\mathcal{E}_{\mathcal{O}}}\,\frac{1-\left(\gamma _{ij} V^i U^j\right)|_{\mathcal{S}}}{1-\left(\gamma _{ij} V^i U^j\right)|_{\mathcal{O}}}\left[\frac{1- \left(\gamma _{ij}U^i U^j\right)|_{\mathcal{S}}}{1-\left(\gamma _{ij}U^i U^j\right)|_{\mathcal{O}}}\right]^{\frac{1}{2}}\, .
\label{eq:redshift_def_3+1}
\end{equation}
The angular diameter distance is formally given by
\begin{equation}
D_{ang} = \left(\ell_{\sigma} u^{\sigma}\right)|_{\cal O} \left| \det \left(\WXL {}\UD{\bm A}{\bm B}\right) \right|^{\frac{1}{2}}\, ,
\label{eq:D_ang_BGO}
\end{equation}
where $\WXL {}\UD{\bm A}{\bm B}$ is the map between the physical size of the source and the angle subtended in the sky, as measured at the observer position, namely
\begin{equation}
\delta \theta^{\bm A}= {\left( \ell_{\sigma} u^{\sigma}\right)|_{\cal O}}^{-1} \left(\WXL {}\UD{\bm A}{\bm B}\right)^{-1} \delta x_{\mathcal{S}}^{\bm B}\, .
\end{equation}
Conversely, the parallax distance is related to the displacement of the observer position and the apparent angular shift of the source position, as measured from the observer
\begin{equation}
\delta \theta^{\bm A}= - {\left( \ell_{\sigma} u^{\sigma}\right)|_{\cal O}}^{-1} \left(\WXL {}\UD{\bm A}{\bm C}\right)^{-1} \WXX {}\UD{\bm C}{\bm B} \delta x_{\mathcal{O}}^{\bm B}\, .
\end{equation}
The expression for the parallax distance is
\begin{equation}
D_{par} =\left(\ell_{\sigma} u^{\sigma}\right)|_{\cal O} \frac{\left| \det \left(\WXL {}\UD{\bm A}{\bm B}\right) \right|^{\frac{1}{2}}}{\left| \det \left(\WXX {}\UD{\bm A}{\bm B}\right) \right|^{\frac{1}{2}}}\, .
\label{eq:D_par_BGO}
\end{equation}
The last observable that we consider in this paper is the redshift drift $\zeta$, given in terms of the BGO by, \cite{Julius}
\begin{equation}
\zeta\equiv\frac{\delta \log(1+z)}{\delta \tau_{\mathcal{O}}}= \Xi_{\rm Doppler}- \left( u_{\mathcal{O}} , \, \frac{u_{\mathcal{S}}}{1+z} \right) \boldsymbol{U} \begin{pmatrix} u_{\mathcal{O}}\\ \dfrac{u_{\mathcal{S}}}{1+z}\end{pmatrix}\, .
\label{eq:z_DRIFT_BGO}
\end{equation}
In the above expression $\tau_{\calO}$ is the proper time of the observer, the first term
\begin{equation}
\Xi_{\rm Doppler}=\left[\dfrac{1}{1+z}\dfrac{\left(\ell^{\bm \mu}w_{\bm \mu}\right)|_{\mathcal{S}}}{\left(\ell^{\bm \mu} u_{\bm \mu}\right)|_{\mathcal{S}}}-\dfrac{\left(\ell^{\bm \mu}w_{\bm \mu}\right)|_{\mathcal{O}}}{\left(\ell^{\bm \mu} u_{\bm \mu}\right)|_{\mathcal{O}}}\right]
\label{eq:doppler}
\end{equation}
represents the Doppler effect caused by the four-acceleration $w^{\sigma}$ of the observer and the source, and $U$ is an $8 \times 8$ matrix given by the following combinations of the BGO
\begin{equation}
U=\begin{pmatrix}
- \WXL^{-1}{}\UD{\bm \nu}{\bm \rho}\WXX{}\UD{\bm \rho}{\bm \sigma} & \WXL^{-1}{}\UD{\bm \nu}{\bm \rho} \\
\WLL{}\UD{\bm \mu}{\bm \nu}\WXL^{-1}{}\UD{\bm \nu}{\bm \rho}\WXX{}\UD{\bm \rho}{\bm \sigma}-\WLX{}\UD{\bm \mu}{\bm \sigma} & - \WLL{}\UD{\bm \mu}{\bm \nu} \WXL^{-1}{}\UD{\bm \nu}{\bm \rho}
\end{pmatrix} \, .
\end{equation}
Let us notice that, even if the BGO formalism is independent of the specific choice of the frame used, the observables are dependent on this choice, as evident by the explicit dependence on $u^{\mu}_{\mathcal{O}}$, $u^{\mu}_{\mathcal{S}}$, $w^{\mu}_{\mathcal{O}}$ and $w^{\mu}_{\mathcal{S}}$ in Eqs. \eqref{eq:D_ang_BGO}-\eqref{eq:doppler}. Indeed, it is possible to transform locally between two different frames using an appropriate Lorentz transformation, but this modifies the observables introducing special relativistic effects like Doppler effect or aberration.

The reader can find the derivation of the Eqs.~\eqref{eq:D_ang_BGO}-\eqref{eq:z_DRIFT_BGO} in \cite{Grasso:2018mei, Korzynski:2018, Julius}). All the expressions in Eqs.~\eqref{eq:D_ang_BGO}, \eqref{eq:D_par_BGO} and \eqref{eq:z_DRIFT_BGO} are new with respect to the standard approach, in the sense that these observables are expressed within a new, unified framework. However, while for $D_{\rm ang}$ and $D_{\rm par}$ there already exist analogous formulas, where instead of the BGO we have the magnification and the parallax matrix (see \cite{Korzynski:2019oal} for the comparison), it did not exist a general formula for the redshift drift: Eq.~\eqref{eq:z_DRIFT_BGO} looks the same for every spacetime model under consideration. Instead, in the standard approach the redshift drift is calculated by taking the derivative with respect to the time coordinate of the definition of the redshift, and this depends on the specific form of the metric tensor and null-geodesic, the latter depending in turns on the symmetries that one gives to the initial conditions. This means that the equations to get the redshift drift in the standard approach look different for each specific model and/or configuration of the light rays\footnote{To be more precise, Eq.~\eqref{eq:z_drift_FLRW} is valid for the FLRW model only as well as Eq.~\eqref{eq:z_drift_Szekeres} is valid for the Szekeres model and geodesics along the symmetry axis only. Instead, Eq.~\eqref{eq:z_DRIFT_BGO} looks the same in both cases.}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

PRENDERE SPUNTO?
Theory of General Relativity presented in chapter $2$ provide a description of gravitation, as due to the geometry of spacetime structure, where all physically possible spacetimes correspond to solutions of Einstein's field equation (\ref{EinsteinField_eq}). So, by solving the Einstein's equation for a specific metric tensor, we are able to obtain complete predictions for that particular gravitational system. Unfortunately, Einstein's field equation represents a complicated coupled system of nonlinear partial differential equations,  so it is very hard to find a solution analytically. 

Due to these difficulties, historically two different approaches have arisen trying to find a solution of the Einstein's equation: the first-one is the \emph{perturbative approach} and the second-one is the \emph{numerical approach}.

\section{The Perturbative Approach}
The known solutions, such as the FLRW (\ref{FLRW_eq}) and the Schwarzschild (\ref{Schwarzschildmet_eq}) metrics discussed in the previous chapter, tell us a great deal about cosmology and gravitational fields. However these solutions have a high degree of symmetry\footnote{This is a necessary condition if we want to resolve the Einstein's equation. The high degree of symmetry of the metrics allow us to reduce in some way the differential equations system.} and thus it is difficult to compare them with real systems. For example, the FLRW metric alone can not explain how small inhomogeneities in the matter distribution evolve over time or we can define what happens if we have two black holes one close to other using the simple Schwarzschild metric. 

However, if the deviation from a known exact solution $g_{\mu \nu}$ is small, it makes sense to look for an approximate solution $ \tilde{g}_{\mu \nu}=g_{\mu \nu}+h_{\mu \nu}$ linearizing Einstein's equation in the perturbation $h_{\mu \nu}$. This is exactly the technique used by Einstein one hundred years ago to find the existance of a gravitational radiation, that was recently observed experimentaly by the LIGO and VIRGO interferometers.

In general the perturbative approach can be summarize with the following procedure: let us consider the Einstein's field equation for a perturbed metric $\tilde{g}_{\mu \nu}$ in vacuum. $\tilde{g}$ describe a spacetime metric that differs from a known metric $g_{\mu \nu}$ linearly. If the deviation from the exact metric is small, we can suppose that the new tensor $\tilde{g}$:
\begin{enumerate}
\item it depends differentiably on a parameter $\lambda$,
\item it is true that $\tilde{g}(\lambda)|_{\lambda=0}=g$
\end{enumerate}

With the previous conditions, small $\lambda$ corresponds to small deviations from $g$ and knowing $\tilde{g}(\lambda)$ we can find an exact solution of the Einstein's field equation. Writing the void Einstein's equation in terms of $\tilde{g}(\lambda)$ as
$$\mathcal{E}[\tilde{g}(\lambda)]=0$$
and differentiating it with respect to $\lambda$ we can find that
\begin{equation}
\dfrac{d}{d \lambda} \left( \mathcal{E}[\tilde{g}(\lambda)] \right) |_{\lambda=0}=0
\label{linear_eq}
\end{equation}


Is easy to see that the last equation (\ref{linear_eq}) is linear in $\frac{d \tilde{g}}{d \lambda}|_{\lambda=0} \equiv h $ and thus we can try to solve it respect to $\gamma$, instead of the original Einstein's equation.
Solving equation (\ref{linear_eq}), finally we have that $\tilde{g}(\lambda)=g+\lambda h$ provide a good approximation to the real metric for sufficient small $\lambda$.

To derive the equation\footnote{A complete and rigorous derivation of the perturbed approach goes beyond our purposes but a more rigorous derivation can be found in reference \cite{wald2010general, misner1973gravitation}} (\ref{linear_eq}) we first need to understand how to compute the Ricci tensor $R_{\mu \nu}(\lambda)$, for the metric $\tilde{g}(\lambda)$, in terms of quantities related to the unperturbed metric $g_{\mu \nu}$. Then we can differentiate this expression with respect to $\lambda$ and imposing that $\lambda=0$ we find the searched equation.
Denoting with $\tilde{\nabla}_{\mu}$ the derivative operator associated with $\tilde{g}(\lambda)_{\mu \nu}$, and $\nabla_{\mu}$ the derivative operator associated with $g_{\mu \nu}$, the difference between the two derivative operators is determined by the quantity $C^{\sigma}_{\mu \nu}(\lambda)$ define\footnote{This is similar to the Christoffel symbols because it express the connection between the two metrics $\tilde{g}_{\mu \nu }(\lambda)$ and $\tilde{g}_{\mu \nu }(0)=g_{\mu \nu }$} as
$$C^{\sigma}_{\mu \nu}(\lambda)=\dfrac{1}{2}\tilde{g}^{\sigma \delta}(\lambda)(\nabla_{\mu}\tilde{g}_{\nu \delta }(\lambda)+\nabla_{\nu}\tilde{g}_{\mu \delta}(\lambda)-\nabla_{\delta}\tilde{g}_{\mu \nu }(\lambda))$$ 
The perturbed Ricci tensor $\tilde{R}_{\mu \nu}$ is then 
\begin{equation}
\tilde{R}_{\mu \nu}= 2[ \nabla_{\rho}C^{\rho}_{\mu \nu}-\nabla_{\mu}C^{\rho}_{\rho \nu}  + C^{\sigma}_{\nu \mu}C^{\rho}_{\rho \sigma}-C^{\sigma}_{\nu \rho}C^{\rho}_{\mu \sigma}]
\label{riccipert_eq}
\end{equation}
where we have used the Einstein's field equation in vacuum $R_{\mu \nu}=0$ for $g_{\mu \nu}$ exact and known solution.
we are seeking the equivalent equation to (\ref{linear_eq}), so we have to differentiate (\ref{riccipert_eq}) respect to $\lambda$. Thus we obtain
\begin{equation}
\dot{\tilde{R}}_{\mu \nu}=2[ \nabla_{\rho}\dot{C}^{\rho}_{\mu \nu}-\nabla_{\mu}\dot{C}^{\rho}_{\rho \nu}]
\label{dotriccipert_eq}
\end{equation}
where $\dot{C}^{\rho}_{\mu \nu}=\frac{d C^{\rho}_{\mu \nu}}{d \lambda}|_{\lambda}= \frac{1}{2}g^{\rho \sigma}(\nabla_{\mu} h_{\nu \sigma}+\nabla_{\nu} h_{\mu \sigma}-\nabla_{\sigma} h_{\mu \nu})$. Substituting this in equation (\ref{dotriccipert_eq}) we finally have 

\begin{equation}
\nabla_{\mu} \nabla_{\nu} h +\nabla^{\rho} \nabla_{\rho}h_{\mu \nu} - \nabla^{\rho} \nabla_{\nu} h_{\mu \rho}+ \nabla^{\rho} \nabla_{\mu} h_{\nu \rho}=0
\label{linearfin_eq}
\end{equation}

where $h=h^{\mu}_{\mu}=g^{\mu \nu}h_{\mu \nu}$. This is a \emph{linear} system of second order differential equations in the perturbation tensor $h_{\mu \nu}$ and thus it is simpler\footnote{We can simplify further this equation noting that exist a gauge freedom in the choice of  the perturbation $h$. Choosing the transverse traceless gauge $\nabla^{\mu}h_{\mu \nu}=0$ and $h=h^{\mu}_{\mu}=g^{\mu \nu}h_{\mu \nu}=0$ the previous equation becomes
$$\nabla^{\rho}\nabla_{\rho} h_{\mu \nu} - 2R^{\rho \ \ \sigma}_{\ \mu \nu }h_{\rho \sigma}=0$$} than the original Einstein's field equation in the perturbed metric $\tilde{g}_{\mu \nu}$.

Although perturbation theory provides a powerful tool for facing the problems related with the Einstein field equation, the procedure is not painless. In fact it is very difficult to estimate the error involved in replacing $\tilde{g}$ by its simplified linear expression $g+\lambda h$ or, in general, we have no way of verifying if there are spurious solutions of equation (\ref{linearfin_eq}). 

Perturbation theory plays an important role in the study of structure formations. As we saw in Chapter $2$, the Standard Model of Cosmology ($\Lambda CDM$) is based on the metric FLRW that describes a homogeneous and isotropic Universe. So, the question how from a homogeneous and isotropic universe, would be possible to develop local structures like galaxies (see discussion in Chapter $1$) arises. A road to find a solution outlined when we was able to see that the cosmic microwave background radiation (CMB) (which initially appeared homogeneous and isotropic) showed small differences in temperature. This fact suggested that the structures we observe today must have originated from primordial inhomogeneities or, as they are poetically called, `` the seeds of galaxies '' Fig. \ref{CMB_fig}.
\begin{figure}
\centering
\includegraphics[scale=0.6]{figure/CMB.png} 
\caption{The Cosmic Microwave Background radiation (CMB) was observed by Penzias and Wilson in $1964$ (figure A). Some notable experiments in the list are COBE, which first detected the temperature anisotropies of the CMB, and showed that it had a black body spectrum. DASI, which first detected the polarization signal. WMAP and the \emph{Planck spacecraft} (figure D, image credit: ESA), which have produced the highest resolution all-sky map. Figure B show the polarization of the signal due to the Earth rotation, while in figure C the polarization is subtracted but we can distinguish a concentration of the radiation due to the electromagnetic emission from the galactic disc.(image credit: NASA)}
\label{CMB_fig}
\end{figure}


\section{The Numerical Approach}

Unlike the perturbation method, the numerical approach tries to find an exact solution to the Einstein's equation using numerical methods to calculate the differential equations involved. The numerical approach is designed to solve exactly the gravitational field equation deriving a metric that was not initially known\footnote{Unlike perturbative approach, which begins with a metric already known and adds a perturbation.}. To achieve this purpose, the numerical formulation must be implemented by powerful computers capable of performing a many  operations in a short time.
Thanks to the rapid development of modern computers capability, numerical simulations play a major role in modern cosmology and astrophysics\footnote{Nowadays, supercomputers are capable of following the evolution of billions to trillions of particles in cosmological volumes; however, upcoming observational missions place higher and higher demands on the realism required by cosmological codes.}.

 The field that applies computational-science techniques to the relativistic Universe is called \emph{Numerical Relativity}. The amount of detail required to simulate the large-scale Universe is formidable: the main purpose of numerical relativists is to tame this task and build more and more realism into the simulations. 
 Numerical relativity is applied to many areas, such as cosmological models, critical phenomena, coalescence of black holes and neutron stars, etc. In any of these cases, Einstein's equations has to be rewrite like a Cauchy problem, splitting the spacetime into three dimensional space on one hand and in time on the other hand.
There exist several different approaches to set the Einstein field equations like a Cauchy problem; here we will present the \emph{$3+1$ formalism}, which allow us to split the spacetime into a three dimensional space on one hand and time on the other.  
 
Let us consider a spacetime $M$ with metric $g_{\mu \nu}$ and let us assume that the spacetime $M$ can be foliated into a family of non-intersecting spacelike $3-$surfaces $\Sigma_t$, which arise as the level surfaces of a scalar function $t$ that can be interpreted as a \emph{global time function} (\ref{gaugefig}). Such a foliation of spacetime into spatial hypersurfaces is also called \emph{synchronization}.
\begin{figure}[htbp]
  \centering
  \includegraphics[scale=0.4]{figure/slices.png}%
  \caption{Two adjacent  spacelike hipersurfaces. The figure show the definitions of the lapse function $\alpha$ and the shift vector $\beta^i$. It is clear that, setting a coordinate base on the hipersurfaces, the gauge functions are closely depended by that choice.}
  \label{gaugefig}
\end{figure}

The geometry of these hypersurfaces could be described by introducing the following quantities:
\begin{enumerate}
\item the three dimensional metric $\gamma_{ij}$ that measures proper distances within the hypersurfaces $$dl^2=\gamma_{ij}dx^i dx^j$$
\item the \emph{lapse function} of proper time $d\tau$ between two adjacent hypersurfaces measured by normal observers to the hypersurfaces (the so-called \emph{normal or Eulerian observers}): $d\tau= \alpha(t,\vec{x}) dt$
\item The relative velocity between the Eulerian observers and the lines of constant spatial coordinates, called \emph{shift vector} $\beta(t, \vec{x}) $: $x^i_{t+dt}=x^i_t- \beta(t, x^j) dt$
\end{enumerate}

Using these quantities, the usual line element $ds^2=g_{\mu \nu}dx^{\mu}dx^{\nu}$ take the following form

$$ds^2=(-\alpha^2+\beta_i \beta^i)dt^2+2 \beta_i dt dx^i + \gamma_{ij}dx^i dx^j$$

Notice that both the way in which we foliate the spacetime and also the way in which the spatial coordinate propagates from a hypersurface to another are not uniquely defined. This because the lapse functions $\alpha$ and shift vector $\beta^i$ are freely specifiable functions that carry information about the choice of coordinate system. For this reason  $\alpha$ and $\beta^i$ are known as the \emph{gauge functions}.

We can use the normal vector $n^{\mu}$ to the spatial hypersurfaces to define the gauge functions and the three dimensional metric $\gamma_{ij}$ in a more formal way. Let us start with the three dimensional metric $\gamma_{ij}$, which is simply defined as the metric induced on each hypersurface $\Sigma$. We can define the projection tensor 
$$P^{\mu}_{\nu}=\delta^{\mu}_{\nu} + n^{\mu} n_{\nu}$$
as the tensor that project an arbitrary spacetime vectors $v$ into the space of vectors tangent to the surface\footnote{Applying $P^{\mu}_{\nu}$ on the normal vector $n^{\nu}$ we simply get $$P^{\mu}_{\nu} n^{\nu}=\delta^{\mu}_{\nu} n^{\nu} + n^{\mu} n_{\nu} n^{\nu}=$$
$$=n^{\mu} + n^{\mu} (\vec{n} \cdot \vec{n})=n^{\mu} - n^{\mu} =0$$}.

 The corresponding tensor with one index lowered define the \emph{spatial metric} on the hypersurface 
$$\gamma_{\mu \nu}=g_{\mu \nu} + n_{\mu} n_{\nu}$$

Notice that, written in this way, it is a full four-dimensional tensor so the adjective ``spatial'' is incorrect. However in an adapted reference frame, the only non-zero components of this tensor are the components of the metric tensor in the surface $\gamma_{ij}$.

Let us consider now the lapse function $\alpha$: we can redefine it using the global time function as $\alpha=(- \nabla t \cdot \nabla t)^{-\frac{1}{2}}$. The unit normal vector can be defined in terms of $t$ and $\alpha$ as
\begin{equation}
n^{\mu}=- \alpha \nabla^{\mu} t
\label{alpha}
\end{equation}
where the minus sign is there to guarantee that $\vec{n}$ is future pointing.

Also for the shift vector we start considering the previous definition 
$$x^i_{t+dt}=x^i_t- \beta^i dt$$
Using the previous definition for $n^{\mu}$, we have

\begin{equation}
\beta^i=- \alpha (\vec{n} \cdot \nabla x^{i})=- \alpha (n^j \nabla_j x^{i})
\label{beta}
\end{equation}

The $\beta^i$ can be interpreted as the scalar components of a $4$-vector $\beta^{\mu}=(0, \beta^i)$, which is orthogonal to $\vec{n}$.

Using the quantities previously defined, we can construct a \emph{time vector} $\vec{t}$
\begin{equation}
t^{\mu}=\alpha n^{\mu} + \beta^{\mu}
\label{ti}
\end{equation}  
which is the tangent vector to the lines of constant spatial coordinates.
It is trivial to observe\footnote{From (\ref{ti}) we have $t^{\mu}n_{\mu}= \alpha n^{\mu} n_{\mu} + \beta^{\mu} n_{\mu}= - \alpha$. This, using the defining equation of $n^{\mu}$ (\ref{alpha}), imply that $\vec{t}$ satisfy the condition $t^{\mu} \nabla_{\mu}t=1$. We then find that the shift is nothing more than the projection of $\vec{t}$ onto the spatial hypersurface $\beta_{\mu}=\gamma_{\mu \nu}t^{\nu}$.} that the shift $\beta^i$ and the lapse $\alpha$ can be introduced in a completely coordinate-independent way 
$$t^{\mu}n_{\mu}= - \alpha \ \ \ \ \ \ \ \ \ \ \ \beta_{\mu}=\gamma_{\mu \nu}t^{\nu}$$
choosing a vector field $t^{\mu}$ which satisfy the condition $t^{\mu} \nabla_{\mu}t=1$. 
Notice that we have not a restriction on the type of the vector field $t^{\mu}$, so it could be a time-like, space-like or null-like vector field: a space-like $t^{\mu}$ vector field would correspond to a superluminal motion of the coordinate, but it is only an effect due to that particular choice of coordinate system and the coordinates can be chosen freely.

Now let us observe that the curvature of spacetime manifests itself on the hypersurfaces $\Sigma_i$ as the changing of the normal vector orientation when it is parallel transported. So the covariant derivative (along the surface) of the unit normal vector $\vec{n}$ projected onto the surface is a measure of how much the orientation of the surface changes from place to place, i.e. a measure of its curvature as seen from the outside. Thus we can define the \emph{Extrinsic Curvature} $K_{\mu \nu}$ as the tensor
\begin{equation}
K_{\mu \nu}=-P^{\alpha}_{\mu} \nabla_{\alpha} n_{\nu}=-(\nabla_{\mu} n_{\nu}+n^{\mu}n_{\alpha}\nabla_{\alpha} n_{\nu})
\label{Defextrinsic_eq}
\end{equation}

The extrinsic curvature tensor $K_{\mu \nu}$ is clearly a purely spatial tensor, in fact it only has components tangent to the hypersurface $n^{\mu} K_{\mu \nu}=n^{\nu} K_{\mu \nu}=0$, implying that $K^{00}=K^{0i}=0$. Thus we can consider only the spatial components of the tensor and we can see that it is a symmetric%\footnote{The symmetry of the extrinsic curvature tensor is not trivial: the ``spatiality'' of $K_{\mu \nu}$ is  guaranteed by the projection of $\nabla_{\mu} n_{\nu}$ on the hypersurface. This imply that the gradient of the normal vector is necessarily orthogonal to it  $n_{\mu}\nabla_{\nu} n_{\mu}=0$. However, in general the $\nabla_{\mu} n_{\nu}$ is not symmetric, so we have that $n_{\mu}\nabla_{\mu} n_{\nu} \neq 0$, unless the normal lines are geodesic. The reason for this is that $n^{\mu}$ is a unitary vector and thus in general is not equal to the gradient of the time function $t$, except when the lapse is unity (see Eq. \ref{alpha}). What we want to proof is that once we project onto the hypersurface, it turns out that $P^{\alpha}_{\mu} \nabla_{\alpha}n_{\nu}$ is indeed symmetric (so $K_{\mu \nu}$). In order to see this, consider the congruence of timelike geodesics orthogonal to the hypersurface $\Sigma$ with unit tangent vector $\vec{\xi}$. Near $\Sigma$ let us consider a new foliation of spacetime given by a time function $\tilde{t}$ such that $\xi_{\mu}=\nabla_{\mu}\tilde{t}$. Since $\xi_{\mu}$ is the gradient of a scalar function, then we will have $\nabla_{\mu}\xi_{\nu}=\nabla_{\nu}\xi_{\mu}$. Moreover, $\nabla_{\mu}\xi_{\nu}$ will be purely spatial without the need to project it since $\vec{\xi}$ is tangent to the timelike geodesics. Now, the vector field $\vec{n}$ will generally not coincide with $\vec{\xi}$ outside of $\Sigma$, but it will coincide within, so its derivatives along directions tangential to the hypersurface must be equal to those of $\vec{\xi}$ that is $$P^{\alpha}_{\mu}\nabla_{\alpha} n_{\nu}=P^{\alpha}_{\mu}\nabla_{\alpha} \xi_{\nu}=\nabla_{\mu} \xi_{\nu}=\nabla_{\nu} \xi_{\mu}=P^{\alpha}_{\nu}\nabla_{\alpha} \xi_{\mu}=P^{\alpha}_{\nu}\nabla_{\alpha} n_{\mu}$$} 
 tensor $K_{\mu \nu}=K_{\nu \mu}$. 
 
As we can see from equation (\ref{Defextrinsic_eq}), we have defined the extrinsic curvature as the parallel transport of the normal vector projected onto the hypersurface. However, it easy to see that $K_{\mu \nu}$ can be defined as the Lie derivative of the spatial metric along the normal direction
\begin{equation}
K_{\mu \nu}= -\dfrac{1}{2} \mathcal{L}_{\vec{n}}\gamma_{\mu \nu}
\label{Klie_eq}
\end{equation}
This came from the definition of the Lie derivative

$$\mathcal{L}_{\vec{n}}\gamma_{\mu \nu} = n^{\alpha} \nabla_{\alpha}\gamma_{\mu \nu} +\gamma_{\mu \alpha} \nabla_{\nu} n^{\alpha} + \gamma_{\nu \alpha} \nabla_{\mu} n^{\alpha}$$
$$=n^{\alpha} \nabla_{\alpha}(n_{\mu}n_{\nu}) +g_{\mu \alpha} \nabla_{\nu} n^{\alpha} + g_{\nu \alpha} \nabla_{\mu} n^{\alpha}$$
$$=n^{\alpha}n_{\mu} \nabla_{\alpha}n_{\nu} + n^{\alpha}n_{\nu} \nabla_{\alpha}n_{\mu} + \nabla_{\nu} n_{\mu} +  \nabla_{\mu} n^{\nu}$$
$$=(\gamma^{\alpha}_{\mu}-g^{\alpha}_{\mu}) \nabla_{\alpha}n_{\nu} + (\gamma^{\alpha}_{\nu}-g^{\alpha}_{\nu}) \nabla_{\alpha}n_{\mu} + \nabla_{\nu} n_{\mu} +  \nabla_{\mu} n^{\nu}$$
$$=\gamma^{\alpha}_{\mu}\nabla_{\alpha}n_{\nu} + \gamma^{\alpha}_{\nu}\nabla_{\alpha}n_{\mu}=-2K_{\mu \nu}$$

We must remember that our purpose is to write the Einstein's equation as a Cauchy problem. Therefore, let us try to use the quantities previously defined to write the gravitational field equation (\ref{EinsteinField_eq}) as a set of dynamical equations and boundary conditions.

In order to achieve this goal, let us see that, since $\vec{n}$ is normal to the hypersurface, it turns out that for any scalar function $\phi$ we have 
$$\mathcal{L}_{\vec{n}}\gamma_{\mu \nu}=\dfrac{1}{\phi}\mathcal{L}_{\phi\vec{n}}\gamma_{\mu \nu}$$  
Using this and taking as scalar function the lapse function $\alpha$, equation (\ref{Klie_eq}) become
$$K_{\mu \nu}=-\dfrac{1}{2 \alpha}\mathcal{L}_{\alpha\vec{n}}\gamma_{\mu \nu}=-\dfrac{1}{2 \alpha}(\mathcal{L}_{\vec{t}}-\mathcal{L}_{\vec{\beta}})\gamma_{\mu \nu}$$ 
where we used (\ref{ti}). 
Taking only the spatial components and noticing that in the adapted coordinate system $\mathcal{L}_{\vec{t}}= \partial_{t}$, we finally find
$$\partial_{t}\gamma_{i j} -\mathcal{L}_{\vec{\beta}} \gamma_{i j}=-2 \alpha K_{i j}$$
\begin{equation}
\implies \ \ \ \partial_{t}\gamma_{i j} =-2 \alpha K_{i j} + D_i \beta_j +  D_j \beta_i
\label{timegamma_eq}
\end{equation}
where $D_i$ is the \emph{$3$-dimensional covariant derivative}, which is defined as the projection of the $4$-dimensional covariant derivative $D_{\mu}= P^{\alpha}_{\mu} \nabla_{\alpha}$.

Equation (\ref{timegamma_eq}) is the evolution equation for the three-metric $\gamma_{ij}$: in order to close the system, we need the evolution equation for the extrinsic curvature. In order to find this equation, we need to rewrite the Einstein's equation in the $3+1$ formalism considering contractions of (\ref{EinsteinField_eq}) with the normal vector $\vec{n}$ and the projector tensor $P^{\mu}_{\nu}$. However, a complete and rigorous derivation of these quantities is beyond the scope of this thesis, so we will limit to state the final results (see  \cite{wald2010general} for more rigorous derivations).
The following are the fundamental relations on which rely all the derivation:
\begin{enumerate}
\item \emph{The Gauss-Codazzi equation}: \begin{equation}
P^{\mu}_{\alpha}P^{\nu}_{\beta}P^{\rho}_{\gamma}P^{\sigma}_{\delta}R_{\mu \nu \rho \sigma}=^{(3)}R_{\alpha \beta \gamma \delta}+K_{\alpha \gamma}K_{\beta \delta}-K_{\alpha \delta}K_{\beta \gamma}
\label{GaussCodaz_eq}
\end{equation}
where $^{(3)}R_{\alpha \beta \gamma \delta}$ is the \emph{intrinsic} $3$-dimensional Riemann tensor of the hypersurfice;
\item \emph{The Gauss-Mainardi equation}:\begin{equation}
P^{\mu}_{\alpha}P^{\nu}_{\beta}P^{\rho}_{\gamma}n^{\sigma}R_{\mu \nu \rho \sigma}=D_{\beta}K_{\alpha \gamma}-D_{\alpha}K_{\beta \gamma}
\label{GaussMainardi_eq}
\end{equation} 
\item The projection of the Riemann tensor contracted twice with $\vec{n}$:\begin{equation}
P^{\mu}_{\beta}P^{\nu}_{\gamma}n^{\rho}n^{\sigma}R_{\mu \nu \rho \sigma}=\mathcal{L}_{\vec{n}}K_{\beta \gamma}+K_{\beta \rho}K^{\rho}_{\gamma}+ \dfrac{1}{\alpha}D_{\beta}D_{\gamma} \alpha
\end{equation}
\end{enumerate}

Let us start considering the last relation, noticing that it involves both the lapse function $\alpha$ and the Lie derivative of the extrinsic curvature along the normal direction, which clearly correspond to evolution in time. Using equation (\ref{GaussCodaz_eq}), we find
$$\mathcal{L}_{\vec{t}}K_{\mu \nu}-\mathcal{L}_{\vec{\beta}}K_{\mu \nu}=-D_{\mu}D_{\nu}\alpha+\alpha(P^{\rho}_{\mu}P^{\sigma}_{\nu}R_{\rho \sigma}+^{(3)}R_{\mu \nu}+KK_{\mu \nu}-2K_{\mu \lambda}K^{\lambda}_{\nu})$$
Projecting the Einstein's equation and substituting into this (concentrating on the spatial components), we finally find
$$\partial_{t}K_{i j}-\mathcal{L}_{\vec{\beta}}K_{i j}=-D_{i}D_{j}\alpha+\alpha(^{(3)}R_{i j}+KK_{i j}-2K_{il}K^{l}_{j})+ 4\pi \alpha[\gamma_{ij}(S-\rho)-2S_{ij}]$$
where $S$ is the trace of the spatial stress tensor $S_{\mu \nu}=P^{\alpha}_{\mu}P^{\beta}_{\nu}T_{\alpha \beta}$, while $\rho=n^{\mu}n^{\nu}T_{\mu \nu}$. Expanding the Lie derivative along the shift vector we finally find:
\begin{equation}
\partial_{t}K_{i j}=\beta^{l} \partial_{l}K_{i j}+K_{li} \partial_{j}\beta^{l} + K_{lj} \partial_{i}\beta^{l} -D_{i}D_{j}\alpha+\alpha(^{(3)}R_{i j}+KK_{i j}-2K_{il}K^{l}_{j})+ 4\pi \alpha[\gamma_{ij}(S-\rho)-2S_{ij}]
\label{timeK_eq}
\end{equation}

These equations give the dynamical equations of the six independent components\footnote{Using the symmetry property of the extrinsic curvature tensor, it is easy to see that $K_{i j}$ has only six independent components.} of the extrinsic curvature $K_{ij}$. Summing this components to those of the space metric $\gamma_{ij}$ ($\gamma_{ij}$ is represented as a symmetric $3 \times 3$ matrix, thus it has six independent components), we have $12$ independent components. Since the Einstein equations can be written as a system of $20$ first-order differential equations,  we still need $8$ independent components to close the system. 
A help comes from the Gauss-Codazzi (\ref{GaussCodaz_eq}) and the Gauss-Mainardi (\ref{GaussMainardi_eq}) equations: we can combine the projected Einstein's field equations
$$P^{\mu \rho}P^{\nu \sigma}R_{\mu \nu \rho \sigma}=(g^{\mu \rho}+n^{\mu}n^{\rho})(g^{\nu \sigma}+n^{\nu}n^{\sigma})R_{\mu \nu \rho \sigma}$$
$$=R+2n^{\mu}n^{\nu}R_{\mu \nu}$$
$$=2 n^{\mu}n^{\nu}G_{\mu \nu}=2 n^{\mu}n^{\nu}(8 \pi T_{\mu \nu}) $$

with the Gauss-Codazzi relations $P^{\rho \mu}P^{\sigma \nu}R_{\rho \sigma \mu \nu}= ^{(3)}R+K^{2}-K_{\mu \nu}K^{\mu \nu}$, we then find
$$^{(3)}R+K^{2}-K_{\mu \nu}K^{\mu \nu}=P^{\rho \mu}P^{\sigma \nu}R_{\rho \sigma \mu \nu}=2 n^{\mu}n^{\nu}G_{\mu \nu}=16 \pi \rho$$
Summing up, through the Einstein equation, we have found
\begin{equation}
^{(3)}R+K^{2}-K_{\mu \nu}K^{\mu \nu}=16 \pi \rho
\label{const1_eq}
\end{equation}  
where $\rho$ corresponds to the local energy density.

Consider now the mixed contraction of the Einstein tensor
$$P^{\lambda \mu}n^{\nu}G_{\mu \nu}=P^{\lambda \mu}n^{\nu}R_{\mu \nu}$$
Using this result, the Gauss-Mainardi equations (\ref{GaussMainardi_eq}) then become
$$\gamma^{\lambda \mu}n^{\nu}G_{\mu \nu}=D^{\lambda}K-D_{\mu}K^{\lambda \mu}$$

Through the Einstein field equation, we find
\begin{equation}
D_{\mu}(K^{\lambda \mu}-\gamma^{\lambda \mu} K)=8 \pi j^{\lambda}
\label{const2_eq}
\end{equation}
where we have defined $j^{\mu}=-P^{\mu \nu}n^{\rho}T_{\nu \rho}$, which corresponds to the momentum density.

Notice that these four equations involve no explicit time derivatives, so they are not evolution equations but rather constraints that must be satisfied at all times. Moreover they are also completely independent of the gauge functions $\alpha$ and $\beta^{i}$, and this means that equations (\ref{const1_eq}) and (\ref{const2_eq}) are constraints that refer purely to a given hypersurface.

The presented $3+1$ decomposition of the space-time is known as the \emph{York formulation of the ADM Evolution Equations} (Arnowitt-Deser-Misner equations) \cite{BrumanteShapiro}:
\begin{equation}
\partial_{t} \gamma_{i j}=-2 \alpha K_{i j} + \mathcal{L}_{\beta}\gamma_{i j}
\label{ADMdin}
\end{equation}
$$ \partial_{t} K_{i j}= -D_i D_j \alpha + \alpha [R_{ij}-2 K^k_i K_{jk}+K K_{ij}] + \mathcal{L}_{\beta}K_{ij}$$

\begin{equation}
\mathcal{H}=R- K_{ij}K^{ij}+K^2=16 \pi \rho
\label{ADMconst}
\end{equation}
$$\mathcal{M}_i=D^jK_{ij}-D_i K= 8 \pi j_i$$
where the (\ref{ADMdin}) are the evolution equations for the spatial metric and the extrinsic curvature, while the (\ref{ADMconst}) are the \emph{Hamiltonian} and \emph{Momentum constraints} respectively. However, we have not obtained constraints on the choice of the \emph{gauge functions} lapse $\alpha(t, x^i)$ and shift $\beta^i(t, x^j)$. The freedom in specifying the \emph{gauge functions} derive from the original tensor nature of the Einstein equation. The freedom in choosing the gauge variables allows us to choose the coordinates in a way that simplifies the evolution equations for treating many of the most important physical and astrophysical problems.% carry information about the choice of coordinate system (Fig.\ref{gauge})
Let us go back to the Einstein equation: we said that it is a set of $10$ second-order differential equations of the metric tensor that is equivalent to a set of $20$ first-order differential equations of the metric components. In the  standard $ADM$ we have in total $16$ conditions: $12$ from the evolution equations (\ref{ADMdin}) plus $4$ conditions (\ref{ADMconst}). The $4$ missing equations represent the gauge freedom inherent to General Relativity and correspond to the freedom in specifying the gauge functions $\alpha$ and $\beta^i$. 

The metric and the extrinsic curvature $(\gamma_{\mu \nu}, K_{\mu \nu})$ can be considered as the equivalent of positions and velocities in classical mechanics - they measure the ``instantaneous'' state of the gravitational field, and form the fundamental variables in our initial value formulation. Moreover, we have derived the evolution equation for $\gamma_{ij}$ from considerations purely geometric while the evolution equation for $K_{ij}$ comes from the Einstein's equation. This means that the three-metric contain information about the kinematics of the gravitational system while the extrinsic curvature $K_{ij}$ contain information about the dynamics of the gravitational system.

%%%%%%%%%%%%%%%%%%%%%%%% PROBLEMI ADM %%%%%%%%%%%%%%%%%%%%%%%%%

Although the $ADM$ formulation has served our purpose of writing the equation of Einstein as a Cauchy problem just fine, there are some problems associated with this kind of $3+1$ formulation. The main issue related to the $ADM$ formulation, and also the main reason why it  was initially abandoned to split the Einstein equations, is that the $ADM$ evolution equations are \emph{weakly hyperbolic}.
To appreciate this statement we need a small digression: a large class of systems in physics can be written as a Cauchy problem, which evolution equations are written as
$$\partial_t \vec{f}(\vec{r}, t) + A \cdot \nabla \vec{f}(\vec{r}, t) = \vec{S}(\vec{r}, t)$$ 
where $\vec{f}(\vec{r}, t)$ is a vector field that express the state of the system, $\vec{S}(\vec{r}, t)$ is a source term and $A$ is a matrix of coefficients. The properties of the system are determined by the features of $A$ and $\vec{S}(\vec{r}, t)$, and in particular we have that 
\begin{enumerate}
\item if the elements of $A$ and $\vec{S}$ are constants, then the system is \emph{linear};
\item if the elements of $A$ and $\vec{S}$ are functions of the spacetime, then the system is \emph{linear} with variable coefficients;
\item if the elements of $A$ are functions of the vector field $A=A(\vec{f})$ then the system is \emph{non-linear}
\end{enumerate}

In order to correctly interpret the physical system, we must verify the \emph{well-posedness} of the Cauchy problem that describe the system. The notion of well-posedness of the Cauchy problem is closely related to the nature of the given system of differential equations, and in particular with the criteria of \emph{hyperbolicity}
\begin{definition}
\centering
\emph{ A system of differential equations is said to be \textsc{(strongly) hyperbolic} if the Cauchy problem is well posed.}
\end{definition}
The following theorem is valid:
\begin{theorem}
If the coefficient matrices $A$ of the equations system is a constant matrices then a necessary condition, in order that the system be strongly hyperbolic, is that:
\begin{enumerate}
\item $A$ has N real eigenvalues $\{ \lambda_1 \cdots \lambda_N \}$;
\item  $A$ is diagonalizable.
\end{enumerate}
\end{theorem}

Thanks to this theorem, we can define other ``hyperbolicity degrees'' to characterize our Cauchy problem:
\begin{definition}
\centering
\emph{ A system of differential equations is said to be \textsc{symmetric hyperbolic} if the coefficients matrix $A$ is symmetric $A=A^T$}
\end{definition}
\begin{definition}
\centering
\emph{ A system of differential equations is said to be \textsc{strictly hyperbolic} if the eigenvalues $\lambda_i$ of the coefficients matrix $A$ are real and distinct.}
\end{definition}
\begin{definition}
\centering
\emph{ A system of differential equations is said to be \textsc{weakly hyperbolic} if the coefficients matrix $A$ is not diagonalizable.}
\end{definition}

So it follows that a weakly hyperbolic system is not guaranteed to be well-posed and therefore the numerical solution of such equations led to the growth of unstable models.
Analyzing the $ADM$ equations, from the mixed derivatives in the Ricci tensor for the solution of the extrinsic curvature\footnote{The evolution equations for the extrinsic curvature is
$$\partial_t K_{ij}= D_i D_j \alpha + \alpha (R_{i j}+\cdots)$$
the term $R_{ij}$ contains $\gamma_l^i \gamma_m^j \partial_i \partial_j$, which led to diagonal second derivatives but also mixed second derivatives ($\partial_x \partial_y$, $\partial_x \partial_z$, $\partial_z \partial_y$).}, we can infer that (\ref{ADMdin}) are weak hyperbolic equations. 
Therefore, in order to continue, we can follow two paths: abandon the $ADM$ formulation, or modify it in such a way that the $ADM$ equations become hyperbolics.

We will choose the second approach, but first it is worth noting that the just presented York formulation of the ADM equation is different from the original ADM formulation. The original ADM formulation uses as dynamical variables the spatial metric $\gamma_{ij}$ and its canonical conjugate momentum $\pi_{ij}$, which are related to the extrinsic curvature as

$$K_{ij}=-\dfrac{1}{\sqrt{\gamma}}(\pi_{i j}- \dfrac{1}{2} \gamma_{i j} \pi)$$

Rewriting the original $ADM$ equations in terms of the extrinsic curvature, we notice that they are different from the formulation \textit{\'a la} York for a term proportional to the Hamiltonian constraint. So the evolution equations of two formulations are \emph{physically equivalent} (since they only differ by the addition of a term proportional to the Hamiltonian constraint), but they are not \emph{mathematically equivalent}.
This consideration take us to a fundamental observation: the evolution equations are highly non-unique since we can always add to them arbitrary multiples of the constraints. The different systems of evolution equations will still coincide in the physical solutions, but might differ dramatically in their mathematical properties.
From now on we will use the ADM equations \textit{\'a la} York, which we will call \emph{Standard ADM}.\\


The non-uniqueness of the $3 + 1$ decomposition allow us to define new formulations of evolution equations (\ref{ADMdin}), physically equivalents to the standard $ADM$ equations but with better stability properties for numerical simulations. 
In particular, we will present a specific formulation which is particularly adapts for numerical simulations: the \emph{Conformal ADM}, or (the more commonly used name) \emph{Baumgarte, Shapiro, Shibata, Nakamura, Oohara and Kojima formulation} ($BSSNOK$).

The starting point of this reformulation is the \emph{conformal rescaling of the spatial metric}
\begin{equation}
\tilde{\gamma}_{i j}= \psi^{-4} \gamma_{ij}
\label{gammaConf_eq}
\end{equation}
$\psi$ is a conformal factor that can be chosen in a number of different ways.
In particular the $BSSNOK$ formulation choose the conformal factor in such a way that the conformal metric $\tilde{\gamma}_{ij}$ has unit determinant during all the evolution, i. e. $\psi^4= \gamma^{\frac{1}{3}}$ with $\gamma$ the determinant of the spatial metric. With this choice we have that is
\begin{equation}
\psi= \gamma^{\frac{1}{12}}
\label{ConfFact}
\end{equation}
Now, using the evolution equation for the spatial metric (\ref{ADMdin}), we find that the evolution equation for the determinant of the metric is
$$\partial_t \gamma = \gamma (-2 \alpha K + 2 D_i \beta^i)=-2 \gamma(\alpha K - \partial_i \beta^i)+ \beta^i \partial_i \gamma$$
which, using the (\ref{ConfFact}), implies
$$\partial_t \psi =-\dfrac{1}{6} \psi(\alpha K - \partial_i \beta^i)+ \beta^i \partial_i \psi $$
Written in this form it is easy to see that, redefining the conformal factor $\psi$ as $\phi=\log \psi= \frac{1}{12} \log \gamma$ so that $\tilde{\gamma}_{ij}=e^{-4 \phi}\gamma_{ij}$, the previous equations are
\begin{equation}
\partial_t \phi =-\dfrac{1}{6} (\alpha K - \partial_i \beta^i)+ \beta^i \partial_i \phi 
\end{equation}  

Another feature of the $BSSNOK$ formulation is the separation of the extrinsic curvature into its trace $K$ and its tracefree part
\begin{equation}
A_{ij}=K_{ij}- \dfrac{1}{3} \gamma_{ij}K
\end{equation}
and the application of a conformal rescaling to the traceless extrinsic curvature
\begin{equation}
\tilde{A}_{ij}= \psi^{-4}A_{ij}=e^{-4 \phi}A_{ij}
\end{equation}
The traceless condition follows from
$$\tilde{A}_{ij}\gamma^{ij}=\tilde{A}^i_i= \psi^4(K^i_i - \dfrac{1}{3}\gamma_{ij}\gamma^{ij}K)=0$$

In addition to the previous quantities, the BSSNOK formalism also define the \emph{Cristoffel symbols of conformal space metric} $\tilde{\Gamma}^i_{jk}$

\begin{equation}
\tilde{\Gamma}^i_{jk}=\Gamma^i_{jk}-2(\delta^i_j \partial_k \phi + \delta^i_k \partial_j \phi - \gamma_{jk}\gamma^{il} \partial_l \phi)
\end{equation}

and the \emph{Gammas}, to separate the mixed derivatives:
\begin{equation}
\tilde{\Gamma}^i= \tilde{\gamma}^{jk} \tilde{\Gamma}^i_{jk}=\tilde{\gamma}^{ij} \tilde{\gamma}^{kl}\partial_l \tilde{\gamma}_{jk}
\end{equation}
this implies $\tilde{\Gamma}^i= 2\tilde{\gamma}^{ij} \partial_j \phi+ e^{4 \phi} \tilde{\Gamma}^i_{jk}$.

The system of evolution equations then takes the form

\begin{equation}
\dfrac{d}{dt} \tilde{\gamma}_{ij}= -2 \alpha \tilde{A}_{ij}
\end{equation}
\begin{equation}
\dfrac{d}{dt} \phi= -\dfrac{1}{6} \alpha K
\end{equation}
\begin{equation}
\dfrac{d}{dt} \tilde{A}_{ij}= e^{-4\phi}\left\{ -D_i D_j \alpha + \alpha R_{ij}+ 4 \pi \alpha [\gamma(S-\rho)-2 S_{ij}]\right\} + \alpha(K \tilde{A}_{ij}-2\tilde{A}_{ik}\tilde{A}^k_j)
\end{equation}
\begin{equation}
\dfrac{d}{dt} K= -D_i D^i \alpha + \alpha( \tilde{A}_{ij}\tilde{A}^{ij}+ \dfrac{1}{3}K^2)+ 4 \pi \alpha (S+\rho)
\end{equation}
where we have posed $\frac{d}{dt}= \partial_t - \mathcal{L}_{\vec{\beta}}$, $TF$ denotes the tracefree part of the expression inside the brackets and, in the evolution equation for $K$, we have used the Hamiltonian constraint in order to eliminate the Ricci scalar:
\begin{equation}
R=K_{ij}K^{ij}-K^2+ 16 \pi \rho= \tilde{A}_{ij}\tilde{A}^{ij}+ \dfrac{2}{3}K^2 + 16 \pi \rho
\end{equation}

In the evolution equations for $\tilde{A}_{ij}$ and $K$ there appear covariant derivatives of the lapse function with respect to the physical metric $\gamma_{ij}$. This can be calculated by using the Cristoffel symbols of conformal space metric previously defined, since $\tilde{\Gamma}^i= 2\tilde{\gamma}^{ij} \partial_j \phi+ e^{4 \phi} \tilde{\Gamma}^i_{jk}$.
From this we can infer the evolution equation for the $\tilde{\Gamma}^i$:
\begin{equation}
\dfrac{d}{dt}\tilde{\Gamma}^i= \tilde{\gamma}^{jk}\partial_j \partial_k \beta^i + \dfrac{1}{3}\tilde{\gamma}^{ij}\partial_j \partial_k \beta^k - 2 \tilde{A}^{ij} \partial_j \alpha
+ 2 \alpha(\tilde{\Gamma}^i_{jk}\tilde{A}^{jk}+ 6 \tilde{A}^{ij} \partial_j \phi - \dfrac{2}{3}\tilde{\gamma}^{ij} \partial_j K -8 \pi \tilde{j}^i) 
\end{equation}
These equations are those normally referred to as the $BSSNOK$ formulation and, when are compared with the $ADM$ equations, we have five more evolution equations to consider ($\partial_t \phi$, $\partial_t K$ and $\partial_t \tilde{\Gamma}^i$) but now the system is hyperbolic and indeed well behaved. Looking more closely to the degrees of freedom, we have $15$ variables (we have found that there are $17$ variables: $\phi$, $K$ and $\tilde{\Gamma}^i$ are $5$ variables, plus $12$ from $\tilde{\gamma}_{ij}$ and $\tilde{A}_{ij}$; however we have that $\tilde{\gamma}_{ij}$ and $\tilde{A}_{ij}$ are traceless or with a known trace, so we have $2$ conditions which bring the number of variables to $15$.)

The constraint equations are then
\begin{equation}
^{(3)}R-\tilde{A}_{ij}\tilde{A}^{ij}+\dfrac{2}{3}K^2=16 \pi \rho
\label{BSSNOKhamilton_eq}
\end{equation}
\begin{equation}
D_j(\tilde{A}^{ij}-\dfrac{2}{3}\psi^4 \tilde{\gamma}^{ij}K)=8 \pi j^i
\label{BSSNOKmomentum_eq}
\end{equation}
where $\rho$ and $j^i$ are the energy and momentum densities seen by the normal observers 
\begin{equation}
\rho=n^{\mu}n^{\nu}T_{\mu \nu}
\end{equation}
\begin{equation}
j^i=-\gamma^{i \mu}n^{\nu}T_{\mu \nu}
\end{equation}

The $BSSNOK$ formulation allows us to write six out of the ten Einstein field equations as the true evolution equations of the spacetime and the remaining four equations as the constraints that must be satisfied at all times. The existence of the constraints implies that, if we want to do a simulation, we have to first solve the initial condition to obtain the initial values of ${\gamma_{ij}, K_{ij}}$ and then we can evolve the system. Moreover, since they must be true during all the evolution, they are used as a measure of the quality of the solution.
Due to their importance, it is fundamental to learn how to handle the constraints, even if it is not a simple task to absolve. In fact (\ref{BSSNOKhamilton_eq}) and (\ref{BSSNOKmomentum_eq}) form a system of four coupled partial differential equations of elliptic type and in general they are difficult to solve. Still there are several procedures that can be used to solve these equations: here we will present the more common \emph{conformal thin-sandwich approach}.

The basic idea of the conformal thin-sandwich approach to construct initial data is to prescribe the conformal metric on each of two nearby spatial hypersurfaces (the ``thin-sandwich''), or equivalently the conformal metric and its time derivative on a given hypersurface. We then start with the same conformal decomposition $\tilde{\gamma}_{ij}= \psi^{-4} \gamma_{ij}$ and, defining $\tilde{u}_{ij}=\partial_t \tilde{\gamma}_{ij}$, we require that
$$\tilde{\gamma}^{ij}\tilde{u}_{ij}=0$$
which is equivalent of demanding that the volume element of the conformal metric remains momentarily fixed.
Now, considering the tracefree part of the evolution equation for the spatial metric, let us define\footnote{We use an algebraic result which states that 
\begin{theorem}
Any symmetric-tracefree tensor $S^{ij}$ can be split in
$$S^{ij}=S^{*ij}+(\mathbf{L} W)_{ij}$$
\end{theorem}
where $S^{*ij}$ is a symmetric, traceless and transverse ($D_jS{*ij}=0$) tensor.}

$$u_{ij}=\partial_t \gamma_{ij}-\dfrac{1}{3}\gamma_{ij}(\gamma_{kl}\partial_t \gamma_{kl})=-2 \alpha A_{ij}+ (\mathbf{L} \beta)_{ij}$$

where $\mathbf{L}$ is the operator associated with the spatial metric and defined as $(\mathbf{L} W)^{ij}=D^iW^j+D^j W^i - \frac{2}{3}\gamma^{ij}D_k W^k$. It is known as the \emph{conformal Killing form}\footnote{$\mathcal{L}_{\vec{W}}(\gamma^{-\frac{1}{3}}\gamma_{ij})=(\mathbf{L}W)_{ij}=0$, that is the conformal metric $\tilde{\gamma}_{ij}=\gamma^{-\frac{1}{3}}\gamma_{ij}$} associated with the vector $W^i$.
From $\tilde{\gamma}^{ij}\tilde{u}_{ij}=0$ follows that $$\partial_t \log \psi=\partial_t \log \gamma^{\frac{1}{12}} $$
so that one finds
$$\tilde{u}_{ij}= \partial_t (\psi^{-4}\gamma_{ij})=\psi^{-4} (\partial_t \gamma_{ij}- 4 \gamma_{ij}\partial_t \log \psi)$$
$$=\psi^{-4} \left( \partial_t \gamma_{ij}-\dfrac{1}{3}\gamma_{ij} \partial_t \log \gamma \right)=\psi^{-4} u_{ij}$$
Solving $A^{ij}$ using the expression for $u_{ij}$, we have
$$A^{ij}=\dfrac{\psi^{-4}}{2 \alpha} \left[ (\tilde{\mathbf{L}}\beta)^{ij}-\tilde{u}^{ij} \right]$$
Taking 
$$\tilde{A}^{ij}= \psi^{10}A^{ij}$$
and defining the \emph{conformal lapse} $\tilde{\alpha}=\psi^{-6} \alpha$, we find
$$\tilde{A}^{ij}=\dfrac{1}{2 \tilde{\alpha}} \left[ (\tilde{\mathbf{L}}\beta)^{ij}-\tilde{u}^{ij} \right]$$
The conformal lapse $\tilde{\alpha}=\psi^{-6} \alpha$, in the case when $\psi=\gamma^{\frac{1}{12}}$, corresponds  to a rescaling of the lapse $\tilde{\alpha}=\gamma^{\frac{1}{2}} \alpha$.
Using the new definition introduced, we can rewrite the constraints as
\begin{equation}
8 \tilde{D}^2 \psi - ^{(3)}\tilde{R} \psi +\psi^{-7}\tilde{A}_{ij}\tilde{A}^{ij}- \dfrac{2}{3}\psi^{5}K^2 + 16 \pi \psi^5 \rho=0
\label{thinHamiltonian_eq}
\end{equation}
\begin{equation}
\tilde{D}_j \left[ \dfrac{1}{2 \tilde{\alpha}}(\tilde{\mathbf{L}}\beta)^{ij} \right]-\tilde{D}_j \left[ \dfrac{1}{2 \tilde{\alpha}}\tilde{u}^{ij} \right]-\dfrac{2}{3}\psi^{6}\tilde{D}^i K -8 \pi \psi^{10}j^i=0
\label{thinMoment_eq}
\end{equation}

The Hamiltonian constraint (\ref{thinHamiltonian_eq}) and the Momentum constraint (\ref{thinMoment_eq}) in this form can be solved to obtain the  conformal factor $\psi$ and the shift vector $\beta^i$, given the conformal metric $\tilde{\gamma}_{ij}$, its time derivative $\tilde{u}^{ij}$, the trace of the extrinsic curvature $K$, the conformal lapse $\tilde{\alpha}$, matter densities $\tilde{\rho}$ and $\tilde{j}^i$. One then reconstructs the physical quantities:
$$\gamma_{ij}=\psi^4 \tilde{\gamma}_{ij}$$
$$K^{ij}=\psi^{-10}\tilde{A}^{ij}+ \dfrac{1}{3} \gamma^{ij}K$$
with $\tilde{A}^{ij}=\dfrac{1}{2 \tilde{\alpha}} \left[ (\tilde{\mathbf{L}}\beta)^{ij}-\tilde{u}^{ij} \right]$.\\

To better understand the advantage of using this approach to find the initial conditions, we will show how to apply the methods just described to the problem of finding initial data for a physical system of multiple black hole spacetimes. This system has the advantage of being a pure vacuum solution, so we will not have to worry about how to describe the matter content. Moreover, it is a solution of great interests in Numerical Relativity both historically, since  the first aim of numerical relativists was to study gravitational waves emitted by rotating binary black holes, and recently, since it is currently used to investigate inhomogeneous cosmological models (that will be analyzed in the following chapters).

Before of evolving the dynamical equations for $(\gamma_{ij}, K_{ij})$, we need to find the initial conditions, so we have to decide an initial time instant. Ideally, we consider the case of time-symmetric initial data, corresponding to a time when the black holes are momentarily static. In this conditions, we clearly have $K_{ij}=0$ as initial data for the extrinsic curvature. This imply that the momentum constraints (\ref{thinMoment_eq}) must be trivially satisfied.

Thus we only need to solve the Hamiltonian constraint (\ref{thinHamiltonian_eq}), which in this case reduces to
\begin{equation}
8 \tilde{D}^2 \psi - \tilde{R} \psi=0
\label{initialMultBH_eq}
\end{equation} 
because $K^{ij}=0$ and we are in vacuum $\rho=0$.
We can chose to simplify the (\ref{initialMultBH_eq}) further by choosing a flat conformal metric $\tilde{R} =0$, obtaining
$$D^2_{flat} \psi=0$$
with $D^2_{flat}$ the standard flat three-Laplace operator.In this way the boundary conditions correspond to an \emph{asymptotically flat spacetime} so that, far away of the gravitational field goes to zero and we have $\psi=1$. Choosing $\psi=1$ everywhere (and this is a solution of the previous boundary equation), we simply recovery the Minkowski spacetime as initial data.

Proceeding to the next approximation, we have
\begin{equation}
\psi=1+\dfrac{k}{r}
\end{equation}
with $k$ an arbitrary constant, and $\lim_{r \to \inf} \psi=1$. Using this conformal factor, the physical metric in spherical coordinates is
$$dl^2=\left( 1+\dfrac{k}{r} \right)^4 \left[ dr^2+r^2 d\Omega^2 \right]$$ 
This metric correspond to the spatial metric for a Schwarzschild black hole written in isotropic coordinates, with $k=M/2$, and thus it corresponds to the solution of the initial data problem for a single Schwarzschild black hole.
As the boundary equation is linear (it was written as a Laplace's equation), we can simply superpose solutions to obtain new solutions. We can build the conformal factor for a multiple $N$ black hole system as

\begin{equation}
\psi= 1+ \sum_{i=1}^{N} \dfrac{m_i}{2 |\vec{r}- \vec{r}_i|}
\label{conformalMultiBH_eq}
\end{equation}
where $\vec{r}_i$ are the positions of each black hole and $m_i$ are known as the \emph{bare masses}\footnote{The bare mass corresponds with the individual mass only in the case of a single black hole, for more than one black hole the definition of the individual masses is somewhat trickier. A commonly used definition is obtained by going to the asymptotically flat end associated with each hole and calculating the $ADM$ mass $M_{ADM}= \sum_i m_i$ there.}. This solution forms the basis of the so called \emph{puncture} of black holes, which we discuss deeply in  Appendix A.

\section{The Einstein Toolkit}

While the formalism of conformal decomposition may appear unnecessarily technical and perhaps confusing initially, this example demonstrates that it provides an extremely powerful tool for constructing solutions to Einstein's equations. In fact, once the formalism has been developed, it is much easier to derive the Schwarzschild solution by going through the above steps then deriving it from Einstein's equations directly. However, except for very idealized problems with special symmetries, such equations must be solved by numerical means and implemented by supercomputers.
This is only one of many examples demonstrating how important the computation is to study natural phenomena.
Also thanks to the rapid development of supercomputers capabilities and of graphics modelling techniques, numerical simulations play a major role in modern physics and in general in all science.

In the field of computational astrophysics, a plethora of codes have been developed to simulate astronomical systems such as galaxies formation and dynamics, merging of binary black holes or neutron stars, supernovae explosions, etc. For instance, a first archievement in this field was the \emph{Millennium Run} \cite{millenium}, which used more than $10$ billion particles to trace the evolution of the matter distribution in a cubic region of the Universe over $2$ billion light-years on a side (Fig. \ref{millenium}). 
\begin{figure}
\centering
\includegraphics[scale=0.17]{figure/millenium.jpg} 
\caption{The Millennium Run is based on a $N$-body code which simulated the evolution of about $10^{10}$ particles under the effects of gravity: Virgo scientists at Max Planck Society in Garching, Germany, have been able to recreate evolutionary histories both for the $20$ million galaxies which populate this enormous volume and for the supermassive black holes which occasionally power quasars at their hearts. By comparing such simulated data to large observational surveys, one can clarify the physical processes underlying the buildup of real galaxies and black holes.
}
\label{millenium}
\end{figure}

A more recent simulation is the \emph{Illustris simulation}: a surprising project in which it is tracked the expansion of the universe, the gravitational pull of matter onto itself, the motion or "hydrodynamics" of cosmic gas, as well as the formation of stars and black holes. These physical components and processes are all modeled starting from initial conditions resembling the very young universe $300,000$ years after the Big Bang and until the present day, spanning over $13.8 $ billion years of cosmic evolution. The simulated volume contains tens of thousands of galaxies captured in high-detail, covering a wide range of masses, rates of star formation, shapes, sizes, and with properties that agree well with the galaxy population observed in the real universe.

Therefore, it is clear that a well-tested and easy to use computational infrastructures would be a great advantage to researchers, which would be able to focus less on the computational aspect of such tasks, and spent more time on the actual physics. In recent years, several codes have been developed with this intent: some of them, such as $N$-body codes, use a typically non-relativistic approach simulating Newtonian gravity effects to which corrective terms are added; others rely on the perturbative approach described above, considering terms of first or second order in relativistic perturbations. Specifically, in this thesis we will focus on that class of totally relativistic codes (relativistic hydrodynamic codes or based on the BSSN formulation), and in particular we will present the \emph{Einstein Toolkit}\cite{loffler2012einstein}, a powerful open-source software platform of core computational tools for relativistic astrophysics and gravitational physics.

\begin{figure}
  \centering
  \includegraphics[width=80mm]{figure/einstool}%
  \qquad\qquad
  \includegraphics[width=90mm]{figure/cactus}
  \caption{Einstein Toolkit and Cactus logos}
  \label{log_fig}
\end{figure}

The Einstein Toolkit $(ET)$ (Fig. \ref{log_fig}) consists of quite a large number of components, of which most currently use the \textsf{Cactus} computational toolkit framework, which provides the basic modular infrastructure for numerical simulations. 
\textsf{Cactus} is a general framework for the development of portable, modular applications, originally developed for numerical relativity, and it is the outcome of many years of code development: its first version was released in $1995$ and over the years it has been generalized for use by scientists in other fields.

\textsf{Cactus} programs are split into two types of components: ``\emph{thorns}'' and ``\emph{flash}''. Flash are the core of the \textsf{Cactus} framework and they represent the \textsf{Cactus} structure that manages how the parts of the program must be carried out. Flash are typically independent of other parts of \textsf{Cactus} and acts as utility and service library. Thorns are separate modules which encapsulate the implementation of some functionality and they can be written in different languages like \textsf{C, C++, Fortran, OpenCL}. Typically they are developed independently and do not directly interact with each other, rather each of them interacts with the flesh which provides the ``glue'' between different thorns. 

Now let us introduce some of the arrangements provided with the \textsf{Cactus} framework, as well as  some of the more important tools.
First of all, \textsf{Cactus} does not provide executable files but it provides infrastructure to \emph{create} executable. So \textsf{Cactus} simulations require an executable to be compiled, which collect all the thorns and modules that will need during the running. This setup allows for quick adaptation to changes in the local environment, (e.g., updated libraries), but also for a simple way to tailor the source code to the users' needs. The executable has one mandatory argument: a \emph{parameter file}. This is a simple text file, containing key-value pairs of parameter names and the desired settings within the simulation. The executable collect and organize all thorns which must be used to model a sample of physical scenarios, while the parameter file is used to choose which of these should be realized.

\textsf{Cactus} separates physics code from infrastructure code; so a typical physics thorn will not care about memory management, parallelization, Input/Output (IO) or grid refinement but these tasks are left to a special thorn called \emph{driver}. Two driver thorns provided with the $ET$ are \textsf{PUGH} and \textsf{Carpet}: both set the the virtual domain of simulations with a Cartesian grid but while \textsf{PUGH} provide a uniform unigrid for the whole domain, \textsf{Carpet} provides a multigrid infrastructure which cover the simulation domain by a set of overlapping patches.

Usually we call \emph{Arrangement} a collections of thorns, which signaling a common task or have a common origin. This grouping is solely done for the benefit of a better overview for the user, in fact being part of one or another arrangement does not have any special meaning for a thorn.
Then, we can continue giving an overview on some of the basic \textsf{Cactus} and ET arrangements:
\begin{enumerate}
\item \emph{Core Arrangement} are all the thorns that provide infrastructure for basic utilities as boundary conditions, coordinates setting, I/O, symmetries (\textsf{CactusBase} and \textsf{CactusUtils}), numerical implementations (\textsf{CactusNumerical}) or external libraries as HDF$5$, FFTW and MPI (\textsf{ExternalLibraries}).
\item \textsf{EinsteinBase} thorns define and register basic variables within numerical relativity. Thorns of this arrangement make use or modify, for example the $ADM$ variables or the stress-energy tensor. Main thorns include \textsf{ADMBase}, which defines groups of grid functions for basic spacetime variables, such as the spatial metric or the extrinsic curvature, based on the $3 + 1$ $ADM$ construction, \textsf{HydroBase} which defines basic variables and grid functions for hydrodynamics evolution or \textsf{TmunuBase} which defines grid functions for stress-energy tensor (``right-hand-side'' of Einstein's equations).
\item \emph{EinsteinEvolve or McLachlan} arrangement contain several thorns related with the numerical evolution of Einstein's field equations. In particular \textsf{McLachlan} thorn is the ET's spacetime evolution code. It uses an accurate finite differencing scheme to discretize spacetime variables in the $BSSN$ form. It is designed to inter-operate through the \textsf{ADMBase}  and \textsf{TmunuBase} interface. Other important thorns are \textsf{GRHydro}, a general relativistic magneto-hydrodynamics (GRMHD) matter evolution, and \textsf{PunctureTracker}, which takes care of black hole tracking.
\item \emph{EinsteinAnalysis} arrangement which includes several thorns useful for analysis such as \textsf{AHFinderDirect}, to find black hole apparent horizons given $(\gamma_{i j}, K_{i j})$; \textsf{ADMAnalysis}, to calculate several quantities from the $ADM$ variables like the components of the Ricci tensor or the Ricci scalar; \textsf{ADMConstraints}, to calculate the $ADM$ constraints violation. 
\end{enumerate}

Now, to better understand how ET works, let us review the main steps we need to follow in order to produce a simulation.
Once we have downloaded the ET on the machine, the first step is having the required \emph{thornlist}\footnote{A thornlist is a text file containing the list of thorns to be downloaded together with the path and version controlling system used for each thorn.} for the configuration intended to be built. Typically, one will not be compiling all the thorns provided with the ET but it is preferable to build a thornlist that is as small as possible, including only the required thorns, but taking care of the (non-trivial) dependencies between thorns. 

In order to compile a \textsf{Cactus} simulation, we first need to create a configuration, specifying the machine features and the thornlist we want to use. The result of this operation is an executable file.

We should now be ready for running. For this, a \emph{parameter file} is needed, specifying which thorns to use within the simulation (not all compiled thorns need to be active), and which specific model parameters have been chosen.
Modifying the thorn activated in the parameter file or the values of the thorn arguments, we change the physical scenarios simulated. 

Therefore, we described core parts of the Einstein Toolkit as generally as possible to give a consistent overview of its capabilities and components. From what has been said, we can consider Einstein Toolkit as a virtual laboratory where we can implement experiments (the simulations) that would otherwise be unfeasible.\\


%In the following chapter we will apply some of the thorns discussed in this chapter, to study the evolution of a Black-Hole Lattice.


Nowadays, both the perturbative approach and the numerical approach are used with pretty good results to investigate the origin and the evolution of the large-scale inhomogeneities of the Universe. However, current and planned galaxy surveys will measure the structure of the Universe with unprecedented precision and we can only make progress in understating the physical laws that govern the Universe if theoretical predictions are made with matching or better accuracy than these measurements. Therefore, we need to improve the realism of our simulations to gain measurements more and more accurate to compare with the experiments.

In this context, the perturbation approach has insurmountable limits, due to its nature, that can only be ignored under certain conditions. On the other hand, the numerical approach to this field is relatively young, and it ``recently'' addressed to the degree of realism required for our purposes. With the intent to pursue this objective, in my thesis I studied the behavior of an inhomogeneous Universe using the numerical approach. In particular, I used the results of Numerical Relativity just treated to simulate the inhomogeneous system of blacks holes lattices\footnote{In particular, in a preliminary phase of this thesis, I riproduced the outcomes already obtained in a previous work by Bentivegna and Korzynski which, using numerical approaches, studied the evolution of closed Universes from initial data on a hypersurface at time-symmetry \cite{eloisaBHL}.}. 
I have choice this particular system for two main reasons:
\begin{enumerate}
\item Black holes, and in particular a system made of multiple black holes is a well-known system in Numerical Relativity (as we have seen before) \cite{mroue2012precessing, sperhake2014numerical}.
\item A discrete distribution of black holes well reproduce the real condition of the mass distribution in the Universe (local concentrations of matter separated by voids).
\end{enumerate}

In order to understand what are the principal features of the black hole lattice Universes, in the following chapter we will present the \emph{Lindquist-Wheeler black hole lattices}.

==> template/contribution.tex <==
%\begin{center}
\section*{Other contributions}
%\end{center}
%\label{sec:declaration}

%\includepdf[pages=-]{papers/contribution.pdf}
\label{contribution} 
\addcontentsline{toc}{chapter}{Other contribution}

Apart from the two original works presented in Chapters~\ref{chap:bigonlight}-\ref{chap:nonlinearities}, the author has been involved in the article \cite{Grasso:2018mei}
\begin{itemize}
     \item {\textbf{``Geometric optics in general relativity using bilocal operators.''} Authors: Michele Grasso, Miko\l{}aj Korzy\'nski, and Julius Serbenta, published in Physical Review D (Phys. Rev. D) (\cite{Grasso:2018mei}). } 
\end{itemize}

In the former work, a new formulation for light propagation in geometric optics by means of the bilocal geodesic operators is presented.
%the new bilocal geodesic operators formulation of geometric optics and its application to describe congruences of null geodesics in general relativity have been presented. 
This novel formulation offers a consistent approach to optical phenomena in curved spacetimes, and it may be used to compute observables like angular diameter distance, luminosity distance, magnification, as well as new real-time observables like parallax and redshift drift, all within the same framework.
Although the results in \cite{Grasso:2018mei} are not included as original work of this thesis, the mathematical machinery of the BGO is presented in Chapter~\ref{chap:BGO} as it provides the theoretical framework on which the results in \cite{Grasso:2021iwq, Grasso:2021zra} are based.

 



==> template/nonlinearities.tex <==
\chapter{Application: Isolating non-linearities in light propagation in inhomogeneous spacetimes}%nonlinearities
\label{chap:nonlinearities}
\MG{intro da paper }
Upcoming galaxy surveys like Euclid, LSST, SKA and others\footnote{{\color{blue}{\tt {http://sci.esa.int/euclid/}}}, {\color{blue}{\tt {https://www.lsst.org}}}, {\color{blue}{\tt {http://skatelescope.org/}}}} mark the beginning of a new exciting era, dubbed \textit{precision cosmology}. The reason behind this name is twofold: on one side these future observations will map almost all the visible universe with the unprecedented precision of $1\%$ and on the other side cosmological modelling aim at the same precision target. 

In this view treating non-linearities, i.e. going beyond (linear) cosmological perturbation theory is of crucial importance and new approximation schemes were developed specifically or approximations used in other contexts were applied to cosmology. They include: the post-Newtonian (PN) approximation (see \cite{mater, carbone2005unified} for formulations of PN cosmology in two different gauges), the post-Friedmann approximation (see \cite{Milillo:2015cva, Rampf:2016wom} for a different approach, which adapts to cosmology the weak-field post-Minkowskian approximation and reproduces linear-order cosmological perturbation theory at their zeroth-order), the weak-field approximation\footnote{The leading order of the last two approximation schemes were shown to be equivalent for a dust universe in the Poisson gauge in \cite{kopp2014newton}, whereas \cite{mater, carbone2005unified} were constructed on purpose to include second-order perturbation theory at their PN order.} (see \cite{green2011new} for the development of the framework and \cite{Adamek:2013wja} for estimations with the use of Newtonian simulations for a plane-symmetric universe), and, more recently, a two-parameters gauge-invariant approximation (see \cite{Goldberg:2016lcq}). In addition, over the past few decades, numerical simulations have increasingly become a powerful tool in cosmology to model the growth of nonlinear structures. Since Newtonian dynamics seems to be a good approximation to describe late-time structure formation, the first generation of cosmological simulations adopted Newtonian gravity to simulate cosmological dynamics. Then, Newtonian simulations were used to feed approximate field equations coming from General Relativity (GR) as e.g. in \cite{Bruni:2013mua, Adamek:2014xba, Fidler:2017pnb}. Only recently we assist to a revolution in cosmological simulations with the birth of codes aiming at simulating fully general relativistic dynamics, \cite{loffler2012einstein, Bentivegna:2016stg, giblin2016departures, adamek2016general, macpherson2017, barrera2020gramses}: for the state of the art and the comparison among different codes, see \cite{Adamek:2020jmr}.

However, a sophisticated general relativistic (exact or approximated) description of cosmological dynamics is not the end of the story. The key point is how (much) it affects light propagation, the final aim being to characterize and (hopefully) measure nonlinear GR effects in the observables on cosmological scales or, at least, quantify their bias in observations. These studies are still in their infancy but they are addressed with several approaches most of which we briefly sketched above. A noncomprehensive list includes \cite{Thomas:2014aga, Barreira:2016wqo, Borzyszkowski:2017ayl, Sanghai:2017yyn, Giblin:2017ezj, Adamek:2018rru, Gressel:2019jxw, Lepori:2020ifz, Macpherson:2021gbh}.
Despite being too early to draw definitive conclusions, it seems that the codes that approximate GR dynamics are in agreement with Newtonian simulations for what concerns weak-lensing observables \cite{Thomas:2014aga, Lepori:2020ifz} but a modification in the statistics of the luminosity distance \cite{Adamek:2018rru} was found. In addition, the PN approximation for some models gives predictions different from $\Lambda$CDM \cite{Sanghai:2017yyn}. A bit of work is still needed to adapt to (observational) cosmology the truly GR numerical codes.

In this paper we examine the differences between linear and nonlinear light propagation. An accurate treatment of the problem would require to analyse light propagation in a realistic model of the universe. However, our aim is not to make general predictions, but rather to deeply investigate the various factors and effects on observables coming from nonlinearities. For this purpose, we decided to employ a toy-model of the universe in which light rays pass through a series of plane-symmetric perturbations around a Friedmann-Lema\^{i}tre-Robertson-Walker (FLRW) background. This model is known as plane-parallel or wall universe, and it was used in the past to study the back-reaction from the small-scale inhomogeneities \cite{Villa:2011vt, diDio2012back, adamek2014distance, Clifton:2019cep}.
We start by extending the results of \cite{Villa:2011vt} by providing the so-called Zel'dovich solution with a $\Lambda$CDM background. In this model, we compute the redshift and the angular diameter distance within three different approximation schemes: linear, Newtonian and post-Newtonian. In order to quantify and isolate nonlinear contributions, we present our results in terms of the relative differences between observables computed with these three different approximations (see Sec. \ref{sec:method} for details). We also analyse different aspects of nonlinearities, e.g. scale-dependence, non-Gaussianity, etc. Even if our modelling is very simple, we believe that this kind of analysis is representative of more general configurations. 

Besides, an important novelty of this work is that we make use of the new {\tt BiGONLight Mathematica} package to study light propagation in GR and compute observables numerically, \cite{Grasso:2021iwq}. Contrary to other software, {\tt BiGONLight} implements light propagation within the new Bilocal Geodesic Operator (BGO) framework, which is applicable to more general situations than the standard formalism and it is also suitable to construct new observables, \cite{Grasso:2018mei, Korzynski:2019oal}. This unique design makes the package adaptable to study various light propagation problems in numerical simulations.

We begin by presenting in Sec. \ref{sec:plane//} the plane-parallel toy-model as introduced in \cite{Villa:2011vt}. Then, in Sec. \ref{sec:lightprop} we briefly describe the BGO framework, pointing out to \cite{Grasso:2018mei} and \cite{Korzynski:2019oal} for further details. In Sec. \ref{sec:method}, we introduce the goals of our analysis and the method which led to the results presented in Sec. \ref{sec:results}. Finally, we address our conclusions in Sec. \ref{sec:concl}.

Notation: Greek indices ($\alpha, \beta, ...$) run from 0 to 3, while Latin indices ($i,j, ...$) run from 1 to 3 and refer to spatial coordinates only. Latin indices ($A,B, ...$) run from 1 to 2. Tensors and bitensors expressed in a seminull frame are denoted using boldface indices: Greek boldface indices ($\boldsymbol{\alpha}, \boldsymbol{\beta}, ...$) run from 0 to 3, Latin boldface indices ($\mathbf{a}, \mathbf{b}, ...$) run from 1 to 3 and capital Latin boldface indices ($\mathbf{A}, \mathbf{B}, ...$) run from 1 to 2. Latin tilded indices ($\tilde{a},\tilde{b}, ...$) run from 0 to 7 and refer to the indices of $8 \times 8$ matrices $\mathcal{W}$ and $\Omega$. A dot denotes derivative with respect to conformal time.
Quantities with a subscript 0 are meant to be evaluated at present, whereas the subscript $``{\rm in}"$ indicates the initial time. 
Similarly, we indicate with a subscript $\mathcal{O}$ ($\mathcal{S}$) quantities defined at the observer (source). An overbar indicates quantities evaluated in the $\Lambda$CDM model.
In this paper we use three different approximations and consequently three different notations: ``N'' for Newtonian, ``PN'' for post-Newtonian, ``Lin'' for first-order perturbation theory. We place these abbreviations up or down depending on convenience.

\section{The wall universe in three approximations}
\MG{paper + pippone N e PN}
\MG{aggiungere pippone Zel'dovic e come si ottiene N and PN}
\label{sec:plane//}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We consider a toy-model characterized by the choice of globally plane-parallel configurations, i.e. the case where the initial perturbation field depends on a single coordinate. The dynamics of this very simple universe consists of a collection of parallel planes that collapse along the direction of their normal to form a pancake. For the purposes of our work, we are not interested in a more realistic modeling of the Universe; rather our main aim is to estimate, isolate and compare purely nonlinear and non-Newtonian contributions in light propagation, e.g. in fundamental observables such as  redshift and angular diameter distance. 

We work in the synchronous-comoving gauge and leave to future work the gauge issue of every perturbation scheme that affects the observables as well as the estimate of the related contributions in other gauges. Despite gauge effects in the observables are known in standard cosmological perturbation theory (see Ref.~\cite{Yoo:2017svj} for a recent discussion of gauge invariance of cosmological observables up to second order), the issue is more delicate for non-standard approximations, such as those considered in this paper.

The starting point of our analysis is the results of Ref.~\cite{Villa:2011vt}: the authors started from the Newtonian background given by the well-known Zel'dovich approximation, \cite{zeldovich70a}, which, for plane-parallel perturbations in the Newtonian limit, represents an exact solution. They then obtained the exact analytical form for the PN metric, thereby providing the exact PN extension of the Zel'dovich solution. Let us remark how the Zel'dovich approximation is constructed: in its conformal version, it is an expansion around the three-dimensional spatial displacement vector of the CDM particles between the position comoving with the Hubble flow and the true position governed by perturbations. The peculiarity is the following: the solution for the displacement vector is strictly linear, as it is found from the linear Newtonian equations of motion. But all other dynamical quantities, such as the mass density, are written in terms of such a displacement vector, as if it was exact, i.e. from their nonperturbative definition. The same construction was first extended to the PN approximation of General Relativity, where the metric tensor also is a dynamical variable, in Ref.~\cite{mater} and specialized in the plane-parallel case in Ref.~\cite{Villa:2011vt}.
The Zel'dovich specific feature is evident in the form of the metric tensor \eqref{eq:metricNWT}, which is quadratic in the perturbations, and the density contrast in Eq.~\eqref{eq:density_N} for the Newtonian background and in Eq.~\eqref{eq:metricPN} and Eq.~\eqref{eq:density_PN} for the PN solution found in Ref.~\cite{Villa:2011vt}.

We provide here the $\Lambda$CDM extension of the PN metric found in Ref.~\cite{Villa:2011vt}, which was obtained for the Einstein-de Sitter background model, i.e. the dust-only universe. 
Starting from the line element
\beq
ds^2=a^2(\eta)\left\{ -c^2 d\eta^2 + \gamma^{\rm{PN}}_{11}(\eta, q_{\rm 1}) dq_{\rm 1}^2 +\gamma^{\rm{PN}}_{22}(\eta, q_{\rm 1}) dq_{\rm 2}^2+\gamma^{\rm{PN}}_{33}(\eta, q_{\rm 1}) dq_{\rm 3}^2\right\}
\eeq

we then obtain the conformal metric given by\footnote{We take this chance to point out a typo in Eq.~(4.37) of Ref.~\cite{Villa:2011vt}: in the first term of the second line of the expression for $\gamma_{11}$ the correct coefficient is $5/756$ instead of $5/576$.}
\begin{equation} \label{eq:metricPN}
\begin{split}
\gamma^{\rm{PN}}_{11} =& \left(1-\frac{2}{3}\frac{\partial_{q_1}^2 \phi_0}{ \stuff} \mathcal{D} \right)^2 +\\
 & +\frac{1}{c^2}\left[-\frac{10}{3} \phi_0 +(4 a_{\rm nl}-5)\frac{ 10}{9}\frac{(\partial_{\rm q_{\rm 1}} \phi_0)^2}{ \stuff}\mathcal{D}  +(a_{\rm nl}-1)\frac{40}{9}\frac{ \phi_0  \partial_{\rm q_{\rm 1}}^2 \phi_0}{ \stuff} \mathcal{D}  + \right.\\
& \left.  \left(\frac{41}{7}-4 a_{\rm nl}\right)\frac{20}{27} \frac{(\partial_{\rm q_{\rm 1}} \phi_0)^2  \partial_{\rm q_{\rm 1}}^2 \phi_0}{(\stuff)^2}\mathcal{D}^2 + \left(3-2 a_{\rm nl}\right) \frac{40}{27}\frac{\phi_0  (\partial_{\rm q_{\rm 1}}^2 \phi_0)^2}{ (\stuff)^2} \mathcal{D}^2 -\frac{80}{189}\frac{(\partial_{\rm q_{\rm 1}} \phi_0)^2 ( \partial_{\rm q_{\rm 1}}^2\phi_0)^2}{(\stuff)^3}\mathcal{D}^3 \right]\\
\gamma^{\rm{PN}}_{22}= & 1+\frac{1}{c^2}\left[ \frac{10}{9}\left( \frac{\mathcal{D} (\partial_{\rm q_{\rm 1}} \phi_0)^2 }{\stuff}-3\phi_0\right)\right]\\
\gamma^{\rm{PN}}_{33}=& 1+\frac{1}{c^2}\left[ \frac{10}{9}\left( \frac{\mathcal{D} (\partial_{\rm q_{\rm 1}} \phi_0)^2 }{\stuff}-3\phi_0\right)\right].
 \end{split}
\end{equation}
In the above expression $\eta$ is the conformal time, $a$ is the scale-factor encoding the evolution of the $\Lambda$CDM  background, $\mathcal{H}_0$, $\Omega_{\rm m_0}$, and $\phi_0$ are the (conformal) Hubble parameter $\mathcal{H} \equiv \dot{a}/a$, the matter (ordinary plus dark) densaity parameter, and the peculiar gravitational potential, respectively, all evaluated at present. The dot denotes differentiation with respect to conformal time. $\mathcal{D}$ is the growing mode solution of the first-order equation for the density contrast which is defined as 
\begin{equation}
\delta(\eta, q_{\rm 1})\equiv \frac{\rho(\eta, q_{\rm 1})}{\bar{\rho}(\eta)}-1,
\end{equation}
where $\bar{\rho}$ the $\Lambda$CDM  background matter density.
At first order in standard perturbation theory and without loss of generality, the space and time dependence of the expression of the growing density contrast can be factored out. In our 
one-dimensional case we have $\delta^{\rm Lin}(\eta, q_{\rm 1})=\mathcal{D}(\eta)\delta^{\rm Lin}_0(q_{\rm 1})$, where we fix the constant $\delta_0$ at the present time, and the growing mode $\mathcal{D}$ obeys the well-known equation
\begin{equation} \label{eqforD+}
\ddot{\cal D} +\mathcal{H}\dot{\cal D}-\frac{3}{2}\mathcal{H}_0^2\Omega_{m_0}\frac{\cal D}{a}=0\,.
\end{equation}
It is worth noticing that these quantities are all connected via the cosmological Poisson equation
\begin{equation}
\mathcal{D} \nabla^2 \phi_{\rm 0} -\frac{3}{2} \stuff  \delta_{\rm Lin} =0 \,.
\label{eq:Poisson_eq}
\end{equation}
Finally, we follow here the parametrization for primordial non-Gaussianity defined in Ref.~\cite{Bartolo:2005kv}: the number $a_{\rm nl}$ parametrizes local primordial non-Gaussianity of the gauge-invariant curvature perturbation of uniform density hypersurfaces. This is linked to the parametrization of the primordial gravitational potential by a simple relation between the respective parameters: $f_{\rm nl}= (5/3) (a_{\rm nl} -1)$.

The metric in~\eqref{eq:metricPN} corresponds to the most sophisticated approximation that we will use in this paper: although being referred to the 1D toy-model, it is fully nonlinear in the standard perturbative sense, i.e. it is not assumed that density perturbations are small. On the contrary, taking advantage of the Zel'dovich prescription, we calculate the density contrast nonperturbatively, see Eq.~\eqref{eq:density_PN} below.
The PN approximation extends standard perturbation theory including the leading-order corrections to the Newtonian treatment, which are the terms proportional to $1/c^2$. For the convergence of the PN expansion in the metric~\eqref{eq:metricPN}, see Ref.~\cite{Villa:2011vt}.  
We will compare light propagation in the spacetime described by~\eqref{eq:metricPN} with other two cases, that are both extended in ~\eqref{eq:metricPN}: the linear order of standard cosmological perturbation theory and the Newtonian approximation. The linear spacetime metric in the synchronous-comoving gauge is very well known and in 1D it reads
\begin{equation} \label{eq:metricIPT}
\begin{split}
\gamma^{\rm{Lin}}_{11} =& 1-\frac{4}{3}\frac{ \mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{ \stuff} -\frac{10}{3\,c^2}\phi_0\\
\gamma^{\rm{Lin}}_{22}= & 1-\frac{10}{3\,c^2}\phi_0\\
\gamma^{\rm{Lin}}_{33}=& 1-\frac{10}{3\,c^2}\phi_0.
 \end{split}
\end{equation}
This metric is the solution of the Einstein's equations expanded at first order around the FLRW background. Note however that the planar symmetry reduces the degrees of freedom to be only scalar (there are no vector or tensor mode in 1D, by construction) and confines the dynamical part in $\gamma^{\rm{Lin}}_{11}$ only, i.e. only in the direction of the perturbations, while in the other two directions we have just the (PN) initial conditions.
On the other hand, in the Newtonian approximation we have
\begin{equation} \label{eq:metricNWT} 
\begin{split}
\gamma^{\rm{N}}_{11} =& \left(1-\frac{2}{3}\frac{ \mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{ \stuff} \right)^2 \\
\gamma^{\rm{N}}_{22}= & 1\\
\gamma^{\rm{N}}_{33}=& 1.
 \end{split}
\end{equation}
This metric can be read off~\eqref{eq:metricPN} by discarding the PN corrections proportional to $1/c^2$. 

For completeness we report here the expressions of the density contrast in the three cases:
\begin{equation}
\delta_{\rm Lin}=\frac{2}{3}\frac{\mathcal{D} \partial^2_{\rm q_{\rm 1}} \phi_0}{\stuff}
\label{eq:density_lin}
\end{equation}
\begin{equation}
\delta_{\rm N}=\frac{\frac{2}{3}\frac{\mathcal{D} \partial^2_{\rm q_{\rm 1}} \phi_0}{\stuff}}{1-\frac{2}{3}\frac{\mathcal{D} \partial^2_{\rm q_{\rm 1}} \phi_0}{\stuff}} 
\label{eq:density_N}
\end{equation}

\begin{equation}
\begin{array}{l}
\delta_{\rm PN}= \frac{\frac{2}{3}\frac{\mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{\mathcal{H}_0^2 \Omega_{\rm m0}}}{\left(1-\frac{2}{3}\frac{\mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{\mathcal{H}_0^2 \Omega_{\rm m0}} \right)}+\frac{1}{c^2}\frac{1}{\left(1-\frac{2}{3}\frac{\mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{\mathcal{H}_0^2 \Omega_{\rm m0}} \right)^2}\left[\frac{5}{9}(3-4 a_{\rm nl})\frac{\mathcal{D}}{\mathcal{H}_0^2 \Omega_{\rm m0}}(\partial_{\rm {q_{\rm 1}}} \phi_{\rm 0})^2+\frac{20}{9}(2-a_{\rm nl})\frac{\mathcal{D}}{\mathcal{H}_0^2 \Omega_{\rm m0}}(\phi_{\rm 0} \partial^2_{\rm {q_{\rm 1}}} \phi_{\rm 0})\right. \\
 \left. +\frac{20}{21}\left(\frac{2}{3}\frac{\mathcal{D}}{\mathcal{H}_0^2 \Omega_{\rm m0}}\right)^2 \partial_{\rm q_{\rm 1}}^2 \phi_0 (\partial_{\rm q_{\rm 1}} \phi_0)^2 \right]
\end{array}
\label{eq:density_PN}
\end{equation}

Note that the Newtonian density contrast, according to the Zel'dovich approximation, is calculated exactly from the continuity equation in the synchronous-comoving gauge (see Eq.~\eqref{eq:delta_ex}) as the PN one, which is just expanded in powers of $1/c^2$.
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figures/deltas.pdf}
\caption{ 
Density contrast at present (conformal) time $\eta_0$ in the three approximations $\delta_{Lin}$, $\delta_{N}$ and $\delta_{PN}$, as in Eqs.~\eqref{eq:density_lin},~\eqref{eq:density_N} and~\eqref{eq:density_PN} respectively. The plots are obtained setting up the potential as $\phi_{\rm 0} =\mathcal{I} \sin(\omega q_{\rm 1})$ with $\omega=\frac{2 \pi}{500 \, \rm Mpc} $ and amplitude $\mathcal{I}$ such that ${\rm max} \Big(\delta_{\rm PN}(\eta_{\rm 0}, q_{\rm 1})\Big)=0.1$. The values for $\Omega_{\rm m0}$, $\Omega_{\rm \Lambda}$, $f_{\rm nl}$ and $\mathcal{H}_{\rm 0}$ are taken from~\cite{planck2018param, planck2019anl}.}
        \label{fig:delta_profile}
\end{figure}
We take our initial conditions at $\eta_{\rm in}$, after the end of inflation and in the matter-dominated era, when linear theory around the Einstein-de Sitter model is still a good approximation. The explicit expression for the initial density contrast is thus
\begin{equation}
\delta_{\rm in}=\frac{2}{3}\frac{\mathcal{D}_{\rm in} \partial^2_{\rm q_{\rm 1}} \phi_0}{\stuff}\,
\label{eq:density_in}
\end{equation}
where $\mathcal{D}_{\rm in}\propto \eta^2_{\rm in}$ is the linear growing mode of the Einstein-de Sitter model. 
We model the profile of the gravitational potential at present as $\phi_{\rm 0} = \mathcal{I} \sin(\omega q_{\rm 1})$, with frequency $\omega=\frac{2 \pi}{500 \, \rm{Mpc}}$ and amplitude $\mathcal{I}$ such that ${\rm max} \Big(\delta_{\rm PN}(\eta_{\rm 0}, q_{\rm 1})\Big)=0.1$. We set the fiducial values of the cosmological parameters from~\cite{planck2018param,planck2019anl} with $\Omega_{\rm m0} =0.3153$, $\Omega_{\rm \Lambda}=0.6847$, $\mathcal{H}_{\rm 0}=67.36$ and $a_{\rm nl}=\frac{3}{5} f_{\rm nl}+1 = 0.46$. 
The three profiles~\eqref{eq:density_lin}, ~\eqref{eq:density_N} and ~\eqref{eq:density_PN} of the density contrast at the present time are shown in Fig.~\ref{fig:delta_profile}. The plot shows the amplitudes of the curves of the N and PN density contrast are shifted to higher values compared to the linear one, namely the N and PN corrections have the effect of increasing both the under- and the over-density peaks by the same amount $\approx4.15\times 10^{-3}$.
The differences in the evolution of the density contrast in the three approximations are more evident from Fig.~\ref{fig:density_variations}, in which we analyse the growth of an initial under-density, $\delta_{\rm in}<0$, over-density, $\delta_{\rm in}>0$, and the case of vanishing $\delta_{\rm in}$.
In Figs.~\ref{fig:delta_Lin_N} and  \ref{fig:delta_PN_N} we show the deviations $\left|\frac{\delta_{\rm Lin}-\delta_{\rm N}}{\delta_{\rm N}}\right|$ and $\left|\frac{\delta_{\rm PN}-\delta_{\rm N}}{\delta_{\rm N}}\right|$ respectively, at fixed position as a function of time for the two cases of initial over- and under-densities. 
In Fig.~\ref{fig:delta_Lin_N} we clearly see that the variation Lin vs N grows with time,
reaching $\approx 9\%$ at present, which is exactly the shift of $4.15\times 10^{-3}$ that we see in Fig.~\ref{fig:delta_profile}. The variation PN vs N grows with time as well, Fig.~\ref{fig:delta_PN_N}, but the value at present is 4 orders of magnitude less. Furthermore, in this figure we can also appreciate how the over-densities accrete faster than the under-densities, as one should expect. This is not visible in Fig.~\ref{fig:delta_Lin_N}, due to the fact that the difference between the linear and the Newtonian approximation is dominant.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}%0.40\textwidth
        \includegraphics[width=\linewidth]{figures/delta_lin_N}
       \caption{$\left|\frac{\delta_{\rm Lin}-\delta_{\rm N}}{\delta_{\rm N}}\right|$}
        \label{fig:delta_Lin_N}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/delta_PN_N.pdf}
        \caption{$\left|\frac{\delta_{\rm PN}-\delta_{\rm N}}{\delta_{\rm N}}\right|$ }
        \label{fig:delta_PN_N}
    \end{subfigure}
    \\
    \begin{subfigure}{0.5\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/delta_homo.pdf}
        \caption{ Difference $\left|\delta_{\rm PN}-\delta_{\rm N}\right|$ and $\left|\delta_{\rm PN}-\delta_{\rm N}\right|$ for regions with $\delta_{\rm in} = 0$ }
        \label{fig:delta_homo}
    \end{subfigure}
    \caption{Comparison between $\delta_{\rm Lin}$, $\delta_{\rm N}$ and $\delta_{\rm PN}$ as functions of conformal time $\eta$. The comparisons  \ref{fig:delta_Lin_N} and \ref{fig:delta_PN_N} are evaluated for an initial over-density $\delta_{\rm in}>0$ and under-density $\delta_{\rm in}<0$, while \ref{fig:delta_homo} is plotted for $\delta_{\rm in}=0$. All the three approximations are obtained for $\phi_{\rm 0} =\mathcal{I} \sin(\omega q_{\rm 1})$ with $\omega=\frac{2 \pi}{500 \, \rm Mpc} $,  amplitude $\mathcal{I}$ such that ${\rm max} \Big(\delta_{\rm PN}(\eta_{\rm 0}, q_{\rm 1})\Big)=0.1$. and cosmological parameters taken from~\cite{planck2018param, planck2019anl}.}\label{fig:density_variations}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The case of $\delta_{\rm in}=0$ is presented in Fig.~\ref{fig:delta_homo}, where we plot the differences $\left|\delta_{\rm Lin}-\delta_{\rm N}\right|$ and $\left|\delta_{\rm PN}-\delta_{\rm N}\right|$. The reason why we took the difference instead of the variation (as was done in the over- and under-density cases) is to avoid the operation of dividing by zero, since we are considering regions with $\delta=0$.
We begin by noticing that for $\delta_{\rm in}=0$ both $\delta_{\rm Lin}$ and $\delta_{\rm N}$ vanish at any time, as evident from~\eqref{eq:density_lin} and~\eqref{eq:density_N}: both $\delta_{\rm Lin}$ and $\delta_{\rm N}$ are proportional to $\partial^2_{\rm q_{\rm 1}}\phi_{\rm 0}$ and they are exactly zero at the same value of $q_{\rm 1}$, in our toy model $\phi_{\rm 0}\propto \sin(\omega q_{\rm 1})$. Conversely, the term $\propto\partial_{\rm q_{\rm 1}}\phi_{\rm 0}$ in $\delta_{\rm PN}$~\eqref{eq:density_PN} implies that $\delta_{\rm PN}(\eta_{\rm in})\neq 0$ at the position where $\delta_{\rm in}=0$. Therefore, what is actually shown in Fig.~\ref{fig:delta_homo} is the evolution of the density contrast in the post-Newtonian approximation, whose absolute value increases up to $\approx 3\ \times 10^{-6}$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Method}
\label{sec:method}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The core of our analysis is to estimate the magnitude of the nonlinear effects on light propagation, through the comparison of some cosmological observables calculated within different approximation schemes. In particular, we will compare the redshift $z$ and the angular diameter distance $D_{\rm ang}$ computed in the following three cases:
\begin{enumerate}
\item using the first-order expansion in standard cosmological perturbation theory of the plane-parallel metric \eqref{eq:metricIPT} and performing light propagation perturbatively, up to first order. We will denote as $O^{\rm Lin}$, the generic observable $O$ obtained in this way, which only includes effects linear in the perturbations; ($z^{\rm Lin}$ and $D_{\rm ang}^{\rm Lin}$ are derived in App. \ref{apx:linear_obs});
\item using the Newtonian part of the plane-parallel metric, namely the metric in Eq.~\eqref{eq:metricNWT}, and performing exact light propagation\footnote{The term ``exact'' refers to the fact that no perturbative approach is used when we derive and solve the equations describing the propagation of light and observables. In other words, even if the spacetime metric was obtained using some perturbation scheme, we use it as if it were exact for the entire procedure to calculate the observables, starting from the very beginning, i.e. the geodesic equation. We will discuss this approach further on in this section.} using numerical integration. The observables calculated in this way will be indicated as $O^{\rm N}$;
\item using the full PN plane-parallel metric \eqref{eq:metricPN} and performing exact light propagation via numerical integration. We denote the observables calculated with this method as $O^{\rm PN}$.
\end{enumerate}
The observables calculated with the last two methods, $O^{\rm N}$ and $O^{\rm PN}$, are obtained using \emph{\texttt{BiGONLight.m}} (\textbf{Bi}-local \textbf{G}eodesic \textbf{O}perators framework for \textbf{N}umerical \textbf{Light} propagation), a publicly available {\tt Mathematica} package ({\color{blue}{\tt {https://github.com/MicGrasso/bigonlight1.0}}}) developed to study light propagation in numerical simulations using the BGO framework. The package contains a collection of function definitions, including those to compute geodesics, parallel transported frames and solve the BGO's equation~\eqref{eq:GDE_for_BGO}. \texttt{BiGONLight.m} works as an independent package that, once is called by a {\tt Mathematica} notebook, can be used to compute numerically the BGO along the line of sight, given the spacetime metric, the four-velocities and accelerations of source and observer as inputs: a sample of the notebook we used for our analysis can be found in the repository folder \emph{Plane-parallel}. An exhaustive description of \texttt{BiGONLight} and several tests of the package are presented in \cite{Grasso:2021iwq}. Here we just report in App. \ref{apx:bigonlight} two case studies of code testing, the $\Lambda$CDM and the Szekeres model. 

Let us now comment about the fact that we use exact light propagation for the Newtonian and post-Newtonian observables, despite the fact that the respective spacetime metric is obtained with perturbative techniques. First, we notice that this method used to compute $O^{\rm PN}$ does not produce observables strictly of PN order: the observables $O^{\rm PN}$ will contain also some of higher than PN contributions, coming from the fact that we start from the PN metric \eqref{eq:metricPN} but we do not expand further the equations for light propagation or the expressions for the observables in powers of $1/c^2$ (we set $c=1$ everywhere). One would naively expect that the higher than PN terms are always subleading with respect to the PN ones, as in any well-defined perturbation scheme. The key point here is if this hierarchy, which starts at the level of metric perturbations, is preserved throughout the full calculation to the final results, especially in our case where the equations to compute the observables are fully non-linear. We find that this is indeed the case, as indicated in similar investigations in the literature. In order to show this explicitly and to give an estimate of the higher than PN corrections, we have compared the density contrast calculated strictly up to PN order $\delta_{\rm PN}$ \eqref{eq:density_PN} and the density contrast $\delta_{\rm ex}$ obtained from its exact expression from the continuity equation in synchronous-comoving gauge, i.e.
\begin{equation}
\delta_{\rm ex}(\eta,q_{\rm 1})= (\delta(\eta_{\rm in},q_{\rm 1})+1)\sqrt{\frac{|\gamma(\eta_{\rm in},q_{\rm 1})|}{|\gamma(\eta
,q_{\rm 1})|}}-1 \, ,
\label{eq:delta_ex}
\end{equation} 
where $|\gamma|$ is the short-hand notation for the determinant of the metric \eqref{eq:metricPN}, calculated here without expanding in powers of $1/c^2$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=1.01\textwidth]{figures/delta_PN_N.pdf}
       \caption{$\left|\frac{\delta_{\rm PN}-\delta_{\rm N}}{\delta_{\rm N}}\right|$}
    \end{subfigure}
    \!\!\! 
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=1.01\textwidth]{figures/delta_ex_PN.pdf}
        \caption{$\left|\frac{\delta_{\rm ex}-\delta_{\rm PN}}{\delta_{\rm PN}}\right|$ }
    \end{subfigure}
    \caption{Evolution of the variation $\delta_{\rm PN}$ vs $\delta_{\rm N}$ (a) and $\delta_{\rm ex}$ vs $\delta_{\rm PN}$ (b) for initial over-density $\delta_{\rm in}>0$ and under-density $\delta_{\rm in}<0$ regions for $k = 500\, \rm Mpc$. The variation $\delta_{\rm ex}$ vs $\delta_{\rm PN}$ (b) is 4 orders of magnitude smaller than the variation $\delta_{\rm PN}$ vs $\delta_{\rm N}$ (a).}\label{fig:over-under_delta_ex_VS_PN}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=1.01\textwidth]{figures/delta_homo_PN_N.pdf}
        \caption{$\left|\delta_{\rm PN}-\delta_{\rm N}\right|$ }
       
    \end{subfigure}
    \!\!\! 
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=1.01\textwidth]{figures/delta_homo_ex_PN.pdf}
        \caption{$\left|\delta_{\rm ex}-\delta_{\rm PN}\right|$ }
    \end{subfigure}
    \caption{Evolution of the variation $\delta_{\rm PN}$ vs $\delta_{\rm N}$ (a) and $\delta_{\rm ex}$ vs $\delta_{\rm PN}$ (b) for regions with $\delta_{\rm in}=0$ and $k = 500\, \rm Mpc$. The variation $\delta_{\rm ex}$ vs $\delta_{\rm PN}$ (b) is 6 orders of magnitude smaller than the variation $\delta_{\rm PN}$ vs $\delta_{\rm N}$ (a).}\label{fig:d=0_delta_ex_VS_PN}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The plots in Fig.~\ref{fig:over-under_delta_ex_VS_PN} show that the variation between $\delta_{\rm PN}$ and $\delta_{\rm ex}$ is 4 orders smaller than the variation between $\delta_{\rm N}$ and $\delta_{\rm PN}$ for initial over- and under-dense regions and it is 6 orders smaller when we consider regions with vanishing initial density contrast, Fig.\ref{fig:d=0_delta_ex_VS_PN}. This is something we expected, since the impact of the corrections gets smaller and smaller with the increase of the order in the expansion and, more importantly, we were able to isolate and quantify the corrections coming from the higher than PN terms. This specific result holds for the density contrast but it is perfectly reasonable that this estimation is roughly valid for the observables too, even if the calculation to get them is different. We believe that the argument just presented validates our method of performing exact light propagation.

In order to compare the observables calculated within different approximations, we introduce the dimensionless variation $\Delta O$ for the generic observable $O$ calculated in the two approximations $\mathit{a}$ and $\mathit{b}$ defined as:
\begin{equation}
\Delta O (b, a)= \frac{O^{\mathit{b}}-O^{\mathit{a}}}{O^{\mathit{a}}}
\label{eq:variation}
\end{equation}
where $\mathit{a}$ and $\mathit{b}$ stand for $\rm \Lambda CDM$, $\rm Lin$, $\rm N$ or $\rm PN$, namely the $\rm \Lambda CDM$ background, the linear order in standard PT, Newtonian or post-Newtonian approximations, respectively.

Having introduced the general method we use for our analysis and we defined the key quantity for our comparisons, we have to specify the free functions and the parameters of the plane-parallel universe we are considering, of the $\rm \Lambda CDM$ background model and its perturbations. We recall that the evolution of the inhomogeneities in our model is governed by the growing mode solution $\mathcal{D}$ \eqref{eqforD+}, while the spatial part of the matter distribution is determined by the gravitational potential $\phi_{\rm 0}$, which is the only free function. We use a sinusoidal profile for the gravitational potential $\phi_{\rm 0}$ defined as:
\begin{equation}
\phi_{\rm 0}= \mathcal{I} \sin(\omega q_{\rm 1})
\label{eq:phi}
\end{equation}
where the frequency $\omega=2 \pi/k$ is determined from the scale of the inhomogeneities $k$, while the amplitude $\mathcal{I}$ is obtained from \eqref{eq:density_PN} for a certain value of the maximum of post-Newtonian density contrast today $\delta^{\rm max}_{0}$. The scale $k$ and the maximum of the density contrast $\delta^{\rm max}_{0}$ are linked by the matter power spectrum and we will repeat our analysis for different values of $(k, \delta^{\rm max}_{0})$ (this will be discussed in the Sec.~\ref{sec:results}). In Table \ref{tab:k-delta} we report the chosen  values for the scales and the corresponding maximum of the density contrast today.
\begin{table}\caption{\label{tab:k-delta}Values $(k, \, \delta^{\rm max}_{0})$ used in our analysis.}
%\begin{ruledtabular}
\begin{tabular}{lccccc}
$k\, (\rm Mpc)\, $ & $\, 500\, $ & $\, 300 \,$ & $\, 100 \,$ & $\, 50 \,$ & $\, 30 \,$\\
$\delta_{\rm 0}^{\rm max}$ & $0.1$ & $0.35$ & $1$ & $1.5$ & $1.8$\\
\end{tabular}
%\end{ruledtabular}
\end{table}
The cosmological parameters are set using the fiducial values from~\cite{planck2018param}, i.e. $\Omega_{\rm m0} =0.3153$, $\Omega_{\rm \Lambda}=0.6847$ and $\mathcal{H}_{\rm 0}=67.36$. For primordial non-Gaussianity we use the parameter $a_{\rm nl}$ introduced in \cite{Bartolo:2005kv}. It is linked to the parameter $f_{nl}$ by:
\begin{equation}
a_{\rm nl}=\frac{3}{5}f_{\rm nl}+1
\end{equation}
where $a_{\rm nl}=1$, i.e. $f_{\rm nl}=0$, correspond to the case of exact Gaussian fluctuations. The latest measurement of $f_{\rm nl}$ from the Planck collaboration \cite{planck2019anl} gives $a_{\rm nl}=0.46 \pm 3.06$ that will fix $a_{\rm nl}=0.46$ as the fiducial value for our analysis. However, since in our case we take deterministic initial conditions, $a_{\rm nl}$ merely represents an extra free parameter of our approach which tunes the post-Newtonian corrections\footnote{This is evident, since $a_{\rm nl}$ appears only in the post-Newtonian terms and some of them can be cancelled or dimmed with an appropriate choice of the $a_{\rm nl}$'s value.}. Given that $a_{\rm nl}$ has a lot of room to vary inside its confidence interval of $\pm 3.06$, we have also investigated how the comparison Newtonian vs post-Newtonian gets modified if we take different values of $a_{\rm nl}$ to calculate post-Newtonian observables $O^{\rm PN}$ (see Sec.~\ref{sec:results}).

The last things we need to specify  are  the observer and emitter positions and their kinematics. In our study we place the observer in a position with vanishing initial density contrast $\delta_{\rm in}=0$ and we will leave the analysis on how the comparison change when the observer is located in an initial overdensity or underdensity for future investigations. 
The geodesic equations and the BGO equations \eqref{eq:GDE_for_BGO} are solved giving the initial conditions at the observer position and they are integrated backwards in time up to redshift $z=10$.
The choice of analysing only sources at $z=10$ still leaves us the freedom in selecting the direction from which the light is coming. The difference between geodesics with different directions is mainly due to the way in which the geodesics cross the parallel planes with uniform density.  
To investigate this effect, we have considered two geodesics, one with direction normal to the planes and one with direction parallel to the bisect as represented in Fig. \ref{fig:directions}, considering in both cases the observer in a position with $\delta_{\rm in}=0$ and the gravitational potential \eqref{eq:phi} set such that $k=500 {\rm Mpc}$ and $\delta^{\rm max}_{\rm 0}=0.1$. For both geodesics we have analysed what are the effects of the direction on the variations Newtonian vs post-Newtonian for $\Delta z$ (Fig.~\ref{fig:delta_z_direz}) and $\Delta D_{\rm ang}$ (Fig.~\ref{fig:delta_D_direz}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
    \centering
        \includegraphics[width=0.35\textwidth]{figures/dir.pdf}
       \caption{Graphic representation of the direction normal to the planes (blue) and the direction along the bisect (red). Two geodesics with these directions will intersect the uniform density planes with different angles. Therefore the matter distribution profiles along the geodesics are also different. }
        \label{fig:directions}
\end{figure}

\begin{figure}[!hb]
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=1.01\textwidth]{figures/dirZ_N_PN.pdf}
       \caption{$\Delta z$}
        \label{fig:delta_z_direz}
    \end{subfigure}
    \!\!\! 
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=1.01\textwidth]{figures/dirD_N_PN.pdf}
        \caption{$\Delta D_{\rm ang}$ }
        \label{fig:delta_D_direz}
    \end{subfigure}
    \caption{$\Delta z(PN, N)$ \eqref{fig:delta_z_direz} and $\Delta D_{\rm ang}(PN, N)$ \eqref{fig:delta_D_direz} according to our definition \eqref{eq:variation} for the two geodesics with directions normal to the planes (blue lines) and parallel to the bisect (orange lines).}\label{fig:diff_directions}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From the plots we can conclude that there are small differences in the comparison post-Newtonian vs Newtonian for geodesics with different directions. However, the change in the matter distribution on the geodesic induced by the different directions does not modify the magnitude of the variations too much, but only their shapes. In conclusion, when we consider geodesics along the normal, the effects of the non-linearities are somewhat smaller than for the geodesics along the bisect direction. Nevertheless, from now on, we will consider only geodesics directed along the bisect: this will not affect our conclusions because we will make all the comparisons using geodesics along the bisect in all the cases under study. 

For clarity, the following list summarizes the conditions we set for our analysis:
\begin{itemize}
\item If not specified, the observer $\mathcal{O}$ is placed in a position with initial vanishing density contrast $\delta_{\rm in}=0$.
\item The sources are at redshift $z=10$ and such that the observer receives the light with direction parallel to the bisect.
\item Our analysis is performed in synchronous comoving gauge implying that both emitter and observer are comoving with the cosmic flow. 
\item The primordial non-Gaussianity parameter $a_{\rm nl}$ is set using the fiducial value from Planck \cite{planck2019anl}, i.e. $a_{\rm nl}=0.46$. However, in Sec.~\ref{sec:results} we will also consider the case when $a_{\rm nl}$ is set equal to the extreme of its confidence interval.
\end{itemize}


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Results}
\label{sec:results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we present the results of our study that we plot in terms of the quantity
\begin{equation}
\Delta O (b, a)= \frac{O^{\mathit{b}}-O^{\mathit{a}}}{O^{\mathit{a}}}\, ,
\label{eq:variation_res}
\end{equation} 
where our observables $O$ are the redshift $z$ and the angular diameter distance $D_{\rm ang}$ and $a, b$ stand for the approximations used in turn.
Let us start with Figs. \ref{fig:dz_point_1} and \ref{fig:dD_point_1} in which we plot the variation between linear and Newtonian approximations, $\Delta z (Lin, N)$ and $\Delta D_{\rm ang} (Lin, N)$, and the PN corrections to the Newtonian approximation, $\Delta z (PN, N)$ and $\Delta D_{\rm ang} (PN, N)$ for three different scales, $k=30\, , 100\, , 300\, \rm Mpc$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}%0.40\textwidth
        \includegraphics[width=\linewidth]{figures/R1_z300.pdf}
       \caption{ k=300}
        \label{fig:dz_point_1_k300}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/R1_z100.pdf}
        \caption{ k=100 }
        \label{fig:dz_point_1_k100}
    \end{subfigure}
    \\
    \begin{subfigure}{0.5\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/R1_z30.pdf}
        \caption{ k=30 }
        \label{fig:dz_point_1_k30}
    \end{subfigure}
    \caption{Redshift variations, as defined in Eq.~\eqref{eq:variation_res}, Linear vs Newtonian (blue) and post-Newtonian vs Newtonian (orange) on three different scales $k=30\, , 100\, , 300\, \rm Mpc$. We see that $\Delta z (Lin, N) \sim 10^2 \, \Delta z (PN, N)$ on every scale $k$. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}\label{fig:dz_point_1}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[h]{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/R1_D300.pdf}
       \caption{ k=300}
        \label{fig:dD_point_1_k300}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/R1_D100.pdf}
        \caption{ k=100 }
        \label{fig:dD_point_1_k100}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/R1_D30.pdf}
        \caption{ k=30 }
        \label{fig:dD_point_1_k30}
    \end{subfigure}
    \caption{Angular diameter distance variations, as defined in Eq.~\eqref{eq:variation_res}, Linear vs Newtonian (blue) and post-Newtonian vs Newtonian (orange) on three different scales $k=30\, , 100\, , 300\, \rm Mpc$. We see that $\Delta D_{ \rm ang} (Lin, N) \sim \Delta D_{\rm ang} (PN, N)$ on every scale $k$. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}\label{fig:dD_point_1}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The main result here is that the variations behave differently for the redshift and for the angular diameter distance. Indeed, while for $z$ the post-Newtonian corrections are two orders of magnitudes smaller than the nonlinear Newtonian contributions with respect to linear theory, for $D_{\rm ang}$ the two corrections are of the same order. This can be clearly seen on $k=300 \, \rm Mpc$, Figs. \ref{fig:dz_point_1_k300} and \ref{fig:dD_point_1_k300}, and the same behavior also holds on smaller scales, Figs. \ref{fig:dz_point_1_k100} - \ref{fig:dz_point_1_k30} and \ref{fig:dD_point_1_k100} - \ref{fig:dD_point_1_k30}.
For $z\lesssim 2$ we have that $\Delta z(\rm PN, N)\sim 10^{-6}$ on $k=300\, \rm Mpc$ with oscillation dumped as the redshift increases. On the other hand, for the angular diameter distance $\Delta D_{ \rm ang} (Lin, N) \sim \Delta D_{ \rm ang} (PN, N) \sim 10^{-4}$ on $k=300\, \rm Mpc$ in the full redshift range $[0, \, 10]$. 

We dedicate a separate study, reported in Figs. \ref{fig:dz_point_2} and \ref{fig:dD_point_2}, to the change of the amplitude of all the variations with the scale. We consider inhomogeneities scales of $k= \, 500, \, 300, \, 100, \, 50,\, 30\, \rm Mpc$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R2_zLN.pdf}
       \caption{$\Delta z (\rm Lin, N)$ }
        \label{fig:dz_LvsN_point2}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R2_zPNN.pdf}
        \caption{$\Delta z (\rm PN, N)$}
        \label{fig:dz_PNvsN_point2}
    \end{subfigure}
    \caption{Variations $\Delta z (\rm Lin, N)$ and $\Delta z (\rm PN, N)$, as defined in Eq.~\eqref{eq:variation_res}, on different scales in the range $[30, \, 500] \, \rm Mpc$. Both the variations show a maximum around $k=100 \, \rm Mpc$. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}\label{fig:dz_point_2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R2_DLN.pdf}
       \caption{$\Delta D_{\rm ang} (\rm Lin, N)$}
        \label{fig:dD_LvsN_point2}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R2_DPNN.pdf}
        \caption{$\Delta D_{\rm ang} (\rm PN, N)$}
        \label{fig:dD_PNvsN_point2}
    \end{subfigure}
    \caption{Variations $\Delta D_{\rm ang} (\rm Lin, N)$ and $\Delta D_{\rm ang} (\rm PN, N)$, as defined in Eq.~\eqref{eq:variation_res}, on different scales in the range $[30, \, 500] \, \rm Mpc$. The amplitudes monotonically decrease as the scale $k$ becomes smaller. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}\label{fig:dD_point_2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Fig. \ref{fig:dz_point_2} shows that both the variations $\Delta z(\rm Lin, \, N)$ and $\Delta z(\rm PN, \, N)$ increase from $k=500\, \rm Mpc$ to reach the maximum amplitude on $k=100 \, \rm Mpc$ and then decreases down to $k=30\, \rm Mpc$. In terms of amplitudes we have: $\Delta z(\rm Lin, \, N) \sim 10^{-4}$, with a maximum $\sim 10^{-3}$ around $k=100\, \rm Mpc$ and $\Delta z(\rm PN, \, N) \sim 10^{-7}$, with a maximum $\sim 10^{-6}$ around $k=100\, \rm Mpc$. We again note that the variations for the redshift are damped as $z$ increases. This is most evident for $\Delta z(\rm Lin, \, N)$.
The angular diameter distance shows in Fig. \ref{fig:dD_point_2} a different behavior: the amplitude of both variations $\Delta D_{\rm ang} (\rm Lin, N)$ and $\Delta D_{\rm ang} (\rm PN, N)$ decreases monotonically as the scale $k$ become smaller. Both the amplitudes start from $\Delta D_{\rm ang} \sim 10^{-4}$ on $k=500 \, \rm Mpc$ and decrease to $10^{-6}$ on $k=30 \, \rm Mpc$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
    \centering
     \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R3_zda.pdf}
        \caption{$\Delta z^{\rm PN} (a_{\rm nl_{\rm 1}},\, a_{\rm nl_{\rm 2}})$}
        \label{fig:zPN_a1_vs_a2}
    \end{subfigure}
   \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R3_zaPNN.pdf}
       \caption{$\Delta z (\rm PN, \, N)$}
        \label{fig:dz_PNvsN_for_anl}
    \end{subfigure}
    \caption{The effect of varying primordial non-Gaussianity for the redshift: the variation in Eq.~\eqref{eq:DeltaO_anls},  \eqref{fig:zPN_a1_vs_a2}, and PN correction for different values of $a_{\rm nl}$, \eqref{fig:dz_PNvsN_for_anl}. We find that $\Delta z^{\rm PN} (a_{\rm nl_{\rm 1}}, a_{\rm nl_{\rm 2}}) \lesssim  \, \Delta z (PN, N)$. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}\label{fig:dz_anl}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R3_Dda.pdf}
        \caption{ $\Delta D_{\rm ang}^{\rm PN} (a_{\rm nl_{\rm 1}},\, a_{\rm nl_{\rm 2}})$}
        \label{fig:DPN_a1_vs_a2}
    \end{subfigure}
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R3_DaPNN.pdf}
       \caption{$\Delta D_{\rm ang}(\rm PN, \, N)$}
        \label{fig:dD_PNvsN_for_anl}
    \end{subfigure}
    \caption{The effect of varying primordial non-Gaussianity for the angular diameter distance: the variation in Eq.~\eqref{eq:DeltaO_anls},  \eqref{fig:DPN_a1_vs_a2},  and PN correction for different values of $a_{\rm nl}$, \eqref{fig:dD_PNvsN_for_anl}. We find that $\Delta D_{\rm ang}^{\rm PN} (a_{\rm nl_{\rm 1}}, a_{\rm nl_{\rm 2}}) \sim 10^{-4}  \, \Delta D_{\rm ang} (PN, N)$. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}\label{fig:dD_anl}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As we mentioned in Sec. \ref{sec:method}, different values of the primordial non-Gaussianity parameter $a_{\rm nl}$ tune some of the post-Newtonian terms in \eqref{eq:metricPN}, e.g. a perfect Gaussian initial perturbation ($a_{\rm nl}=1$) cancels out the third term in the PN part of the metric \eqref{eq:metricPN}. We then decided to quantify how the PN observables change when we vary the values of $a_{\rm nl}$ inside the confidence interval measured by Planck, \cite{planck2019anl}. For this analysis, we choose $a_{\rm nl}= 1, 0.46, -2.6, 3.52$, corresponding to Gaussian perturbations ($a_{\rm nl}= 1$), Planck 2018 fiducial value ($a_{\rm nl}= 0.46$), and extremes of confidence interval ($a_{\rm nl}= -2.6, 3.52$). We start the discussion of our results by looking at Figs. \ref{fig:zPN_a1_vs_a2} and \ref{fig:DPN_a1_vs_a2}, in which we plot for the PN observables the quantity
\begin{equation}
\Delta O^{\rm PN} (a_{\rm nl_{\rm 1}}, a_{\rm nl_{\rm 2}})= \frac{O^{\rm{PN}}_{a_{\rm nl_{\rm 1}}}-O^{\rm{PN}}_{a_{\rm nl_{\rm 2}}}}{O^{\rm{PN}}_{a_{\rm nl_{\rm 2}}}}\, ,
\label{eq:DeltaO_anls}
\end{equation} 
where we fix $a_{\rm nl_{\rm 2}}$ to the Planck best-fit value and we vary $a_{\rm nl_{\rm 1}}$.
The effect is different for the redshift and for the angular diameter distance: the variation in $D_{\rm ang}^{\rm PN}$ is $\sim 10^{-9}$, two orders of magnitude smaller than the one in $z^{\rm PN}$. This very difference is evident when we plot the PN corrections for different values of $a_{\rm nl}$, see Figs. \ref{fig:dz_PNvsN_for_anl} and \ref{fig:dD_PNvsN_for_anl}. The effect of tuning primordial non-Gaussianity is roughly of the same order as the PN correction for the redshift and also changes its shape. On the contrary, $D_{\rm ang}$ is completely insensitive to the variation of the non-Gaussianity parameter, since $\Delta D_{\rm ang}^{\rm PN} (a_{\rm nl_{\rm 1}}, a_{\rm nl_{\rm 2}}) \sim 10^{-4}  \, \Delta D_{\rm ang} (PN, N)$.

To conclude our analysis, we isolate and quantify the contribution of the linear PN initial seed proportional to the gravitational potential, i.e. $\gamma_{i j}= - \frac{10}{3 c^2}\phi_{\rm 0} \delta_{i j}$ in the spacetime metric \eqref{eq:metricPN}. To do so, we define an hybrid spacetime metric, labelled with $\tilde{N}$, by adding the initial PN seed to the Newtonian metric~\eqref{eq:metricNWT}, i.e.
\begin{equation} \label{eq:metricNt} 
\begin{split}
\gamma^{\tilde{\rm{N}}}_{11} =& \left(1-\frac{2}{3}\frac{ \mathcal{D} \partial_{\rm q_{\rm 1}}^2 \phi_0}{ \stuff} \right)^2 - \frac{10}{3 c^2}\phi_{\rm 0} \\
\gamma^{\tilde{\rm{N}}}_{22}= & 1 - \frac{10}{3 c^2}\phi_{\rm 0}\\
\gamma^{\tilde{\rm{N}}}_{33}=& 1 - \frac{10}{3 c^2}\phi_{\rm 0}\, ,
 \end{split}
\end{equation}
and we have compared the angular diameter distance computed from the two have compared the angular diameter distance computed from the two approximations in Eq.~\eqref{eq:metricNWT} and in Eq.~\eqref{eq:metricNt}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
    \centering
     \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R4_DPNrN.pdf}
        \caption{Comparison PN vs N (blue) and PN vs $\tilde{N}$ (orange) for the angular diameter distance, as defined in Eq.~\eqref{eq:variation_res}, on $ k= 300 \, \rm Mpc$. The variation $\Delta D_{ \rm ang} (PN, \tilde{N}) \sim \, 10^{-6}$ is two orders of magnitude smaller than $\Delta D_{\rm ang} (PN, N)$. The variable on the horizontal axis is the $\Lambda CDM$ redshift.}
        \label{fig:dD_PNvsRN_k=300}
    \end{subfigure}
    \\
    \begin{subfigure}[h]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/R4_Dlcdm.pdf}
       \caption{Comparison between the different approximations $\rm Lin$, N, $\tilde{N}$, PN and the $\Lambda CDM$ background for the angular diameter distance.}
        \label{fig:dD_PPvsLCDM_withRN_k=300}
    \end{subfigure}
    \caption{Results for the contribution of the initial seeds to the angular diameter distance. For the definition of $\tilde{N}$ see Eq. \eqref{eq:metricNt}.}\label{fig:point_3_LCDM}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The inclusion of the initial seed in the modified Newtonian model is such that the PN variation is reduced by two orders of magnitude, see Fig. \ref{fig:dD_PNvsRN_k=300}. In other words the initial seed is the leading order of the post-Newtonian correction. The effect is even more evident when we consider the variations of each of the approximation $\rm Lin$, N, $\tilde{N}$, PN respect to the $\Lambda CDM$ background: we can clearly distinguish between the two approximations, observing that $\tilde{N}$ behaves as expected very close to the PN approximation.

\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> template/tests.tex <==
\chapter{Code Tests}%tests
\MG{incollare da bigonlight}
\label{chap:test}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we test the accuracy of \texttt{BiGONLight} within well-known cosmological models. The tests are performed by considering the following observables: redshift, angular diameter distance, parallax distance, and redshift drift. We compare the results obtained with three different procedures, by defining the estimator $\Delta O({\rm BGO, X})$
\begin{equation}
\Delta O({\rm BGO, X}) \equiv \dfrac{O^{\rm BGO}-O^{\rm X}}{O^{\rm X}}\, ,
\label{eq:deltaO_def}
\end{equation}
where $O^{\rm BGO}$ refers to Eqs.~\eqref{eq:redshift_def},~\eqref{eq:D_ang_BGO},~\eqref{eq:D_par_BGO}, and~\eqref{eq:z_DRIFT_BGO}. We consider the following three cases: (i) the $\Lambda$CDM model, where the specetime metric is the analytical input for {\tt BiGONLight} to compute $O^{\rm BGO}$ and for $O^{\rm X}$ we use the analytical well-known solutions for all the four observables, see Sec.~\ref{sec:LCDM}; (ii) the inhomogeneous Szekeres model \cite{Meures:Szekeres}, where the specetime metric is again the analytical input for {\tt BiGONLight} but to obtain $O^{\rm X}$ we solve numerically a specific differential equation for each observable, see Sec.~\ref{sec:Szekeres}; (iii) the Einstein-de Sitter model, where the input for {\tt BiGONLight} are the $3+1$ quantities coming from the {\tt Einstein Toolkit} simulation and $O^{\rm X}$ is obtained analytically, see Sec.~\ref{sec:ET}.

It worth noting that if $O^{\rm X}$ is obtained analytically, then $\mathrm{max}\left|\Delta O({\rm BGO, X})\right|$ represents the simulation error: in case (i) we have just the computational error from {\tt BiGONLight} whereas in case (iii) the final error in the observables is the combined effect of both the {\tt Einstein Toolkit} and {\tt BiGONLight} finite precision. On the other hand, if $O^{\rm X}$ is obtained numerically, as in case (ii), then $\Delta O({\rm BGO, X})$ gives only an estimation of the accuracy of the two methods used.

\section{Light propagation in homogeneous cosmologies: LCDM, EdS}
\label{sec:LCDM}
\MG{add EdS together with LCDM + fix intro}
The first group of tests regards the study of light propagation in the flat $\Lambda$CDM model. %This is an exact solution of the Einstein field equations representing an homogeneous and isotropic spacetime and the matter-energy content consists of irrotational dust of cold dark matter and a cosmological constant $\Lambda$. The line element is given by
%\begin{equation}
%ds^2=a(\eta)^2\left(-d\eta^2+ \delta_{i j} dx^idx^j \right)
%\label{eq:FLRW_ds}
%\end{equation} 
%where $\eta$ is the conformal time and $a(\eta)$ is the scale factor, which is the solution of Einstein equations and describes the dynamics of the model. The explicit result is found to be \cite{gradshteyn2014table}
%\begin{equation}
%a(\eta)=\frac{\sqrt[3]{\frac{\Omega_{\rm m_0}}{\Omega_{\rm \Lambda}}} \Big(1-{\rm cn}\left(\mathit{y} |\mathit{r} \right)\Big)}{(\sqrt{3}-1)+(\sqrt{3}+1) {\rm cn}\left(\mathit{y} |\mathit{r} \right)}\, ,\label{eq:a_LCDM}
%\end{equation}
%where ${\rm cn}(\mathit{y}|\mathit{r})$ is the Jacobi elliptic cosine function, with $\mathit{y}=\left(\sqrt[4]{3} \sqrt[6]{\Omega_{\rm \Lambda}} \sqrt[3]{\Omega_{\rm m_0}}\right) \mathcal{H}_0 \eta$, $\mathcal{H}_{\rm 0}$ being the Hubble parameter $\mathcal{H}=\frac{1}{a}\frac{d a}{d \eta}$ evaluated today, and $\mathit{r}=\sqrt{\frac{\sqrt{3}+2}{4}}$.

To test {\tt BiGONLight} we consider two classical observables, namely the redshift $z$ and the angular diameter distance $D_{\rm ang}$, and two interesting observables that are not yet measured in the cosmological context as they belong to the new research field named Real-time Cosmology, see Ref.~\cite{Quercellini:2010zr}. One is the parallax distance which exploits the motion of the Solar System with respect to the Cosmic Microwave Background frame providing a baseline of $78 \, {\rm AU}$ per year for the cosmic parallax\footnote{For an exhaustive definition of the parallax see e.g.  Ref.~\cite{rasanen}, in which the author distinguishes between the three different cases: one source observed by two  observers separated by spacelike interval (classic parallax), two sources observed by two  observers separated by spacelike interval and two sources observed by one observer at two different moments (cosmic parallax also known as position drift).}. Cosmic parallax was first proposed in $1986$ in Ref.~\cite{kardashev} and it is expected to be measured by the Gaia satellite,~\cite{refId0}, in the next few years. For discussions and forecasts about the measurements of the cosmological parallax distance we refer to Refs.~\cite{Ding:2009xs, Quartin:2009xr, Quercellini:2008ty, Quercellini:2010zr, rasanen, singal2015cosmological, Marcori:2018cwn, PhysRevLett.121.021101} and Refs. therein. The other is the redshift drift, i.e. the time variation of the redshift of a source. It was first derived for the FLRW models in Refs.~\cite{sandage, McVittie1962}. Since then, and particularly in recent years, a lot of work has been done to investigate the measurability of the redshift drift in cosmology and the information gained, see e.g. Refs.~\cite{Corasaniti:2007bg, Uzan:2007tc, Uzan:2008qp, Martinelli:2012vq,  Lazkoz:2017fvx}.

The analytical expressions in the flat FLRW cosmologies for the four observables that we consider are
\begin{align}
z^{\rm \Lambda CDM} =& \dfrac{a_0}{a}-1 \label{eq:z_FLRW}\\
D^{\rm \Lambda CDM}_{\rm ang}=&\dfrac{a_0}{1+z}\displaystyle\int^z_0 \dfrac{d z'}{ (1+z')\mathcal{H}(z')}%=\dfrac{1}{1+z} \displaystyle\int^z_0 \dfrac{d z'}{ H_0 E(z')}
 \label{eq:D_ang_FLRW}\\
\nonumber \\
D^{\rm \Lambda CDM}_{\rm par}=& \dfrac{a_0}{\mathcal{H}_{\rm 0}}\dfrac{\displaystyle\int^z_0 \dfrac{\mathcal{H}_{\rm 0} d z'}{ (1+z')\mathcal{H}(z')}}{1+\displaystyle\int^z_0 \dfrac{\mathcal{H}_{\rm 0} d z'}{ (1+z')\mathcal{H}(z')}}%=\dfrac{1}{H_{\rm 0}}\dfrac{\displaystyle\int^z_0 \dfrac{d z'}{ E(z')}}{1+\displaystyle\int^z_0 \dfrac{d z'}{ E(z')}}
 \label{eq:D_par_FLRW}\\
\nonumber  \\
\zeta^{\rm \Lambda CDM}=& \dfrac{\mathcal{H}_{\rm 0}}{a_{\rm 0}}\left(1-\dfrac{\mathcal{H}(z)}{\mathcal{H}_{\rm 0}}\right)%=H_{\rm 0}\left(1-\dfrac{E(z)}{1+z}\right)
\, , \label{eq:z_drift_FLRW}
\end{align}
where the Hubble parameter in the $\Lambda$CDM model is given by
\begin{equation}
\mathcal{H}(z)=\mathcal{H}_{\rm 0}\sqrt{\Omega_{\rm m_0}(1+z)+\Omega_{\rm \Lambda}(1+z)^{-2}}\, .
\label{eq:E(z)}
\end{equation}
We normalize the today scale factor $a_{\rm 0}=1$ and we take $\mathcal{H}_{\rm 0}=67.36\ {\rm km\, s^{-1}\, Mpc^{-1}}$, the matter parameter today $\Omega_{\rm m_0}=0.315$, and the cosmological constant parameter  $\Omega_{\Lambda}=0.685$ from  \cite{planck2018param}.
The integral in Eq.~\eqref{eq:D_ang_FLRW} and~\eqref{eq:D_par_FLRW} can be solved analytically and the results is, \cite{gradshteyn2014table}
\begin{equation}
\displaystyle\int^z_0 \dfrac{d z'}{ (1+z')\mathcal{H}(z')}=\dfrac{
{\rm F}\big[ \xi(z) |\mathit{r} \big] - {\rm F}\big[ \xi(0)|\mathit{r} \big]}{ (\Omega_{\rm m_0})^{\frac{1}{3}}(\Omega_{\rm \Lambda})^{\frac{1}{6}} 3^{\frac{1}{4}}}
\end{equation}
where ${\rm F}\big[ \xi(z) | \mathit{r} \big]$ the elliptic integral of the first kind, with arguments $\mathit{r}=\sqrt{\frac{2+\sqrt{3}}{4}}$ and
\begin{equation}
\xi(z)=\arccos \left( \frac{2\sqrt{3}}{1+\sqrt{3}+(1+z)\sqrt[3]{\frac{\Omega_{\rm m_0}}{\Omega_{\rm \Lambda}}}}-1 \right)\, .
\end{equation}

The fact that we have analytical expressions for the observables makes this model a perfect test-bed for the code.
We compare the results from {\tt BiGONLight} with the one in Eq.~\eqref{eq:z_FLRW}-\eqref{eq:z_drift_FLRW} by considering the variation
\begin{equation}
\Delta O({\rm BGO, \Lambda CDM}) \equiv \dfrac{O^{\rm BGO}-O^{\rm  \Lambda CDM}}{O^{\rm  \Lambda CDM}}\, .
\label{eq:deltaO_LCDM}
\end{equation}
As shown in Fig.~\ref{fig:LCDM}, the numerical implementation of the BGO method is in excellent agreement with the analytical formulas in $\Lambda$CDM, the variation $\Delta O$ being $10^{-22}\, \div \,10^{-32}$. The maximum value of $\Delta O$, of the order of $10^{-22}$, represents the numerical error over the observables and we reached such small values by using the precision control options {\tt WorkingPrecision, PrecisionGoal} and {\tt AccuracyGoal} implemented in {\tt Mathematica}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}%0.40\textwidth
        \includegraphics[width=\linewidth]{figures/LCDM_z.pdf}
       \caption{Redshift}
        \label{fig:LCDM_z}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/LCDM_drift.pdf}
        \caption{Redshift drift}
        \label{fig:LCDM_drift}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/LCDM_Dang.pdf}
        \caption{Angular diameter distance}
        \label{fig:LCDM_Dang}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}%{0.8\columnwidth}
        \includegraphics[width=\linewidth]{figures/LCDM_Dpar.pdf}
        \caption{Parallax distance}
        \label{fig:LCDM_Dpar}
    \end{subfigure}
    \caption{Variations in the $\Lambda$CDM model, Eq.~\eqref{eq:deltaO_LCDM}, for the redshift~\ref{fig:LCDM_z}, the redshift drift~\ref{fig:LCDM_drift}, the angular diameter distance~\ref{fig:LCDM_Dang}, and the parallax distance~\ref{fig:LCDM_Dpar}. The variable in the horizontal axis is the redshift in $\Lambda$CDM. The values for the cosmological parameters are taken from \cite{planck2018param}.}\label{fig:LCDM}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Light propagation in exact inhomogeneous cosmologies}
%\MG{scrivere breve intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{LTB} 
%\MG{scrivere dopo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{The Szekeres model}
\label{sec:Szekeres}
\MG{USED IN CHAP 1: The second group of code tests is performed considering an inhomogeneous cosmological model which is an exact solution of Einstein equations, firstly presented in \cite{Szekeres:1974ct}. The line element for the Szekeres spacetime is:
\begin{equation}
ds^2=- dt^2+e^{2 \alpha} {dx^{\rm 1}}^2+e^{2 \beta} ({dx^{\rm 2}}^2+{dx^{\rm 3}}^2)
\label{eq:Sz_generic}
\end{equation}
with $\alpha$ and $\beta$ functions of the spacetime coordinates $(t, x^{\rm 1},x^{\rm 2},x^{\rm 3})$ that are determined by solving the Einstein equations. We can distinguish two different families of Szekeres models depending whether $\partial_{\rm x^{\rm 3}} \beta \neq 0$ or $\partial_{\rm x^{\rm 3}} \beta = 0$: the first case defines the ``class I'' family, which is a generalization of LTB models (with non-concentric shells), while the case $\partial_{\rm x^{\rm 3}} \beta = 0$ corresponds to a simultaneous generalization of the Friedmann and Kantowski-Sachs models and it defines the ``class II'' family. For a cosmological formulation of the Szekeres spacetimes see e.g. \cite{Goode:1982pg}.
For our tests, we will use a class II Szekeres model filled with dust and a positive cosmological constant as presented in~\cite{Meures:Szekeres}. For this model, the line element \eqref{eq:Sz_generic} is rewritten as:
\begin{equation}
ds^2=a(\eta)^2 \left[- d\eta^2 + {dx^{\rm 1}}^2+{dx^{\rm 2}}^2 +Z(\eta,x^{\rm 1}, x^{\rm 2}, x^{\rm 3})^2 {dx^{\rm 3}}^2\right]
\label{eq:Sz_line}
\end{equation}
and, for the special case of axial symmetry around $x^{\rm 3}$, we have the following form for the function $Z$:
\begin{equation}
Z(\eta,x^{\rm 1},x^{\rm 2},x^{\rm 3})=1+\beta_{\rm +}(x^{\rm 3}) \mathcal{D}(\eta)+\beta_{\rm +}(x^{\rm 3}) B \left({x^{\rm 1}}^2+{x^{\rm 2}}^2\right)\, .
\label{eq_met_func}
\end{equation}
The function $\mathcal{D}$ is the growing mode solution of the first-order Newtonian density contrast defined as $\delta=\dfrac{\rho -\rho_{\rm \Lambda CDM}}{\rho_{\rm \Lambda CDM}}$ and it is given by, see e.g. \cite{Villa:2015ppa},
\begin{equation}
\mathcal{D} (\eta) = \frac{a}{\frac{5}{2}\Omega_{\rm{m 0}} } \sqrt{1+\frac{\Omega_{\rm{\Lambda}}}{\Omega_{\rm{m 0}}}a^3}\,  {}_2 F_{1} \left( \frac{3}{2}, \frac{5}{6}, \frac{11}{6}, -\frac{\Omega_{\rm{\Lambda 0}}}{\Omega_{\rm{m 0}}}a^3 \right)\,,
\label{eq:grow_mode}
\end{equation}
with ${}_2 F_{1} \left(a,b,c, y\right)$ being the Gaussian (or ordinary) hypergeometric function. The term $B$ in Eq.~\eqref{eq_met_func}
 is constant and given by (see App. C in \cite{Grasso:2021zra})
\begin{equation}
B= \frac{5}{4} \stuff \frac{\cal D_{\rm in}}{a_{\rm in}}\, ,
\label{eq:link_on_B}
\end{equation}
where $\mathcal{D}_{\rm in}= a_{\rm in}$ for initial conditions set deeply in the matter-dominated era. The function $\beta_{\rm +}$ specifies the spatial distribution of the first-order density contrast and it can be related to the peculiar gravitational potential $\phi_{\rm 0}$ via the cosmological Poisson equation at present time
\begin{equation}
\beta_{\rm +}=-\dfrac{2}{3}\dfrac{\partial^2_{\rm x^{\rm 3}}\phi_{\rm 0}}{\stuff}\, .
\end{equation}}
For the tests, we will use a sinusoidal profile for the peculiar gravitational potential $\phi_{\rm 0}= \mathcal{A} \sin(\omega x^{\rm 3})$ with $\omega=\dfrac{2 \pi}{500\, \rm Mpc}$ and amplitude $\mathcal{A}$ such that $\delta_{\rm 0}=0.1$ for the density contrast today. 

In the following, we will present the tests over the redshift, the angular diameter distance and the redshift drift. Contrary to the $\Lambda$CDM case, here the observables are obtained using two numerical methods and the difference is expressed by
\begin{equation}
\Delta O({\rm BGO, Sz}) \equiv \dfrac{O^{\rm BGO}-O^{\rm  Sz}}{O^{\rm  Sz}}\, .
\label{eq:deltaO_Sz}
\end{equation}
All the three tests are done considering that the observer $\mathcal{O}$ is located at the origin of the reference frame, with coordinates $(\eta_0, 0,0,0)$, and she/he sees the light coming from a comoving distant source $\mathcal{S}$, with coordinates $(\eta, 0,0, x^3)$. The light beam is propagating along the $x^3$ axis, with tangent vector $\ell^{\mu}=(\ell^{0},0,0,\ell^{3})$.

The first observable we test is the redshift: for a photon travelling along the $x^{\rm 3}$-axis it is
\begin{equation}
1+z^{\rm Sz}=\dfrac{\left(a \ell^0\right)|_{\rm \mathcal{S}} }{ \left(a \ell^0\right)|_{\rm \calO}}\, ,
\label{eq:Szekeres_z}
\end{equation}
where $\ell^0$ is obtained by solving the geodesic equation
\begin{equation}
\dfrac{d \ell^0}{d \eta} = - \ell^0 \left(2 \mathcal{H} + \dfrac{\dot{Z}}{Z}\right)\, . \label{eq:l0_Szekeres}
\end{equation}
In the above expressions $Z$ is given in Eq.~\eqref{eq_met_func}, $a$ is the scale factor \eqref{eq:a_LCDM}, and $\mathcal{H}$ the Hubble parameter \eqref{eq:E(z)} of the $\Lambda CDM$ background.
The variation $\Delta z(\rm BGO, Sz)$ refers to the numerical solution of Eq.~\eqref{eq:l0_Szekeres} as opposite to the $3+1$ geodesic solved by {\tt BiGONLight}.

The second observable under analysis is the angular diameter distance $D_{\rm ang}$. The standard procedure to compute $D_{\rm ang}$ is solving the Sachs focusing equation 
\begin{equation}
\dfrac{d^2 D_{\rm ang}}{d \lambda^2}= -\left(|\sigma|^2 + \dfrac{1}{2 }R_{\mu \nu}\ell^{\mu}\ell^{\nu}\right)D_{\rm ang}\, ,
\end{equation}
where the initial conditions given at $\cal O$ (i.e. the focusing point) are $D_{\rm ang}|_{\cal O}=0 $ and $\left. \dfrac{d D_{\rm ang}}{d \lambda}\right|_{\cal O}=(\ell_{\sigma}u^{\sigma})_{\rm \calO}$, and $|\sigma|$ is the shear that in the Szekeres model Eqs.~\eqref{eq:Sz_line}-\eqref{eq_met_func} simply vanishes, as shown in~\cite{Meures:2011ke}.
Using the Einstein equations to express $R_{\mu \nu}\ell^{\mu}\ell^{\nu}$ in terms of the density contrast and using conformal time instead of the affine parameter, the focusing equation assumes the form
\begin{equation}
\ddot{D}^{\rm Sz}_{\rm ang}+\dfrac{\dot{\ell}^0}{\ell^0} \dot{D}^{\rm Sz}_{\rm ang}=-  \dfrac{3}{2}\dfrac{\mathcal{H}_{\rm 0}^2\Omega_{\rm m_0}}{a}(\delta+1) D_{\rm ang}^{\rm Sz}\, ,
\label{eq:focusing_eq}
\end{equation}
where the dots refers to derivatives respect to conformal time $\eta$ and the initial conditions at the observation point are $ \ D_{\rm ang} \left|_{\rm \calO}\right.=0$ and $ \dot{D}_{\rm ang} \left|_{\rm \calO}\right.=\dfrac{(\ell_{\sigma}u^{\sigma})_{\rm \calO}}{\ell^0_{\rm \calO}}$.
In synchronous-comoving gauge the density contrast along the geodesic comes directly from the continuity equation and reads
\begin{equation}
\delta= - \dfrac{\mathcal{D} \beta_{\rm +}}{Z}=\dfrac{\dfrac{2}{3}\dfrac{\partial^2_{\rm x^{\rm 3}}\phi_{\rm 0}}{\stuff}\mathcal{D}}{1-\dfrac{2}{3}\dfrac{\partial^2_{\rm x^{\rm 3}}\phi_{\rm 0}}{\stuff}\mathcal{D}-\dfrac{2}{3}\dfrac{\partial^2_{\rm x^{\rm 3}}\phi_{\rm 0}}{\stuff} B ({x^{\rm 1}}^2+{x^{\rm 2}}^2)}\, .
\label{eq:Sz_delta}
\end{equation}
In our estimator Eq.~\eqref{eq:deltaO_Sz} the angular diameter distance $D_{\rm ang}^{\rm Sz}$ is obtained by integrating  Eq.~\eqref{eq:focusing_eq}, whereas $D_{\rm ang}^{\rm BGO}$ is obtained from Eq.~\eqref{eq:D_ang_BGO} with {\tt BiGONLight}.

The last test concerns the calculation of the redshift drift, namely the secular variation of the redshift of the source. It was calculated for some inhomogeneous cosmological models, see e.g. \cite{quartin, yoo2011redshift, Mishra2012,balcerzak2013redshift, mishra2014redshift}, but to our knowledge there is no expression for the Szekeres model considered here, thus we give in the following a short derivation.
Let us consider that during the proper time lapse $\delta \tau_{\mathcal{O}}$ the spacetime coordinates of the observer change from $x^{\mu}_{\mathcal{O}}=(\eta_{\mathcal{O}}, 0,0,0)$ to $X^{\mu}_{\mathcal{O}}=(\Theta_{\mathcal{O}}, 0,0,0)$. Similarly, in the corresponding proper time lapse $\delta \tau_{\mathcal{S}}$, the spacetime coordinates of the source change from $x^{\mu}_{\mathcal{S}}=(\eta_{\mathcal{S}}, 0,0,x^3)$ to $X^{\mu}_{\mathcal{S}}=(\Theta_{\mathcal{S}},0,0,x^3)$. 
Note that in this gauge $\mathcal{O}$ and $\mathcal{S}$ are comoving, meaning that they both have fixed spatial positions (i.e. $\delta x^i_{\mathcal{O}} = \delta x^i_{\mathcal{S}}=0$), but the time changes differently at $\mathcal{O}$ and at $\mathcal{S}$ (i.e. $\Theta_\mathcal{O} - \eta_\mathcal{O} \neq \Theta_\mathcal{S} - \eta_\mathcal{S}$). The redshift and the conformal time of the source change according to\footnote{On the R.H.S. of Eqs.~\eqref{eq:Sz_Z(t)}-\eqref{eq:Sz_T(t)} we use the fact that the source location $x^i_{\mathcal{S}}$ has components on the $x^3$ axis only.}
\begin{align}
\mathcal{Z}(\Theta_{\mathcal{S}}, x^{i}_{\mathcal{S}})&=z(\eta_{\mathcal{S}} ,x^3_{\mathcal{S}})+\delta z(\eta_{\mathcal{S}} ,x^3_{\mathcal{S}})\label{eq:Sz_Z(t)}\\
\Theta(x^{i}_{\mathcal{S}})&=\eta(x^3_{\mathcal{S}})+\delta \eta(x^{3}_{\mathcal{S}})\, ,\label{eq:Sz_T(t)}
\end{align}
while the same quantities at the observer position $X^{\mu}_{\mathcal{O}}$ are $\mathcal{Z}(X^{\mu}_{\mathcal{O}})=z(x^{\mu}_{\mathcal{O}})=0 $ and $ \Theta(X^{i}_{\mathcal{O}})=\eta(x^{i}_{\mathcal{O}})+\delta \eta(x^{i}_{\mathcal{O}})$.
Our final aim is to compute the redshift drift, namely 
\begin{equation}
\zeta=\dfrac{\delta \ln(1+z)}{\delta \tau_{\mathcal{O}}}\, .
\label{eq:Sz_def_drift}
\end{equation}
Let us begin with the variation of the source redshift with respect to the observer proper time  $\frac{\delta z}{\delta \tau_{\mathcal{O}}}$, where it is better to obtain first $\frac{d \delta z}{d x^3}$ (Eq.~\eqref{eq:Sz_delz_dx1}) and $\frac{d \delta \tau}{d x^3}$ (Eq.~\eqref{eq:Sz_deltau_dx}) separately, and then combine them to get an ODE (Eq.~\eqref{eq:z_drift_Szekeres}), whose solution gives the redshift drift.
The starting point are the differentials $\frac{d \eta}{d x^3}$ and $\frac{d z}{d x^3}$. The first is simply given by the null condition $\ell^0=-Z \ell^3$, and reads
\begin{equation}
 \frac{d \eta}{d x^3}=-Z\, ,
\label{eq:Sz_deta_dx}
\end{equation}
while $\frac{d z}{d x^3}$ is obtained by differentiating Eq.~\eqref{eq:Szekeres_z}\footnote{From now on we drop the index $\mathcal{S}$, since  all the quantities are evaluated at the source.}
\begin{align}
\dfrac{d z}{d x^3}=\dfrac{1}{ \left(a \ell^0\right)|_{\rm \calO}}\left(\frac{d a}{d x^3} \ell^0 +\frac{d \ell^0 }{d x^3} a \right)|_{\rm \calS}&=\dfrac{\left(a \ell^0\right)|_{\rm \calS}}{ \left(a \ell^0\right)|_{\rm \calO}}\left(\frac{1}{a}\frac{d a}{d \eta}\frac{d \eta}{d x^3} +\frac{1}{\ell^0}\frac{d \ell^0 }{d \eta}\frac{d \eta}{d x^3} \right)|_{\rm \calS} \nonumber \\
&=(1+z)\left(\mathcal{H} Z + \dot{Z} \right)\, ,
\label{qe:Sz_dz_dx} 
\end{align}
where we used Eq.~\eqref{eq:Sz_deta_dx}, Eq.~\eqref{eq:l0_Szekeres}, and the fact that the redshift at the observer is fixed.
Now we use Eq.~\eqref{eq:Sz_deta_dx} to differentiate Eq.~\eqref{eq:Sz_T(t)}
\begin{align}
\frac{d \delta \eta}{d x^3}=\frac{d \Theta}{d x^3}-\frac{d \eta}{d x^3}=-Z(\Theta, x^3)+Z(\eta, x^3)&=-\left[Z(\eta, x^3)+\dot{Z}(\eta, x^3) \delta \eta\right]+Z(\eta, x^3) \nonumber \\
&=-\dot{Z} \delta \eta\, ,
\label{eq:Sz_deleta_dx}
\end{align} 
and similarly for the redshift we have
\begin{equation}
\dfrac{d \delta z}{d x^3}=\dfrac{d \mathcal{Z}}{d x^3}-\dfrac{d z}{d x^3}=(1+z)\left( Z \mathcal{H}+\dot{Z}\right)^{\cdot}\delta \eta +\left( Z \mathcal{H}+\dot{Z}\right)\delta z \, ,
\label{eq:Sz_delz_dx1}
\end{equation} 
where we keep first-order terms in $\delta \eta$ and $\delta z$ only.
Rearranging terms and using Eq.~\eqref{qe:Sz_dz_dx} again, we get
\begin{equation}
\dfrac{d }{d x^3}\left(\dfrac{\delta z}{1+z} \right)=\left( Z \mathcal{H}+\dot{Z}\right)^{\cdot}\delta \eta\, . \label{eq:Sz_delz_dx2}
\end{equation}
The final step is to express the variation of the conformal time $\delta \eta$ in terms of the proper time at the observer $\delta \tau_{\mathcal{O}}$. We use their relation, which is simply
\begin{equation}
\delta \tau=\sqrt{|g_{\mu \nu} \delta x^{\mu} \delta x^{\nu}|}=a \sqrt{|-\delta \eta^2 + Z^2 \delta {x^{\rm 3}}^2|}= a \delta \eta\, ,
\label{eq:Sz_tau_eta}
\end{equation}
since $\delta x^i=0$. We need the derivative with respect to $x^3$, which reads
\begin{equation}
\frac{d \delta \tau}{d x^3}=\frac{d (a \delta \eta)}{d x^3}=\frac{d a}{d x^3}\delta \eta +a \frac{d \delta \eta}{d x^3}=\left( \frac{1}{a} \frac{d a}{d \eta}\frac{d \eta }{d x^3} - \dot{Z}\right) a \delta \eta=-\left( \mathcal{H} Z + \dot{Z}\right) \delta \tau\, ,
\label{eq:Sz_deltau_dx}
\end{equation}
and, together with Eq.~\eqref{qe:Sz_dz_dx} and Eq.~\eqref{eq:Sz_tau_eta},   the solution of the last equality is
\begin{equation}
\delta \eta=\frac{1}{a}\dfrac{\delta \tau_{\mathcal{O}}}{1+z}\, . \label{Sz_eta}
\end{equation}
By changing $x^3$ to conformal time $\eta$ with the chain rule $\frac{d}{dx^3}=\frac{d\eta}{dx^3}\frac{d}{d\eta}=-Z\frac{d}{d\eta}$, we get from Eq.~\eqref{eq:Sz_delz_dx2} the ODE in $\eta$ for the redshift drift in the Szekeres model
\begin{equation}
\frac{d\zeta}{d \eta}\equiv\frac{d}{d \eta}\left(\frac{\delta \log(1+z)}{\delta \tau_{\mathcal{O}}}\right)=-\frac{1}{a(1+z)}\frac{\left(H Z+ \dot{Z}\right)^{\cdot}}{Z}\, .
\label{eq:z_drift_Szekeres}
\end{equation}
For our test, in the estimator Eq.~\eqref{eq:deltaO_Sz}, $\zeta^{\rm Sz}$ is the numerical solution of Eq.~\eqref{eq:z_drift_Szekeres} and $\zeta^{\rm BGO}$ is the expression in Eq.~\eqref{eq:z_DRIFT_BGO} obtained with {\tt BiGONLight}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/Szekeres_z.pdf}
       \caption{Redshift}
        \label{fig:Sz_z}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/Szekeres_drift.pdf}
        \caption{Redshift drift}
        \label{fig:Sz_drift}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/Szekeres_Dang.pdf}
        \caption{Angular diameter distance}
        \label{fig:Sz_Dang}
    \end{subfigure}
    \caption{Variations in the Szekeres model, Eq.~\eqref{eq:deltaO_Sz}, for the redshift~\ref{fig:Sz_z}, the redshift drift~\ref{fig:Sz_drift}, and the angular diameter distance~\ref{fig:Sz_Dang}. The variable in the horizontal axis is the redshift in the Szekeres model.}\label{fig:Sz}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As for the $\Lambda$CDM model, also for the Szekeres model we have a very good agreement between the observables calculated using  the standard procedure and the observables from \texttt{BiGONLight}. The smallness of all the variations $\Delta z (\rm BGO, Sz)$, $\Delta \zeta(\rm BGO, Sz)$ and $\Delta D_{\rm ang}(\rm BGO, Sz)$ shown in Fig.~\ref{fig:Sz} means that our code could be a reliable tool for light propagation in inhomogeneous cosmologies, represented here with the Szekeres model, which is computationally more complicated than the homogeneous $\Lambda$CDM case.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A dust universe in Numerical Relativity}
\label{sec:ET}
The main application of the {\tt BiGONLight} package is the computation of observables from numerically simulated spacetimes. 
 For our test we choose to use the {\tt FLRWSolver}\footnote{{\color{blue}{\tt {https://github.com/hayleyjm/FLRWSolver\_public}}.}}, \cite{macpherson2017}, which is a module (or {\it thorn}) of the {\tt Einstein Toolkit} (ET), \cite{loffler2012einstein}: the ET is a collection of  open-source codes, called thorns, based on the {\tt Cactus} framework, \cite{goodale2002cactus}, which allows to solve the Einstein equations in the BSSN formulation of the 3+1 splitting, \cite{shibata1995evolution, baumgarte1998numerical}. The role of the {\tt FLRWSolver} is to provide the initial conditions in the form of linear perturbations around the Einstein-de Sitter (EdS) background, which are then evolved with the ET. Here, we limit ourself to the EdS background model and set perturbations to zero. In other words, we consider a FLRW model in which the Universe is flat and contains only cold dark matter.  The line element of the EdS model in conformal time is
\begin{equation}
ds^2={a^2_{\rm EdS}}(\eta) \left(-d\eta^2+ {dx^2}^2 + {dx^2}^2 + {dx^3}^2 \right)\, ,
\end{equation}
where $a_{\rm EdS}(\eta)=\eta^2$ is the scale factor. 
We carry out the simulation in a cubic domain $-L \le \{x^1, x^2, x^3 \}\le L$ with periodic boundary conditions and spatial resolution $\Delta x=\Delta y=\Delta z= \frac{L}{20}$, where $L$ is the simulation unit length in Mpc\footnote{The physical value is $L=268.11\, {\rm Mpc}$, as it is explained in \ref{apx:Units}.}. The initial data are given at $\eta_{\rm in}=L$ and such that $\gamma^{\rm in}_{i j}=\delta_{i j}$. % and $\rho_{\rm in}= \frac{3 \mathcal{H}_{\rm in}^2}{8 \pi}=\frac{3}{2 \pi L^2}$. 
 The simulation runs with the ET up to $\eta_0=33.2 L$, which corresponds to integrating from redshift $z = 1100$ to present time $z=0$, and we choose a fixed temporal resolution $\Delta \eta=\frac{L}{100}$ due to computational time convenience.
To give an estimation of the simulation error we define
\begin{equation}
\Delta a({\rm ET, EdS}) \equiv \dfrac{a^{\rm ET}-a^{\rm EdS}}{a^{\rm EdS}}\, ,
\label{eq:DeltaA}
\end{equation}
which is the variation between the analytical scale factor in EdS, i.e. $a^{\rm EdS}=\eta^2$ and the scale factor from the numerical simulation $a^{\rm ET}={\rm det}(\gamma_{i j})^{\frac{1}{6}}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
    \centering
        \includegraphics[width=0.8\linewidth]{figures/ET_a_StoO_fullRange.pdf}
\caption{Scale factor in EdS: ET simulation precision. The variable on the horizontal axis is the conformal time in computational units (see \ref{apx:Units}).}
    \label{fig:scale_ET}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
The result, shown in Fig.~\ref{fig:scale_ET}, is of the order of $ 10^{-10}$ and this value is determined by the specific setting that we choose for the ET simulation.

The simulated EdS model constitutes the playground of our tests. We perform light propagation with {\tt BiGONLight} using forward integration in time with the method described in Sec.~\ref{sec:W3+1}. We start from the source $\mathcal{S}$, placed at redshift $z= 10$ in $x^{\mu}_{\calS}=(\eta_{\calS}, 0, 0, 0)$, and we end at the observer $\calO$. The emitted light moves along the diagonal of the cubic domain with initial tangent vector $\ell^{\mu}_{\calS}=(-1, -\frac{1}{2}, \frac{1}{2},\frac{\sqrt{2}}{2})$, until it reaches the observer at $x^{\mu}_{\calO}$. 
The numerical accuracy in the calculation of the observables is tested by means of the variation $\Delta O({\rm BGO, ET})$ defined as
\begin{equation}
\Delta O({\rm BGO, EdS}) \equiv \dfrac{O^{\rm BGO}-O^{\rm  EdS}}{O^{\rm  EdS}}\, ,
\label{eq:deltaO_ET}
\end{equation}
where $O^{\rm BGO}$ is computed numerically with {\tt BiGONLight} using as input the EdS model simulated with the ET and $O^{\rm EdS}$ is the analytical expression in the EdS model that reads
\begin{align}
D_{\rm ang}^{\rm EdS}&=\dfrac{2 a_0}{\mathcal{H}_{\rm 0}}\dfrac{\sqrt{1+z}-1}{(1+z)^{\frac{3}{2}}} \label{eq:ET_Dang}\, , \\
D_{\rm par}^{\rm EdS}&=\dfrac{a_0}{\mathcal{H}_{\rm 0}} \dfrac{\sqrt{1+z}-1}{\frac{3}{2}\sqrt{1+z}-1} \label{eq:ET_Dpar}\, , \\
\zeta^{\rm EdS}&=\dfrac{\mathcal{H}_{0}}{a_0} (1-\sqrt{1+z}) \label{eq:ET_drift} \, .
\end{align}
These are obtained by integrating Eqs.~\eqref{eq:D_ang_FLRW}-\eqref{eq:z_drift_FLRW} with $\Omega_{\rm m_0}=1$ and $\Omega_{\rm \Lambda}=0$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/ET_z_StoO.pdf}
       \caption{Redshift}
        \label{fig:ET_z}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/ET_drift_StoO.pdf}
        \caption{Redshift drift}
        \label{fig:ET_drift}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/ET_Dang_StoO.pdf}
        \caption{Angular diameter distance}
        \label{fig:ET_Dang}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/ET_Dpar_StoO.pdf}
        \caption{Parallax distance}
        \label{fig:ET_Dpar}
    \end{subfigure}
    \caption{Variations in the EdS model with ET, Eq.~\eqref{eq:deltaO_ET}, for the redshift~\ref{fig:ET_z}, the redshift drift~\ref{fig:ET_drift}, the angular diameter distance~\ref{fig:ET_Dang}, and the parallax distance~\ref{fig:ET_Dpar}. The variable in the horizontal axis is the redshift in EdS.}
    \label{fig:ET}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The results are shown in Fig.~\ref{fig:ET}. 
What we see is the error on $\Delta O({\tt BGO, EdS})$ which has in principle two contributions: one from the simulation of the EdS model and the other from the simulation of light propagation. We have already isolated the second contribution coming from {\tt BiGONLight} in the $\Lambda$CDM test. Indeed, since we use the analytical solution for $\Lambda$CDM both in the numerical and analytical computation for the observables, the error $\Delta O({\tt BGO, \Lambda CDM})$ we find in Fig.~\ref{fig:LCDM} is entirely due to the simulation of light propagation and is of the order of $10^{-22} \div 10^{-31}$.
On the other hand, in Fig.~\ref{fig:scale_ET} we see that the accuracy of the ET simulation we use is much larger, i.e. of the order of $10^{-10}$, which is of the same order of the one for $\Delta O({\tt BGO, EdS})$ in Fig.~\ref{fig:ET}. Therefore we can conclude that the final error on the observables we find in Fig.~\ref{fig:ET} is settled by the accuracy of the ET in simulating the EdS model. Let us finally remark that for this test we perform light propagation using forward integration, namely from the source $\calS$ to the observer $\calO$. We also repeated the computation of $\Delta O({\tt BGO, EdS})$ using backward integration, form $\calO$ to $\calS$, in {\tt BiGONLight} and we found the same results.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	

\endinput

